Distributed Interview Selection for Stable Matching in Large Random Markets

In real-world settings of the Deferred Acceptance stable matching algorithm, such as the American medical residency match (NRMP), school choice programs, and various national university entrance systems, candidates need to decide which programs to list. In many of these settings there is an initial phase of interviews or information gathering which affect the preferences on one or both sides. We ask: which interviews should candidates seek? We study this question in a model, introduced by Lee (2016) and modified by Allman and Ashlagi (2023), with preferences based on correlated cardinal utilities. We describe a distributed, low-communication strategy for the doctors and students, which lead to non-match rates of $e^{(-\widetilde{O}(\sqrt{k}))}$ in the residency setting and $e^{(-\widetilde{O}(k))}$ in the school-choice setting, where $k$ is the number of interviews per doctor in the first setting, and the number of proposals per student in the second setting; these bounds do not apply to the agents with the lowest public ratings, the bottommost agents, who may not fare as well. We also obtain bounds on the expected utilities each non-bottommost agent obtains. These results are parameterized by the capacity of the hospital programs and schools. Larger capacities improve the outcome for the hospitals and schools, but don't significantly affect the outcomes of the doctors or students. Finally, in the school choice setting we obtain an $\epsilon$-Nash type equilibrium for the students apart from the bottommost ones; importantly, the equilibrium holds regardless of the actions of the bottommost students. We also discuss to what extent this result extends to the residency setting. We complement our theoretical results with an experimental study that shows the asymptotic results hold for real-world values of $n$.

==> app-ext.tex <==

\subsection{The Request Interview Setting}\label{sec::app-full-int}

\begin{theorem}\label{clm::improved-eps}
% Let $\alpha_l = \big(\frac{8b(c+2)\kappa}{2a-1}\big)^{1/2}\cdot \big(\frac{\ln n}{n}\big)^{1/2}$, the minimum allowed value for $\alpha$, and let $\alphabar=\big(\frac{4(4a+1)\ln k}{k}\big)^{1/2}$, the value of $\alpha$ when $\nu_d=\nu_h=1$.
Suppose that the hospitals list the doctors they interview in preference order and all but the bottommost $a\alpha$ doctors follow the recommended strategy.
Then, all but the bottommost $a\alpha$ doctors achieve an $\eps$-Nash equilibrium,
with the following bounds, depending on the values of $\nu_d$ and $\nu_h$.
Let $\alpha_{\min}= 3\exp\big(-\frac{k}{4(4a+1)}\big)$.

Case 1: $\alpha_{\min}\le \alpha\le \nu_h\le \nu_d\le 1$. \\
Let $\sigma=\min\big\{1,\frac{3\kappa}{8}\big\}$.
With our choice for $\alpha$ given shortly, this amounts to 
$\nu_h\ge \frac {v_d(4a+1)}{k\sigma} \ln \frac{ek\sigma}{\nu_h\nu_d(4a+1)}$.
Let $x=\frac{\nu_h\nu_d(4a+1)}{k\sigma}$; then we set $\alpha = x^{1/2}\cdot\big[\ln (ex)^{1/2} \big]$.
Then $\eps= O(\alpha)$,
and the mismatch/not-fully matched rates for the doctors and hospitals are
$\exp\big(-\frac{\alpha k}{(4a+1)\nu_h}\big)$
and $\exp\big(-\frac{3\kappa k\alpha}{8(4a+1)\nu_d}\big)$, respectively.

Case 2: $\max\{\alpha_{\min},\nu_h\} < \alpha\le \nu_d\le 1$.\\
Then $\eps= O(\alpha)$, with
$\alpha \ge \frac{4(4a+1)\nu d}{k}\cdot \ln\big(\frac{3ek}{4(4a+1)\nu d}\big)$ and $3k\ge 4(4a+1)\nu_d$;
the mismatch/not-fully matched rates for the doctors and hospitals are
$\exp\big(-\frac{k}{4a+1}\big)$ and $\exp\big(-\frac{3\kappa k\alpha}{8(4a+1)\nu_d}\big)$.

Case 3: $\nu_h\le \nu_d\le 3\alpha$.\\
We set $\alpha = \alpha_{\min}$.
Then $\eps= O(\alpha_{\min})$ and
the mismatch/not-fully matched rates for the doctors and hospitals are
$\exp(-k/4(4a+1))=\frac 13\alpha_{\min}$ and $\exp\big(-\frac{\kappa k}{8(4a+1)}\big)$.
\end{theorem}
\begin{proof}
    Let $\beta_d=\min\big\{1,\frac{\alpha}{\nu_d}\big\}$ 
    and $\beta_h=\min\big\{1,\frac{\alpha}{\nu_h}\big\}$.
    To maintain the surplus bounds from the setting in which doctors select the interviews, the simple interview setting for short, we need to ensure that the fraction of unmatched doctors or hospitals is at most $\alpha$---see Claims \ref{lem::surplus-hosp-prop-one-doc}, \ref{lem::surplus-hosp-prop-one-hosp}, \ref{clm::surplus-interval-hosp-prop}, and \ref{clm::surplus-interval-doc-prop}; i.e.\ we need 
    $3\exp\big(-\frac{\beta_h\cdot k}{4(4a+1)}\big)\le \alpha$
    and $3\exp\big(-\frac{\beta_d\cdot k}{4(4a+1)}\big)\le \alpha$. As $\beta_h\ge \beta_d$,
    $\alpha \cdot \exp\big(\frac{\beta_d\cdot k}{4(4a+1)}\big) \ge 3$ suffices.
    Accordingly, when $\beta_d =\frac{\alpha}{\nu_d}$,  $\alpha \ge \frac{\nu_d\cdot 4(4a+1)}{k}\ln \frac{3k}{\nu_d\cdot4(4a+1)}$ suffices, if $3k\ge e\nu_d\cdot4(4a+1)$,
    and when $\beta_d=1$, $\alpha \ge 3\exp\big(-k/4(4a+1)\big)$ suffices.

    The value of $\eps$ in the $\eps$-Nash analysis (see \Cref{lem::typical-student-eps-nash}) is dominated by two terms: the size $2a\alpha$ of the cone, and the probability that the doctor's match has an interview value less than $1-\psibar_d$; to obtain $\eps=O(\alpha)$, we want the second term to be bounded by $O(\alpha)$. 

    To obtain the doctor non-high-quality match failure probability we set $\psibar_d=\beta_d$, giving a non-high-quality-match failure probability of at most $\exp\big(-\frac{k\beta_h\beta_d}{(4a+1)}\big)$, and we want this to be at most $2\alpha$ (high-quality means that the match has interview value at least $\psibar_d$).
    Likewise, for the hospital not-fully matched high-quality failure probability, we set $\psibar_h=\beta_h$, giving a not-fully matched high-quality failure probability of at most $\exp\big(-\frac{3\kappa k\beta_h\beta_d}{8(4a+1)}\big)$, which we also want to bound by $2\alpha$.
    Then $\alpha\exp\big(\frac{k\beta_h\beta_d}{(4a+1)}\big)\ge 1$  suffices.
    
    To complete the analysis we need to consider several cases.\\
    Case 1. $\alpha\le \beta_h\le \beta_d\le 1$.\\
    To satisfy the second condition
    $\alpha \ge \big(\frac{\nu_h\nu_d(4a+1)}{k\sigma})^{1/2}\cdot \big[\ln\big(\frac{ek\sigma}{\nu_h\nu_d(4a+1)})^{1/2}\big]^{1/2}$ suffices, so long as $k\ge \nu_u\nu_d(4a+1)\sigma$.
    Combining conditions yields the first bound.
\hide{    
    Then for the doctor high-quality mismatch condition, we want
    $\alpha \ge \big(\frac{\nu_d\nu_h(4a+1)\ln 1/\alpha}{k}\big)^{1/2}$;
    $\alpha \ge \big(\frac{\nu_d\nu_h(4a+1)}{k}\cdot \ln \frac{k}{\nu_d\nu_h(4a+1)}\big)^{1/2}$ suffices.
   Similarly, for the hospital mismatch condition, $\alpha \ge \big(\frac{3\kappa\nu_d\nu_h(4a+1)}{8k}\cdot \ln \frac{8k}{3\kappa\nu_d\nu_h(4a+1)}\big)^{1/2}$ suffices.
   }
\\
    Case 2. $\beta_h<\alpha \le \beta_d\le 1$.\\
    The first constraint, $\exp\big(\frac{k\alpha}{\nu_d\cdot 4(4a+1)}\big)\ge 3$ is now the tighter one, so $\alpha \ge \frac{4(4a+1)\nu d}{k}\cdot \ln\big(\frac{3ek}{4(4a+1)\nu d}$ suffices,
    if $3k\ge 4(4a+1)\nu_d$.
    \\
    Case 3: $\nu_h\le \nu_d\le 3\alpha$.\\
    Here it suffices to set $\alpha =3\exp\big(-\frac{k}{4(4a+1)}\big)$.
\end{proof}

==> app-student-school.tex <==
\subsection{The Student-School Setting}

\begin{lemma}\label{lem::doctors-high-value-match-prob-noid}
Let $\delta>0$ be an arbitrarily small constant.
    Let $d$ be a doctor with public rating at least $a\alpha$.
    Suppose we run the hospital-proposing double-cut DA for doctor $d$ using the discretized utilities
as specified in \Cref{clm::discrete-dist-idio}.
    Suppose the fraction of unmatched hospitals with public rating in $[r(d)+(a+1)\alpha,1)$ is at most $3\exp\big(-\alpha\kappa k/4(4a+1)\big)$.
    Also, suppose that the event ${\mathcal B}$ does not occur.
    Finally, suppose we run the hospital-proposing double-cut DA for $d$.
     Then the probability that $d$ fails to receive a match for which it has interview value $1-\psibar_d$ or larger is at most $\exp\big(-\frac{4k\psibar_d}{4a+1}\big)$, if both $a\ge 5$ and $\alpha\cdot\exp\big(\alpha k/4(4a+1)\big)\ge 3$.
\end{lemma}

The final lemma is a simplified version of \Cref{lem::hosp-high-value-match-prob}, obtained by setting
$\psibar_h=0$.
\begin{lemma}\label{lem::hosp-high-value-match-prob-noid}
Let $\delta>0$ be an arbitrarily small constant.
    Let $h$ be a hospital with public rating at least $a\alpha$.
    Suppose we run the doctor-proposing double-cut DA for hospital $h$ using the discretized utilities as specified in \Cref{clm::discrete-dist-idio}.
    Suppose the fraction of unmatched doctors with public rating in $[r(d)+(a+1)\alpha,1)$ is at most $3\exp\big(-\alpha k/4(4a+1)\big)$.
    Also, suppose that the event ${\mathcal B}$ does not occur.
    Finally, suppose we run the doctor-proposing double-cut DA for $h$.
     Then the probability that $h$ fails to obtain $\kappa$ matches is at most $\exp\big(-\frac{3\kappa k\alpha}{8(4a+1)}\big)$, if $a\ge 5$, $k\ge 4a+1$, and $\alpha\cdot\exp\big(3\alpha k/4(4a+1)\big)\ge 3$.
\end{lemma}





\subsubsection{Proof of \Cref{lem::doctors-high-value-match-prob-noid}}\label{sec::proof-doc-match-prob-noid}

We fix the utilities for all edges other than those incident on $d$.
\Cref{clm::matching-bounds-extend} continues to hold here.
The analysis from the resident setting simplifies.


\begin{claim}\label{lem::surplus-hosp-prop-one-doc-noid}
    Suppose the following bad events do not occur:
    $\Bdbm([r(d),1))$ and $\Bhbf([r(d)-a\alpha,r(d)+a\alpha)\cup[r(d)+(a+1)\alpha,1))$, and also suppose that both $a\ge 5$ and $\alpha\cdot\exp\big(3\alpha\kappa k/8(4a+1)\big)\ge 3$.
    Then the surplus $s\ge 2\alpha n/\kappa$.
\end{claim}
\begin{proof}
    As $\Bdbm([r(d),1))$ does not occur, the number of doctors with public rating at least $r(d)-\alpha$ is at most $[1-r(d)+\frac 12\alpha ]n$. 
    By the assumption in \Cref{lem::doctors-high-value-match-prob-noid} and by \Cref{clm::matching-bounds-extend}, the number of not-fully matched hospitals in $[r(d)+(a+1)\alpha,1)$ is at most
    $3\frac n{\kappa}\cdot\exp\big(-3\alpha\kappa k/8(4a+1)\big)\le  \alpha \cdot \frac n{\kappa}$, if $\exp\big(- 3\alpha\kappa k/8(4a+1)\big)\le \frac 13\alpha$.
    In addition, some or all of the hospitals in $[r(d)+a\alpha,r(d)+(a+1)\alpha)$ may not be fully matched.
    As $\Bhbf([r(d)-a\alpha,r(d)+a\alpha)\cup[r(d)+(a+1)\alpha,1))$ does not occur,
    the number of hospitals with public rating in this range is at least $[1-r(d)+(a-\frac32)\alpha] n/\kappa$.
    Thus the surplus, the number of not-fully matched available hospitals in $d$'s cone, i.e., hospitals that could propose to $d$, is at least
    \begin{align*}
        \big[1-r(d)+(a-\tfrac32)\alpha\big] \cdot\frac{n}{\kappa} - \big[1-r(d)+\tfrac 12\alpha\big]\cdot\frac{n}{\kappa} -  \alpha \cdot\frac{n}{\kappa}
        \le \big(a - 3\big)\alpha\cdot \frac{n}{\kappa}\ge 2\alpha \cdot \frac{n}{\kappa},
    \end{align*}
    if $a\ge 5$.
\end{proof}

The stochastic dominance argument is not needed here. A simple direct argument suffices.

\begin{claim}\label{noid-doctor-no-match-prob}
    Suppose the surplus $s\ge 2\alpha \frac{n}{\kappa}$, and $\Bhbm(C(d))$ does not occur.
    Then the probability that $d$ receives no proposal with interview value
    at least $1-\psibar_d$ is at most $\exp\big(-4k\psibar_d/(4a+1)\big)$.
\end{claim}
\begin{proof}
  Consider a run of the double-cut DA for $d$. It ends with at least $s$ hospitals in $C(d)$ having either run through all their proposals or finishing with a proposal to $d$. Since the edges from $d$ are uniformly randomly distributed over $C(d)$, the probability that none of the surplus hospitals has an edge to $d$ with interview value
    at least $1-\psibar_d$ is at most $\big(1 - \frac{\psibar_d \cdot s}{(2a+\frac12)\alpha n/\kappa}\big)^{k}$, as $\Bhbm(C(d))$ does not occur. This probability is at most $\exp\big(-4k\psibar_d/(4a+1)\big)$.
\end{proof}



\begin{claim}\label{clm::conditions-hosp-prop-one-doctor-noid}
 The conditions in Claims~\ref{lem::surplus-hosp-prop-one-doc-noid} and~\ref{noid-doctor-no-match-prob} amount to the following constraints: $a\ge 5$,  and $\alpha\cdot\exp\big(\alpha k/4(4a+1)\big)\ge 3$.
 They also exclude events with total probability at most $3n^{-(c+1)}$.
 \end{claim}


\subsubsection{Proof of \Cref{lem::doctors-interval-non-match} for the School Setting}
%\label{sec::doc-int-noid-no-match}
%
The proof is very similar to the proof in the residency setting.
We slightly reduce the set of participating doctors to be those with public rating at least $f$.
The effect is to increase the surplus (but we are going to ignore the slightly improved bound we could obtain).
The main change is in the definition of $\qtilde(v)$. Where before we choose $s-x-y$ hospitals with the smallest residual utilities, now we simply choose any $s-x-y$ hospitals that have not yet attempted to propose to $I$, i.e.\ they still have utility at least $g$. Otherwise the argument is unchanged.


\subsubsection{The $\eps$-Nash Equilibrium for all but the Bottommost Doctors}

We have the same constraints as in the residency setting and the same bad events, so
Claims \ref{clm::final-cstrnts-idio} and 
\ref{clm::prob-B} continue to hold.

\begin{lemma}\label{lem::typical-student-eps-nash-noid}
Suppose the constraints in \Cref{clm::final-cstrnts-idio} hold.
    Let $d$ be a doctor with public rating at least $a\alpha$, and let $\alpha=\frac{4(4a+1)\ln k}{k}\cdot\max\{1,2/\kappa\}$.
        In expectation, ex-ante, $d$ could improve her utility by at most $\taubar +22n^{-(c+1)}+ 3/k^4+8a\cdot \frac{(4a+1)\ln k}{k}\cdot\max\{1,2/\kappa\}=O(\ln k/k)$, if $k\ge a+\frac14$.
\end{lemma}
\begin{proof}
If $\mathcal B$ does not occur, $d$ could improve her private value by at most $\taubar$.
If $\mathcal B$ occurs, $d$ could improve her outcome by at most $2+\taubar$ units of utility; 
by \Cref{clm::prob-B}, $\mathcal B$ occurs with probability at most $11n^{-(c+1)}$.
This accounts for the first two terms.

By \Cref{lem::doctors-high-value-match-prob-noid}, $d$ fails to obtain a match providing utility $r(d)+2-\taubar-\psibar_d$ with probability at most $\exp\big(-\frac{k\psibar_d}{4a+1}\big)$.
Setting  $\psibar_d=\alpha$, yields a probability of at most $\exp\big(-\frac{4(4a+1)\ln k}{4a+1}\big)\le 1/k^4$.  Therefore changing her proposals to improve her match probability (not that it is clear how to do this), yields an expected gain of at most $3/k$, which accounts for the third term in the bound.

When changing her bids, in expectation, there is no improvement in the interview value.

When bidding below her cone the public rating of potential matches only decreases.
When bidding in cone, the public rating can improve by
at most $2a\alpha=2a\cdot \frac{4(4a+1)\ln k}{k}\cdot\max\{1,2/\kappa\}$, which accounts for the fourth term in the bound. 

Finally, if $d$ switches to one or more proposals above her cone, we show that the expected gain is fairly small.
In expectation, there is no improvement in the interview value. So the gain comes from the improved public rating. A move from the bottom of the cone to the top increases the public rating by up to $2a\alpha$. A further increase of $x$ to the public rating
has a match probability of
at most $\exp\big(-\frac{4k x}{4a+1}\big)$, as can be seen by setting $\psibar_h= x$ in \Cref{lem::doctors-high-value-match-prob-noid}. For $x\ge 0$, the expected improvement due to the increase by $x$, $x\cdot \exp\big(-\frac{4kx}{4a+1}\big)$, is maximized at $x=0$, if $k \ge a+\frac14$.  This is no better than the gains in-cone.
\end{proof}

We note from the proof of \Cref{clm::final-cstrnts-idio} that the constraints in \eqref{eqn::alpha-cstrnt} suffice.
Substituting $\alpha =\frac{4(4a+1)\ln k}{k}\cdot\max\{1,2/\kappa\}$ yields the constraints in the next claim.

\begin{claim}\label{clm::final-cstrnts-noid}
    With $\alpha=\frac{4(4a+1)\ln k}{k}$, $a=5$, and $b=3$, constraints \Cref{eqn::alpha-cstrnt} and \Cref{lem::typical-student-eps-nash-noid} are satisfied if 
\begin{align*}
 %       1&\le \Big(\frac{\ln k}{k}\Big)^{1/2}\cdot\exp\Big(\frac{(4k\ln k)^{1/2}}{20}\Big)\\
        8&\le k \le \frac 12(c+2)\ln n \notag\\
         \frac{n}{\ln n}& \ge\frac{(c+2) k^{5}\kappa^2}{25\ln k}.
    \end{align*}
\end{claim}

This concludes the proof of \Cref{thm::eps-nash-no-idio-large-cap}.

Finally, we show that there is exactly one stable matching in this setting.
This is straightfoward, but does not appear to be widely known.

\begin{claim}\label{clm::unique-sm}
    In the student-school setting the stable matching is unique.
\end{claim}
\begin{proof}
    We will show that the school proposing DA yields the same outcome as the student proposing DA.
    First, consider the student-proposing DA. We start by having student 1 propose. Once students $1$ to $i$ are matched, student $i+1$ proposes. Note that every hospital prefers its current matches to student $i+1$. So all tentative matches are actually final matches.
    Now consider the school proposing DA. Note that the schools all order the students by decreasing public rating.
    Recall that we are free to choose which available school makes the next proposal.
    So we first have the schools propose to the rank 1 student. One school matches, namely the school preferred by student 1. This is the school student 1 would match with in the student-proposing DA.
    Then all non-fully matched schools propose to student 2. Once the first $i$ students have received proposals (it some cases there may be 0 proposals to a student), the not-fully matched schools propose the student $i+1$.
    The inductive claim is that the two runs of DA produce the same matches for the first $i$ doctors.
    But then whether the hospitals propose to doctor $i+1$, or doctor $i+1$ proposes to the hospitals, 
    they are going to obtain the same match, for in the first case, doctor $i+1$ selects her favored hospital among the available hospitals, and in the second case, this is her preferred choice among the available hospitals, which demonstrates the inductive claim.
\end{proof}




  

==> bottom-agents.tex <==

We show that the bottommost agents have a fairly small $O((\ln k)^{1/2}/k^{1/4})$ mismatch rate.

We start by considering the doctors.
We will need to group the edges from the doctors according to the hospital interview values.

\begin{definition}\label{def::hosp-low}
    $h$'s interview value for doctor $d$  is \emph{low} if it 
    is in the range $[2a\alpha-r(d),1-r(d))$, and
    it is \emph{very low} if it is in the range $[0,2a\alpha-r(d))$.
    Otherwise the interview value is \emph{high}.
    We also say the corresponding edges $(d,h)$ are low, very-low, or high.
\end{definition}
When the $h$'s interview value is low it obtains a utility in the
range $[2a\alpha,1)$, and when it is very low it obtains a utility in the range
$[0,2a\alpha)$.

Let $D$ be the set of doctors all of whose edges give the hospitals low or very low interview values.

\begin{claim}\label{clm::size-D}
Suppose $\alpha = {(2a+\frac12)\ln k/k}^{1/2}$. Then
    $|D|< n/8k$ with probability at most $n^{-(c+2)}$, if $\frac{n}{\ln n} \ge 32(c+2)k$.
\end{claim}
\begin{proof}
Consider a doctor $d$ with public rating less than $\alpha/{2(2a+\frac12)k\ln k}^{1/2}=1/2k$.
The probability that an edge $(d,h)$ is high is
at most $1/2k$.
So, the expected number of high edges from $d$ is at most $1/2$.
Therefore the
the probability that $d$ has no high edges is at least $1/2$.
Therefore, the expected number of doctors with no high edges and public rating less than $1/2k$ is at least $n/4k$,
and by a Chernoff bound it is at least $n/8k$
with failure probability at most $\exp\big(-n/32k\big)\le n^{-(c+2)}$, if
$\frac{n}{\ln n} \ge 32(c+2)k$.
\end{proof}

Now, consider running the doctor proposing DA, at the point where all the doctors except those in $D$  are matched or have run through their entire preference lists, while the doctors in $D$ have not yet made any proposals. There must be at least $|D|-m$ available slots, where $m$ is the number of unmatched
hospital slots for hospitals with public ranking at least $a\alpha$; let $\Sd$ denote the set of these slots.
We will show that $m=o(|D|)$.
Now consider what happens as the doctors in $D$ propose.
Either they find a match in $\Sd$, or they match elsewhere causing another doctor to be displaced, which we call bumping. The chain of bumping may end in $\Sd$. We need to monitor how often a doctor outside of $D$ is placed in $\Sd$, and furthermore if it is due to a high edge.
The probability of a high edge is at most $(2a+1)\alpha$.
So this accounts for at most $(2a+1)\alpha|D|$ of the slots. \rnote{Not quite right. Need to argue that most of $\Sd$ is in the bottom $a\alpha$ public rating. Why? Revision of $I$ hospital bound: removal of $D$ makes little difference.}
Also, a doctor outside of $D$ may be bumping through $\Sd$ and eventually gets to a high edge.}

Each doctor will have $O(\sqrt{k/\ln k})$ edges to $\Sd$, so on average there are $O([\kappa k/\ln k]^{1/4})$ proposals to each hospital with slots in $\Sd$.
 


==> double-cutDA-ver2.tex <==
\section{Overview of the Double Cut DA}\label{sec::double-cutDA}

This methodology was introduced in \cite{AC23} to bound the number of proposals needed to obtain a stable matching with high probability, meaning probability $1-n^{-c}$, for any constant $c$ (the bound on the number of proposals increases as $O(\sqrt{c})$).

\input{double-cut-figure}

% There are two sets of agents, doctors and hospitals.
Suppose we want to show that a hospital $h$ receives a high-quality proposal with high probability.
% To keep the overview simple, let's suppose there are $n$ doctors and $n$ hospitals.
Our overview uses the setting from \cite{AC23}. There the doctors and hospitals obtain their utilities for potential partners by adding a private value for that partner to the partner's public rating, where values and ratings are uniform random draws from $[0,1)$. 
% \footnote{A natural way of obtaining such a number is by repeated sampling of a 0/1 choice, stopping when the number is unique; this will always be in the range $[0,1)$.}

To demonstrate the quality of $h$'s match, if any, we analyze a partial run of the doctor-proposing DA.
Agarwal and Cole called this the double-cut DA for $h$.
The participants are the hospitals with public rating in the range $[r(h)-\alpha,1)$ and the doctors with public rating in the range $[r(h)-a\alpha,1)$, where $a>1$ and $\alpha$ are suitable parameters.
Our choice of $\alpha$ will ensure that with high probability there are at least $\alpha n$ more doctors than hospitals participating in the partial run.

The run of the doctor-proposing DA is further restricted as follows. Each doctor in $h$'s cone, i.e.\ with public rating in $[r(h)-a\alpha,r(h)+a\alpha)$, stops making proposals as soon as she reaches a proposal providing her utility less than $r(h)+1-\alpha$ (she does not make this proposal). This means that she will not make any proposals to hospitals with public rating less than $r(h)-\alpha$.
She also stops if she is about to make a proposal to $h$; this will then be her final proposal, so long as it provides utility at least $r(h)+1-\alpha$. The doctors above $h$'s cone are unconstrained. 

In order to obtain useful bounds on the quality of $h$'s match one needs to show the following three bounds on the performance of the double-cut DA.
\begin{enumerate}
    \item There is a sufficiently larger surplus $s$ of doctors who could either propose to $h$ or remain unmatched (depending on their random choices of private value). 
    \item If each of the $s$ surplus doctors $d$ were to propose independently to $h$ with probability $\alpha$ (because $d$ has a private value for $h$ providing her utility at least $r(h)+1-\alpha$), then $h$ would receive a high-quality match with the desired probability. %(Note that this is not what actually happens.)
    \item Inconveniently, the actions of the surplus doctors need not be independent. The final step is to show that the case of independent proposals yields a failure probability that is at least as large as the failure probability for the actual run of the double-cut DA. This argument was carried out by a methodology we name \emph{tree stochastic dominance}.\footnote{This name is being coined in this paper.}
\end{enumerate}


An important property of the double-cut DA for $h$ is that the outcome for $h$ in the full run of the doctor-proposing DA is at least as good as its outcome in the double-cut DA (see \Cref{clm::double-cutDA-provides-bounds} below).
The full analysis uses analogous runs of a double-cut DA for doctors.
An immediate implication of this analysis is that with high probability, for each doctor $d$, her possible matches have public ratings in the cone $C(d)=[r(d)-a\alpha,r(d)+a\alpha)$, and similarly for the hospitals.

In the current work, we need to substantially modify Steps 1 and 3 above to achieve our new results.

In \cite{AC23}, with high probability---meaning polynomially small failure probability---all the doctors more than $a\alpha$ above $h$ in public rating will be matched in the current double-cut DA (this stems from a top-down induction we will explain later) and these matches are all with hospitals above $h$. This leaves roughly $a\alpha n$ hospitals and $2a\alpha n$ doctors unmatched, and furthermore all these doctors are in $h$'s cone. Consequently there is a surplus of $\alpha n$ doctors who either propose to $h$ or remain unmatched, and with high probability, among these doctors some will have high private values for $h$, and $h$ will have high private values for them, resulting in a high private value match on both sides.

\hide{
Step 1 depended on every agent ending up matched with high probability (except for some of the bottommost agents, meaning those with public rating less than $a\alpha$).
Then the surplus is simply the number of participating doctors minus the number of participating hospitals, and with high probability these numbers are close to their expected value, as shown by Chernoff bounds. On setting $a=3$, they obtain a surplus of size at least $\alpha n$.
}

In the current work, as we are limiting each doctor to making $k$ proposals, we no longer have a polynomially small probability of failing to match. In fact, we expect at least an $e^{-\Theta(k)}$ fraction of the doctors to fail to match. In computing the surplus, we will need to subtract the number of unmatched doctors whose public rating lies above $h$'s cone (because they fail to match hospitals above $h$, which therefore could be matched by some of doctors in the previous surplus, thereby reducing the surplus). As it turns out, we will need a high-probability bound on this number, and on the analogous numbers for the not-fully matched hospitals.

The difficulty is that while we can obtain an upper bound on the probability that a single hospital (or doctor) is unmatched, and hence an upper bound on the expected number of unmatched hospitals, we cannot apply a Chernoff bound, as the probabilities for the various hospitals need not be independent nor negatively correlated.
Instead, we modify the double-cut DA to lower bound the number of unmatched hospitals in a suitably sized interval $I$ of hospitals (the interval is given by public ratings). In this modification, we no longer use the full set of doctors in a range $[r(h)-a\alpha,1)$ as before, but a subset of these doctors chosen to ensure that the possible runs of the double-cut DA are close to uniform w.r.t.\ the hospitals in $I$. For then it turns out that the match/non-match probabilities for the hospitals in $I$ become negatively correlated, allowing us to apply a Chernoff bound.

We will also need to analyze an analogous double-cut DA for intervals of doctors. This is not completely symmetric for the hospitals can only make proposals on the edges the doctors selected, and different hospitals in general have differing numbers of available proposals.

The runs of the double-cut DA described in the previous two paragraphs are used to bound the number of unmatched hospitals and doctors. These bounds are used inductively. They are also used in the analysis of runs of the original double-cut DAs; these runs are used to lower bound the quality of the matches achieved by individual doctors and hospitals. The quality bounds in turn are used in the $\eps$-Nash analysis.

A further generalization provides each hospital a capacity $\kappa>1$. For simplicity, we suppose all hospitals have the same capacity, so there are now $n$ doctors and $n/\kappa$ hospitals. As $\kappa$ increases, the probability that a hospital is fully matched increases. Indeed, when $\kappa=\Omega(\ln n)$, all but the bottommost hospitals will be fully matched with failure probability at most $n^{-c}$.

In general, we can describe the double-cut DA as follows. Some collection $\cd$ of proposers (WLOG doctors) all use an initial portion of their preference lists in a run of doctor-proposing DA to propose to a collection $\ch$ of hospitals (these are the destinations of the edges in the above truncated preference lists). Suppose it produces an outcome $\mathcal O$ for the hospitals in $\ch$.

Now suppose we use a larger set of edges in a new run of doctor-proposing DA, which includes all the edges in the previous run. The new edges need not be consecutive in their preference lists and can also come from doctors outside $\cd$. Let ${\mathcal O}'$ be the new outcome.
The following claim is immediate.

\begin{claim}\label{clm::double-cutDA-provides-bounds}
    For every hospital in $\ch$, the outcome in ${\mathcal O}'$ is at least as good as the outcome in ${\mathcal O}$. An analogous claim applies to runs of the hospital-proposing DA. 
\end{claim}
\begin{proof}
    In the doctor-proposing DA, as more proposals are made, the outcome for the receiving hospitals only improves. And because the first run uses initial portions of the preference lists for the doctors in $\cd$, in the second run, these edges, for each preference list, are all proposed before any new edges. Therefore, outcome ${\mathcal O}$ can be achieved before any of the new edges are used, and hence using these new edges can only improve the outcome beyond ${\mathcal O}$.
\end{proof}

This immediately implies that the outcome for the hospitals in the full run of the doctor-proposing DA is at least as good as the outcome in the double-cut run, which is why the bounds in the double-cut run are useful.


==> double-cutDA.tex <==
\section{Overview of the Double Cut DA}\label{sec::double-cutDA}

This methodology was introduced in \cite{AC23} to bound the number of proposals needed to obtain a stable matching with high probability, meaning probability $1-n^{-c}$, for any constant $c$ (the bound on the number of proposals increases as $O(\sqrt{c})$).

\input{double-cut-figure}

% There are two sets of agents, doctors and hospitals.
Suppose we want to show that a hospital $h$ receives a high-quality proposal with high probability.
% To keep the overview simple, let's suppose there are $n$ doctors and $n$ hospitals.
Our overview uses the setting from \cite{AC23}. There the doctors and hospitals obtain their utilities for potential partners by adding a private value for that partner to the partner's public rating, where values and ratings are uniform random draws from $[0,1)$. 
% \footnote{A natural way of obtaining such a number is by repeated sampling of a 0/1 choice, stopping when the number is unique; this will always be in the range $[0,1)$.}

To demonstrate the quality of $h$'s match, if any, we analyze a partial run of the doctor-proposing DA.
The participants are the hospitals with public rating in the range $[r(h)-\alpha,1)$ and the doctors with public rating in the range $[r(h)-a\alpha,1)$, where $a>1$ and $\alpha$ are suitable parameters.
Our choice of $\alpha$ will ensure that with high probability there are at least $\alpha n$ more doctors than hospitals participating.

The run of the doctor-proposing DA is further restricted as follows. Each doctor in $h$'s cone, i.e.\ with public rating in $[r(h)-a\alpha,r(h)+a\alpha)$, stops making proposals as soon as she reaches a proposal providing her utility less than $r(h)+1-\alpha$ (she does not make this proposal). This means that she will not make any proposals to hospitals with public rating less than $r(h)-\alpha$.
She also stops if she is about to make a proposal to $h$; this will then be her final proposal, so long as it provides utility at least $r(h)+1-\alpha$. The doctors above $h$'s cone are unconstrained. Agarwal and Cole called this the double-cut DA for $h$.

In order to obtain useful bounds on the quality of $h$'s match one needs to show the following three bounds.
\begin{enumerate}
    \item There is a sufficiently larger surplus $s$ of doctors who could propose to $h$ (depending on their random choice of private value) and they either propose to $h$ or remain unmatched. 
    \item If each of the $s$ surplus doctors $d$ were to propose independently to $h$ with probability $\alpha$ (i.e.\ $d$ has a private value for $h$ providing her utility at least $r(h)+1-\alpha$), then $h$ would receive a high-quality match with the desired probability. %(Note that this is not what actually happens.)
    \item Inconveniently, the actions of the surplus doctors need not be independent. The final step is to show that the case of independent proposals yields a failure probability that is at least as large as the failure probability for the actual run of the double-cut DA. This argument was carried out by a methodology we name \emph{tree stochastic dominance}.\footnote{This name is being coined in this paper.}
\end{enumerate}


An important property of the double-cut DA is that the outcome for $h$ in the full run of the doctor-proposing DA is at least as good as its outcome in the double-cut DA (see \Cref{clm::double-cutDA-provides-bounds} below).
The full analysis uses analogous runs of a double-cut DA for doctors.
An immediate implication of this analysis is that with high probability, for each doctor $d$, her possible matches have public ratings in the cone $C(d)=[r(d)-a\alpha,r(d)+a\alpha)$, and similarly for the hospitals.

In the current work, we need to substantially modify Steps 1 and 3 above to achieve our new results.

In \cite{AC23}, Step 1 depended on every agent ending up matched with high probability (except for some of the bottommost agents, meaning those with public rating less than $a\alpha$).
Then the surplus is simply the number of participating doctors minus the number of participating hospitals, and with high probability these numbers are close to their expected value, as shown by Chernoff bounds. On setting $a=3$, they obtain a surplus of size at least $\alpha n$.

In the current work, as we are limiting each doctor to making $k$ proposals, we no longer have a polynomially small probability of failing to match. In fact, we expect at least an $e^{-\Theta(k)}$ fraction of the doctors to fail to match. In computing the surplus, we will need to subtract the number of unmatched doctors whose public rating lies above $h$'s cone. As it turns out, we will need a high-probability bound on this number, and on the analogous numbers for the not-fully matched hospitals.
The difficulty is that while we can obtain an upper bound on the probability that a single hospital (or doctor) is unmatched, and hence an upper bound on the expected number of unmatched hospitals, we cannot apply a Chernoff bound, as the probabilities for the various hospitals need not be independent nor negatively correlated.
Instead, we modify the double-cut DA to lower bound the number of unmatched hospitals in a suitably sized interval $I$ of hospitals (the interval is given by public ratings). In this modification, we no longer use the full set of doctors in a range $[r(h)-a\alpha,1)$ as before, but a subset of these doctors chosen to ensure that the possible runs of the double-cut DA are close to uniform w.r.t.\ the hospitals in $I$. For then the match/non-match probabilities for the hospitals in $I$ become negatively correlated, allowing us to apply a Chernoff bound.

We will also need to analyze an analogous double-cut DA for intervals of doctors. This is not completely symmetric for the hospitals can only make proposals on the edges the doctors selected, and different hospitals in general have differing numbers of available proposals.

The runs of the double-cut DA described in the previous two paragraphs are used to bound the number of unmatched hospitals and doctors. These bounds are used inductively. They are also used in the analysis of runs of the original double-cut DAs; these runs are used to lower bound the quality of the matches achieved by individual doctors and hospitals. The quality bounds in turn are used in the $\eps$-Nash analysis.

A further generalization provides each hospital a capacity $\kappa>1$. For simplicity, we suppose all hospitals have the same capacity, so there are now $n$ doctors and $n/\kappa$ hospitals. As $\kappa$ increases, the probability that a hospital is fully matched increases. Indeed, when $\kappa=\Omega(\ln n)$, all but the bottommost hospitals will be fully matched with failure probability at most $n^{-c}$.

In general, we can describe the double-cut DA as follows. Some collection $\cd$ of proposers (WLOG doctors) all use an initial portion of their preference lists in a run of doctor-proposing DA to propose to a collection $\ch$ of hospitals (these are the destinations of the edges in the above truncated preference lists). Suppose it produces an outcome $\mathcal O$ for the hospitals in $\ch$.

Now suppose we use a larger set of edges in a new run of doctor-proposing DA, which includes all the edges in the previous run. The new edges need not be consecutive in their preference lists and can also come from doctors outside $\cd$. Let ${\mathcal O}'$ be the new outcome.
The following claim is immediate.

\begin{claim}\label{clm::double-cutDA-provides-bounds}
    For every hospital in $\ch$, the outcome in ${\mathcal O}'$ is at least as good as the outcome in ${\mathcal O}$. An analogous claim applies to runs of the hospital-proposing DA. 
\end{claim}
\begin{proof}
    In the doctor-proposing DA, as more proposals are made, the outcome for the receiving hospitals only improves. And because the first run uses initial portions of the preference lists for the doctors in $\cd$, in the second run, these edges, for each preference list, are all proposed before any new edges. Therefore, outcome ${\mathcal O}$ can be achieved before any of the new edges are used, and hence using these new edges can only improve the outcome beyond ${\mathcal O}$.
\end{proof}

This immediately implies that the outcome for the hospitals in the full run of the doctor-proposing DA is at least as good as the outcome in the double-cut run.


==> extensions-ver2.tex <==


\section{Extensions}\label{sec::extensions}

\subsection{Unequal Numbers of Doctors and Hospital Places}

In practice, it is likely that these two numbers will differ somewhat. Indeed, in the NRMP data
for 2024 \cite{NRMP24}, there were roughly 40,000 positions and 50,000 applicants (including those from foreign medical schools). Our results are essentially unchanged. All that happens is that if we align
the doctors and hospitals by public rating order, then the results for  the non-bottommost agents
continue to hold as before, but it is possible for this group to include all the agents on the short side.
To make this precise, suppose there are $n+m$ doctors and $n$ positions, with public rating
 ranges $[0,1+\frac mn)$ and $[\frac nm,1+\frac nm)$ (we can always shift the range; it is defined this way for convenience).
 Then, for the doctors, the bottommost agents are those with public rating in the interval
 $[0,a\alpha+\frac nm)$, and for the hospitals, it is $[\frac nm, \max\{a\alpha,\frac nm\})$;
 note that if $\frac nm\ge a\alpha$, there are no bottommost hospitals.
 If there are more hospitals than doctors, the definition is reversed.
 This is in contrast with the outcome in random markets \cite{AKL17} where all agents on the short side benefit substantially.

\subsection{Reducing the Weight of the Interview Values}

In our main analysis, the interview values largely determine the preference orderings,
though not completely; there is still a modest bias in favor of higher public ratings.
What happens if we reduce the weight of the interview values?
By this we mean that a doctor $d$ will obtain utility $r(h)+v(d,h)+\nu_d\cdot\iota(d,h)$ for hospital $h$,
where $0\le \nu_d<1$ is a parameter, and similarly a hospital $h$ obtains utility $r(d)+\nu_h\cdot \iota(h,d)$ for doctor $d$, where $0\le \nu_h<1$ is another parameter.

We obtain improved bounds in Claims \ref{lem::fail-prob-hospital-prop} and \ref{lem::fail-prob-doctor-prop}, which concern the non-match probability for doctors, and the not-fully matched probability for hospitals, resp.
We also obtain better bounds in Claims \ref{qtilde-bound-at-root-hosp-to-doc-int} and \ref{qtilde-bound-at-root-doc-to-hosp-int}; they concern, respectively, the collective mismatch rate for doctors and hospitals in an interval $I$.
This allows us to reduce the value of $\alpha$
for the $\eps$-Nash analysis in \Cref{lem::typical-student-eps-nash}, leading to smaller values of $\epsilon$. 
We begin by showing the improvement to the bound in \Cref{lem::fail-prob-hospital-prop}.

\begin{claim}\label{lem::fail-prob-hospital-prop-ext}
    Let $d$ be a doctor with public rating at least $a\alpha$.
    Suppose $s\ge \frac{\alpha n}{\kappa}$ and that
    there are at most $\frac12(4a+1)\frac{\alpha n}{\kappa}$ hospitals in $C(d)$. Then the probability that $d$ receives no proposal for which $d$ has interview value at least $1-\psibar_d$ is at most $\exp\big(-k\beta_h\psibar_d/(4a+1)\big)$, where $\beta_h = \min\{1, \frac{\alpha}{\nu_h}\}$.
\end{claim}
\begin{proof}
 The change to the proof of \Cref{lem::fail-prob-hospital-prop} is that now we only require the
 hospitals to have interview value at least $1- \beta_h$. The reason we use this bound is that
 the reduction to the hospital's utility when using this bound is at most $\alpha$, which is what
 is needed to ensure that all the proposals in the double-cut DA have utility above the cut point.
\end{proof}

Similarly, in \Cref{lem::hosp-high-value-match-prob}, the not-fully matched probability improves to
$\exp\big(-\frac{3\kappa k\beta_d\psibar_h}{2(4a+1)}\big)$, where $\beta_d=\min\{1,\frac{\alpha}{\nu_d}\}$. The bounds in Claims \ref{qtilde-bound-at-root-hosp-to-doc-int} and \ref{qtilde-bound-at-root-doc-to-hosp-int} improve to at most $3|I|\exp\big(-\frac{\beta_h k}{2(4a+1)}\big)$ unmatched doctors,
and at most $3|I|\exp\big(-\frac{\beta_d k}{2(4a+1)}\big)$ unmatched hospitals.

Next, we state the resulting improvements to the $\eps$-Nash result. Basically, $\alpha$ can shrink almost linearly in $(\nu_h\nu_d)^{1/2}$ (offset by a logarithmic factor) until it reaches a minimum value $\alpha_{\min}$, and $\eps=O(\alpha)$.

\begin{theorem}\label{clm::improved-eps}
% Let $\alpha_l = \big(\frac{8b(c+2)\kappa}{2a-1}\big)^{1/2}\cdot \big(\frac{\ln n}{n}\big)^{1/2}$, the minimum allowed value for $\alpha$, and let $\alphabar=\big(\frac{4(4a+1)\ln k}{k}\big)^{1/2}$, the value of $\alpha$ when $\nu_d=\nu_h=1$.
Suppose that the hospitals list the doctors they interview in preference order and all but the bottommost $a\alpha$ doctors follow the recommended strategy.
Then, all but the bottommost $a\alpha$ doctors achieve an $\eps$-Nash equilibrium,
with the following bounds, depending on the values of $\nu_d$ and $\nu_h$.
Let $\alpha_{\min}= 3\exp\big(-\frac{k}{2(4a+1)}\big)$.


Case 1: $\alpha_{\min}\le \alpha\le \nu_h\le \nu_d\le 1$. \\
Let $\sigma=\min\big\{1,\frac{3\kappa}{8}\big\}$.
With our choice for $\alpha$ given shortly, this amounts to 
$\nu_h\ge \frac {v_d(4a+1)}{k\sigma} \ln \Big(\frac{ek\sigma}{\nu_h\nu_d(4a+1)}\Big)^{1/2}$.
Let $x=\frac{\nu_h\nu_d(4a+1)}{k\sigma}$; then we set $\alpha = x^{1/2}\cdot\big[\ln (ex)^{1/2} \big]$.
Then $\eps= O(\alpha)$,
and the mismatch/not-fully matched rates for the doctors and hospitals are
$\exp\big(-\frac{\alpha k}{(4a+1)\nu_h}\big)$
and $\exp\big(-\frac{3\kappa k\alpha}{8(4a+1)\nu_d}\big)$, respectively.

Case 2: $\max\{\alpha_{\min},\nu_h\} < \alpha\le \nu_d\le 1$.\\
Then $\eps= O(\alpha)$, with
$\alpha \ge \frac{2(4a+1)\nu d}{k}\cdot \ln\big(\frac{3ek}{4(4a+1)\nu d}\big)$ and $3k\ge 4(4a+1)\nu_d$;
the mismatch/not-fully matched rates for the doctors and hospitals are
$\exp\big(-\frac{k}{4a+1}\big)$ and $\exp\big(-\frac{3\kappa k\alpha}{8(4a+1)\nu_d}\big)$.

Case 3: $\nu_h\le \nu_d\le 3\alpha$.\\
We set $\alpha = \alpha_{\min}$.
Then $\eps= O(\alpha_{\min})$ and
the mismatch/not-fully matched rates for the doctors and hospitals are
$\exp(-k/4(4a+1))=\frac 13\alpha_{\min}$ and $\exp\big(-\frac{3\kappa k}{8(4a+1)}\big)$.
\end{theorem}


\hide{
\rnote{Other things to consider: some uncertainty about one's public rating.
I think all one needs to do is to expand the cone to cover the uncertainty, but I am not totally clear as to the effect on the bounds.}
}


==> extensions.tex <==

\section{Extensions}\label{sec::extensions}

\subsection{Unequal Numbers of Doctors and Hospital Places}

In practice, it is likely that these two numbers will differ somewhat. Indeed, in the NRMP data
for 2024 \cite{NRMP24}, there were roughly 40,000 positions and 50,000 applicants (including those from foreign medical schools). Our results are essentially unchanged. All that happens is that if we align
the doctors and hospitals by public rating order, then the results for  the non-bottommost agents
continue to hold as before, but it is possible for this group to include all the agents on the short side.
To make this precise, suppose there are $n+m$ doctors and $n$ positions, with public rating
 ranges $[0,1+\frac mn)$ and $[\frac nm,1+\frac nm)$ (we can always shift the range; it is defined this way for convenience).
 Then, for the doctors, the bottommost agents are those with public rating in the interval
 $[0,a\alpha+\frac nm)$, and for the hospitals, it is $[\frac nm, \max\{a\alpha,\frac nm\})$;
 note that if $\frac nm\ge a\alpha$, there are no bottommost hospitals.
 If there are more hospitals than doctors, the definition is reversed.
 This is in contrast with the outcome in random markets \cite{AKL17} where all agents on the short side benefit substantially.

 

 \subsection{Reducing the Weight of the Interview Values}

In our main analysis, the interview values largely determine the preference orderings,
though not completely; there is still a modest bias in favor of higher public ratings.
What happens if we reduce the weight of the interview values?
By this we mean that a doctor $d$ will obtain utility $r(h)+v(d,h)+\nu_d\cdot\iota(d,h)$ for hospital $h$,
where $0\le \nu_d<1$ is a parameter, and similarly a hospital $h$ obtains utility $r(d)+\nu_h\cdot \iota(h,d)$ for doctor $d$, where $0\le \nu_h<1$ is another parameter.

We obtain improved bounds in Claims \ref{lem::fail-prob-hospital-prop} and \ref{lem::fail-prob-doctor-prop}, which concern the non-match probability for doctors, and the not-fully matched probability for hospitals, resp.
We also obtain better bounds in Claims \ref{qtilde-bound-at-root-hosp-to-doc-int} and \ref{qtilde-bound-at-root-doc-to-hosp-int}; they concern, respectively, the collective mismatch rate for doctors and hospitals in an interval $I$.
This allows us to reduce the value of $\alpha$
for the $\eps$-Nash analysis in \Cref{lem::typical-student-eps-nash}, leading to smaller values of $\epsilon$. 
We begin by showing the improvement to the bound in \Cref{lem::fail-prob-hospital-prop}.



\begin{claim}\label{lem::fail-prob-hospital-prop-ext}
    Let $d$ be a doctor with public rating at least $a\alpha$.
    Suppose $s\ge \frac{\alpha n}{\kappa}$ and that
    there are at most $\frac12(4a+1)\frac{\alpha n}{\kappa}$ hospitals in $C(d)$. Then the probability that $d$ receives no proposal for which $d$ has interview value at least $1-\psibar_d$ is at most $\exp\big(-k\beta_h\psibar_d/(4a+1)\big)$, where $\beta_h = \min\{1, \frac{\alpha}{\nu_h}\}$.
\end{claim}
\begin{proof}
 The change to the proof of \Cref{lem::fail-prob-hospital-prop} is that now we only require the
 hospitals to have interview value at least $1- \beta_h$. The reason we use this bound is that
 the reduction to the hospital's utility when using this bound is at most $\alpha$, which is what
 is needed to ensure that all the proposals in the double-cut DA have utility above the cut point.
\end{proof}

Similarly, in \Cref{lem::hosp-high-value-match-prob}, the not-fully matched probability improves to
$\exp\big(-\frac{3\kappa k\beta_d\psibar_h}{8(4a+1)}\big)$, where $\beta_d=\min\{1,\frac{\alpha}{\nu_d}\}$. The bounds in Claims \ref{qtilde-bound-at-root-hosp-to-doc-int} and \ref{qtilde-bound-at-root-doc-to-hosp-int} improve to at most $3|I|\exp\big(-\frac{\beta_h k}{4(4a+1)}\big)$ unmatched doctors,
and at most $3|I|\exp\big(-\frac{\beta_d k}{4(4a+1)}\big)$ unmatched hospitals.

Next, we state the resulting improvements to the $\eps$-Nash result. Basically, $\alpha$ can shrink almost linearly in $(\nu_h\nu_d)^{1/2}$ (offset by a logarithmic factor) until it reaches a minimum value $\alpha_{\min}$, and $\eps=O(\alpha)$.

\begin{theorem}\label{clm::improved-eps}
% Let $\alpha_l = \big(\frac{8b(c+2)\kappa}{2a-1}\big)^{1/2}\cdot \big(\frac{\ln n}{n}\big)^{1/2}$, the minimum allowed value for $\alpha$, and let $\alphabar=\big(\frac{4(4a+1)\ln k}{k}\big)^{1/2}$, the value of $\alpha$ when $\nu_d=\nu_h=1$.
Suppose that the hospitals list the doctors they interview in preference order and all but the bottommost $a\alpha$ doctors follow the recommended strategy.
Then, all but the bottommost $a\alpha$ doctors achieve an $\eps$-Nash equilibrium,
with the following bounds, depending on the values of $\nu_d$ and $\nu_h$.
Let $\alpha_{\min}= 3\exp\big(-\frac{k}{4(4a+1)}\big)$.


Case 1: $\alpha_{\min}\le \alpha\le \nu_h\le \nu_d\le 1$. \\
Let $\sigma=\min\big\{1,\frac{3\kappa}{8}\big\}$.
With our choice for $\alpha$ given shortly, this amounts to 
$\nu_h\ge \frac {v_d(4a+1)}{k\sigma} \ln \frac{ek\sigma}{\nu_h\nu_d(4a+1)}$.
Let $x=\frac{\nu_h\nu_d(4a+1)}{k\sigma}$; then we set $\alpha = x^{1/2}\cdot\big[\ln (ex)^{1/2} \big]$.
Then $\eps= O(\alpha)$,
and the mismatch/not-fully matched rates for the doctors and hospitals are
$\exp\big(-\frac{\alpha k}{(4a+1)\nu_h}\big)$
and $\exp\big(-\frac{3\kappa k\alpha}{8(4a+1)\nu_d}\big)$, respectively.

Case 2: $\max\{\alpha_{\min},\nu_h\} < \alpha\le \nu_d\le 1$.\\
Then $\eps= O(\alpha)$, with
$\alpha \ge \frac{4(4a+1)\nu d}{k}\cdot \ln\big(\frac{3ek}{4(4a+1)\nu d}\big)$ and $3k\ge 4(4a+1)\nu_d$;
the mismatch/not-fully matched rates for the doctors and hospitals are
$\exp\big(-\frac{k}{4a+1}\big)$ and $\exp\big(-\frac{3\kappa k\alpha}{8(4a+1)\nu_d}\big)$.

Case 3: $\nu_h\le \nu_d\le 3\alpha$.\\
We set $\alpha = \alpha_{\min}$.
Then $\eps= O(\alpha_{\min})$ and
the mismatch/not-fully matched rates for the doctors and hospitals are
$\exp(-k/4(4a+1))=\frac 13\alpha_{\min}$ and $\exp\big(-\frac{\kappa k}{8(4a+1)}\big)$.
\end{theorem}


\hide{
\rnote{Other things to consider: some uncertainty about one's public rating.
I think all one needs to do is to expand the cone to cover the uncertainty, but I am not totally clear as to the effect on the bounds.}
}


==> intro-ver2.tex <==

\section{Introduction}\label{sec::intro}

Consider a doctor applying for residency positions.
Which programs should she apply to? The very top ones?
Or those where she has a reasonable chance of admission (if these are not the same)?
And if the latter, how does she identify them?
We study this issue in settings where Gale and Shapley's deferred acceptance (DA) algorithm~\cite{GS62} is being used to match applicants to positions.
It is well-known that in DA the optimal strategy for the proposing side is to list their choices in order of preference. However, this does not indicate which choices one should list.

Consider the US residency match, which matches prospective residents to positions in hospital programs, which we refer to as hospitals henceforth. The most well-known part of this process is the National Residency Matching Program (NRMP), which runs the doctor-proposing DA to compute the matching (modulo a few details, such as allowing couples to submit joint preferences). Before this happens, both sides determine their preferences as follows. First, doctors apply to hospitals for interviews. Hospitals grant some of the requested interviews. Following the interviews, hospitals and doctors create their preference lists. It is well understood that if there is no interview a hospital will not list the doctor, so the only hospitals worth listing are those at which an interview occurs.

As time is limited, doctors and hospitals can afford only a relatively small number of interviews compared to the size of the pool, as least for larger fields such as pediatrics. Were doctors to all seek interviews at their favorite hospitals, given that preferences are likely to be correlated, this would result in many programs having too few applications, leading to a poor match rate. Clearly, doctors should apply to places where they have some reasonable chance of receiving a position. Indeed, the advice from the NRMP is that doctors should be ``realistic''. But can we make this more precise?

Let's also consider school choice programs in large school districts such as the one in New York City, where the matching is computed using the DA algorithm. This setting differs in that the schools preferences are largely public or random: they depend on a variety of factors, depending on the school, such as gpa, living in a designated zone, and random selection if needed. Similarly, university entrance in many countries is based solely on students performance in a national exam, e.g.\ the gaokao in China or the Joint Entrance Examination in India. In all these settings, students need to decide which schools to list.
% We can think of this as being informed by an information gathering phase, even if in reality this is largely based on word-of-mouth. 
Here too, students are well-advised to be realistic.

To model these settings, we use a model proposed by Allman and Ashlagi~\cite{AA23}, which extends a model introduced by Lee~\cite{Lee16}.

To keep the analysis tractable, we simplify the residency match setting and suppose that each doctor requests exactly $k$ interviews, and the hospitals grant all the requested interviews. Later in the paper, we comment on why we believe it may be feasible to extend our analysis to the more general setting.
Similarly, for the school choice setting, we suppose that each student gathers information to inform their choices (which we will call interviewing) at exactly $k$ schools.

In the residency setting, both sides create preference lists for the agents they interviewed and no others. In the school choice setting, students only list schools at which they interviewed; schools list all students. The doctor-proposing or student-proposing DA algorithm is then run using these preference lists as its input.
%
Another salient aspect of both these settings is that the hospitals and schools each have multiple positions, which for simplicity we assume is the same size $\kappa$ for all programs.

We obtain the following results.
In our utility-based model of preferences, 
\begin{itemize}
\item  
The probability of failing to match is $e^{-\widetilde{\Theta}(\sqrt{k})}$  in the residency setting and $e^{-\widetilde{\Theta}(k)}$ in the school-choice setting,\footnote{The $\widetilde{O}$ notation suppresses logarithmic terms.} apart possibly for a small bottommost tier of agents. 
\item We obtain bounds on the expected utilities the agents achieve.
\item 
In the school choice setting, this yields an $\epsilon$-Nash style equilibrium: for all but the bottommost $O(\eps)$ students, if the students follow the recommended strategy, deviation yields at most an expected $\epsilon=O(\ln k/k)$ improvement in utility, and this bound is unaffected by the actions of the bottommost students. Note that, by definition, in this setting the schools are non-strategic.
\item 
In the residency setting, if we assume the hospitals are non-strategic, again there is an $\eps$-Nash style equilibrium; here, a bound of $\eps=O(\sqrt{\ln k/k})$ applies to the non-bottommost doctors, and this is unaffected by the actions of the bottommost doctors.
\end{itemize}
Loosely speaking, these results are achieved if applicants (students or doctors) spread their proposals around their assortative match.

\subsection{Related Work}

Knuth \cite{Kn76,Kn96} initiated the analysis of randomized preference lists, considering lists that were uniform random permutations. Pittel provided definitive analyses of this setting~\cite{Pit89,Pit92}. Immorlica and Madhian~\cite{IM15} introduced a generalization of this model, which they called the \emph{popularity model};  it enables certain correlations among different agents' preferences.
In their model, the first side---men---can have arbitrary preferences; on the second side---women---preferences are selected by weighted random choices, the weights representing the ``popularity'' of the different choices. These results were further extended by Kojima and Parthak
in~\cite{KP09}.

The popularity model does not capture behavior in settings 
where bounds on the number of proposals lead to proposals
being made to plausible partners, i.e.\ partners with
whom one has a realistic chance of matching.
One way to capture such settings is by way of tiers~\cite{ABKS19},
also known as block correlation~\cite{CKN13}:
agents on each side are partitioned into tiers, with all agents in a higher tier preferred to agents in a lower tier, and with uniformly random preferences within a tier. Tiers on the two sides may have different sizes.
If we assign tiers successive intervals of ranks equal to their size,
then, in any stable matching, the only matches will be between agents in tiers whose rank intervals overlap.

A more nuanced way of achieving these types of preferences 
bases agent preferences on cardinal utilities; for each side, these utilities are functions of an underlying common assessment of the other side, together with idiosyncratic individual adjustments for the agents on the other side.
These include the separable utilities defined by Ashlagi, Braverman, Kanoria and Shi~\cite{ABKS19},
and another class of utilities
introduced by Lee~\cite{Lee16}. This last model will be the focus of our study. 

% In Lee's model, utilities are a function of a common or public assessment and idiosynchratic individual assessments. 
To make this more concrete, we review a simple special case of Lee's model, the \emph{linear
separable model}. Suppose that there are $n$ doctors and $n$ hospitals seeking to match with each other.
Each doctor $d$ has a public rating $r(d)$, a uniform random draw from $[0,1)$ \footnote{A natural way of obtaining such a number is by repeated sampling of a 0/1 choice, stopping when the resulting number, viewed as being of the form $0.***\cdots$, is sufficiently precise; this will always be in the range $[0,1)$.}. These ratings can be viewed
as the hospitals' joint common assessment of the doctors. In addition, each doctor $d$ has an individual adjustment $v(d,h)$  for each hospital $h$, which we call a private value;
again, this is a uniform random draw from $[0,1)$. All the draws are independent. Doctor $d$'s utility for hospital $h$ is given
by $r(h) + v(d,h)$; her full preference list has the hospitals in decreasing utility order. The hospital utilities are defined similarly: $h$ has utility $r(d)+v(h,d)$ for doctor $d$, where $v(h,d)$ is her private value for $d$, also a uniform random draw from $[0,1)$.

Lee showed that for $\eps>0$, for large enough $n$, with failure probability at most $\eps$, all but an $\eps$ fraction of the pairings in a matching would provide the doctor $d$ utility of at least $r(d)+1-\eps$ and hospital $h$ utility of at least $r(h)+1-\eps$. We call $r(d)+1$ doctor $d$'s benchmark and $r(h)+1$ hospital $h$'s benchmark. Informally speaking, most agents achieve utility which is at least their benchmark minus $\eps$. Lee showed $\eps$ could be as small as $O(n^{-1/4})$. The main technical tool in his work was results about the maximum size of bi-cliques in random bipartite graphs.

Later, Agarwal and Cole~\cite{AC23} reanalyzed this setting using a different methodology which analyzed the DA algorithm itself. They showed that, for any constant $c>0$, with failure probability at most $n^{-c}$, the only agents that failed to achieve their benchmark minus $\eps=\widetilde{O}(n^{-1/3})$ were thosewith public rating at most $\widetilde{O}(n^{-1/3})$. \footnote{The tight log term they obtained was $\ln^{2/3}n$.}
Their main technical tool was to use truncated runs of DA, which they called the double-cut DA, and a specialized stochastic dominance argument. In this work, we generalize these tools, which enables us to analyze the interview setting.

The first analysis of the interview process in Lee's model was by Echenique et al.~\cite{EGWY22}.
They supposed the interview pairs were determined by an initial computation that determined a $k$--$k'$ stable match (meaning that doctors obtained up to $k$ matches and hospitals up to $k'$ matches; setting $k'=\kappa k$ corresponds to each hospital having capacity $\kappa$). They then ran the doctor-proposing DA on these edges using the same utilities; i.e.\ there was no post-interview alteration of the utilities. The goal of the work was to see if one could explain why doctors mostly seem to obtain their declared first or second preference matches in the NRMP matching. By means of extensive simulations, they showed that with $k=k'=5$, match rates and doctor outcomes similar to the NRMP happened. 
% They also proved a theoretical bound.
%, but its conclusions were not as clear-cut as the simulations.

Allman and Ashlagi~\cite{AA23} extended Lee's model by adding a third component to the utilities, the interview value, again a random draw from $[0,1)$. In this model, interviews were determined based on the utility given by the first two components. Then, following the interview, the interview values were added to the utilities, and these new utilities were used to provide preferences over the interviewed partners. We adopt this model in our paper.
Unfortunately, the proofs in Ashlagi et al.\ turned out to be incorrect. These were based on the random graph approach used by Lee. In contrast, our results extend the techniques introduced in \cite{AC23}.

In other recent work, Ashlagi et al.\ \cite{ACRS25} have sought to guarantee matches in the presence of interviews;
in tiered markets a bound of $O(\log^3 n)$ interviews is achieved, in contrast to the $O(1)$ interviews that is our focus.

The impact of short lists on the quality of matches has been studied previously \cite{Arnosti15,KMQ21}; we touch on this issue at the end of the paper.

The engineering of admissions systems for universities and schools has received considerable attention \cite{APR05,APR09,BCCKP19,CEEetal19,RLPC21}, which partly motivates our analysis of this case.

Another line of work seeks to evaluate the use of signaling in stable matching settings \cite{ABKS19,AASY25}.

\paragraph{Roadmap}
In \Cref{sec::model} we define our model and then in \Cref{sec::results} we state our main results.
In \Cref{sec::double-cutDA} we review the double-cut DA, a class of truncated runs of the DA algorithm, which was introduced in \cite{AC23} and is generalized in the current work.
In \Cref{sec::proof-idio-thm} we outline the analysis of the residency setting, and then 
in \Cref{sec::student-school} we briefly explain how the analysis changes for the school choice setting.
In \Cref{sec::extensions}, we explain how our results extend to unequal sized sides (e.g.\ more doctors than hospitals) and discuss how to support generalizations of the utility functions; then, in
\Cref{sec::open-prob} we indicate why the analysis might be extended to the full interview setting as mentioned above and mention an unresolved issue. Next, in \Cref{experiments}, we complement our theoretical results with some experimental results, which indicate that the conclusions from our asymptotic bounds hold for real-world values of $n$, the number of agents. Finally, in \Cref{sec::conc}, we offer some concluding remarks. All omitted proofs can be found in the appendix. 

==> intro.tex <==

\section{Introduction}\label{sec::intro}

Consider a doctor applying for residency positions.
Which programs should she apply to? The very top ones?
Or those where she has a reasonable chance of admission (if these are not the same)?
And if the latter, how does she identify them?
We study this issue in settings where Gale and Shapley's deferred acceptance (DA) algorithm~\cite{GS62} is being used to match applicants to positions.
It is well-known that in DA the optimal strategy for the proposing side is to list their choices in order of preference. However, this does not indicate which choices one should list.

Consider the US residency match, which matches prospective residents to positions in hospital programs, which we refer to as hospitals henceforth. The most well-known part of this process is the National Residency Matching Program (NRMP), which runs the doctor-proposing DA to compute the matching (modulo a few details, such as allowing couples to submit joint preferences). Before this happens, both sides determine their preferences as follows. First, doctors apply to hospitals for interviews. Hospitals grant some of the requested interviews. Following the interviews, hospitals and doctors create their preference lists. It is well understood that if there is no interview a hospital will not list the doctor, so the only hospitals worth listing are those at which an interview occurs.

As time is limited, doctors and hospitals can afford only a relatively small number of interviews compared to the size of the pool, as least for larger fields such as pediatrics. Were doctors to all seek interviews at their favorite hospitals, given that preferences are likely to be correlated, this would result in many programs having too few applications, leading to a poor match rate. Clearly, doctors should apply to places where they have some reasonable chance of receiving a position. Indeed, the advice from the NRMP is that doctors should be ``realistic''. But can we make this more precise?

Let's also consider school choice programs in large school districts such as the one in New York City, where the matching is computed using the DA algorithm. This setting differs in that the schools preferences are largely public or random: they depend on a variety of factors, depending on the school, such as gpa, living in a designated zone, and random selection if needed. Similarly, university entrance in many countries is based solely on students performance in a national exam, e.g.\ the gaokao in China or the Joint Entrance Examination in India. In all these settings, students need to decide which schools to list.
% We can think of this as being informed by an information gathering phase, even if in reality this is largely based on word-of-mouth. 
Here too, students are well-advised to be realistic.

To model these settings, we use a model proposed by Allman and Ashlagi~\cite{AA23}, which extends a model introduced by Lee~\cite{Lee16}.

To keep the analysis tractable, we simplify the residency match setting and suppose that each doctor requests exactly $k$ interviews, and the hospitals grant all the requested interviews. Later in the paper, we comment on why we believe it may be feasible to extend our analysis to the more general setting.
Similarly, for the school choice setting, we suppose that each student gathers information to inform their choices (which we will call interviewing) at exactly $k$ schools.

In the residency setting, both sides create preference lists for the agents they interviewed and no others. In the school choice setting, students only list schools at which they interviewed; schools list all students. The doctor-proposing or student-proposing DA algorithm is then run using these preference lists as its input.
%
Another salient aspect of both these settings is that the hospitals and schools each have multiple positions, which for simplicity we assume is the same size $\kappa$ for all programs.

We obtain the following results.
In our utility-based model of preferences, 
\begin{itemize}
\item  
The probability of failing to match is $e^{-\widetilde{\Theta}(\sqrt{k})}$  in the residency setting and $e^{-\widetilde{\Theta}(k)}$ in the school-choice setting,\footnote{The $\widetilde{O}$ notation suppresses logarithmic terms.} apart possibly for a small bottommost tier of agents. 
\item We obtain bounds on the expected utilities the agents achieve.
\item 
In the school choice setting, this yields an $\epsilon$-Nash style equilibrium: for all but the bottommost $O(\eps)$ students, in expectation, if the students follow the recommended strategy, in expectation, deviation yields at most an $\epsilon=O(\ln k/k)$ improvement in utility, and this bound is unaffected by the actions of the bottommost students. Note that, by definition, in this setting the schools are non-strategic.
\item 
In the residency setting, if we assume the hospitals are non-strategic, again there is an $\eps$-Nash style equilibrium; here, a bound of $\eps=O(\sqrt{\ln k/k})$ applies to the non-bottommost doctors, and this is unaffected by the actions of the bottommost doctors.
\end{itemize}

\subsection{Related Work}

Knuth \cite{Kn76,Kn96} initiated the analysis of randomized preference lists, considering lists that were uniform random permutations. Pittel provided definitive analyses of this setting~\cite{Pit89,Pit92}. Immorlica and Madhian~\cite{IM15} introduced a generalization of this model, which they called the \emph{popularity model};  it enables certain correlations among different agents' preferences.
In their model, the first side---men---can have arbitrary preferences; on the second side---women---preferences are selected by weighted random choices, the weights representing the ``popularity'' of the different choices. These results were further extended by Kojima and Parthak
in~\cite{KP09}.

The popularity model does not capture behavior in settings 
where bounds on the number of proposals lead to proposals
being made to plausible partners, i.e.\ partners with
whom one has a realistic chance of matching.
One way to capture such settings is by way of tiers~\cite{ABKS19},
also known as block correlation~\cite{CKN13}:
agents on each side are partitioned into tiers, with all agents in a higher tier preferred to agents in a lower tier, and with uniformly random preferences within a tier. Tiers on the two sides may have different sizes.
If we assign tiers successive intervals of ranks equal to their size,
then, in any stable matching, the only matches will be between agents in tiers whose rank intervals overlap.

A more nuanced way of achieving these types of preferences 
bases agent preferences on cardinal utilities; for each side, these utilities are functions of an underlying common assessment of the other side, together with idiosyncratic individual adjustments for the agents on the other side.
These include the separable utilities defined by Ashlagi, Braverman, Kanoria and Shi~\cite{ABKS19},
and another class of utilities
introduced by Lee~\cite{Lee16}. This last model will be the focus of our study. 

% In Lee's model, utilities are a function of a common or public assessment and idiosynchratic individual assessments. 
To make this more concrete, we review a simple special case of Lee's model, the \emph{linear
separable model}. Suppose that there are $n$ doctors and $n$ hospitals seeking to match with each other.
Each doctor $d$ has a public rating $r(d)$, a uniform random draw from $[0,1)$ \footnote{A natural way of obtaining such a number is by repeated sampling of a 0/1 choice, stopping when the resulting number, viewed as being of the form $0.***\cdots$, is sufficiently precise; this will always be in the range $[0,1)$.}. These ratings can be viewed
as the hospitals' joint common assessment of the doctors. In addition, each doctor $d$ has an individual adjustment $v(d,h)$  for each hospital $h$, which we call a private value;
again, this is a uniform random draw from $[0,1)$. All the draws are independent. Doctor $d$'s utility for hospital $h$ is given
by $r(h) + v(d,h)$; her full preference list has the hospitals in decreasing utility order. The hospital utilities are defined similarly: $h$ has utility $r(d)+v(h,d)$ for doctor $d$, where $v(h,d)$ is her private value for $d$, also a uniform random draw from $[0,1)$.

Lee showed that for $\eps>0$, for large enough $n$, with failure probability at most $\eps$, all but an $\eps$ fraction of the matches would provide the doctor $d$ utility of at least $r(d)+1-\eps$ and hospital $h$ utility of at least $r(h)+1-\eps$. We call $r(d)+1$ doctor $d$'s benchmark and $r(h)+1$ hospital $h$'s benchmark. Informally speaking, most agents achieve utility which is at least their benchmark minus $\eps$. Lee showed $\eps$ could be as small as $O(n^{-1/4})$. The main technical tool in his work was results about the maximum size of bi-cliques in random bipartite graphs.

Later, Agarwal and Cole~\cite{AC23} reanalyzed this setting using a different methodology which analyzed the DA algorithm itself. They showed that, for any constant $c>0$, with failure probability at most $n^{-c}$, the only agents that failed to achieve their benchmark minus $\eps=\widetilde{O}(n^{-1/3})$ were thosewith public rating at most $\widetilde{O}(n^{-1/3})$. \footnote{The tight log term they obtained was $\ln^{2/3}n$.}
Their main technical tool was to use truncated runs of DA, which they called the double-cut DA, and a specialized stochastic dominance argument. In this work, we generalize these tools, which enables us to analyze the interview setting.

The first analysis of the interview process in Lee's model was by Echenique et al.~\cite{EGWY22}.
They supposed the interview pairs were determined by an initial computation that determined a $k$--$k'$ stable match (meaning that doctors obtained up to $k$ matches and hospitals up to $k'$ matches; setting $k'=\kappa k$ corresponds to each hospital having capacity $\kappa$). They then ran the doctor-proposing DA on these edges using the same utilities; i.e.\ there was no post-interview alteration of the utilities. The goal of the work was to see if one could explain why doctors mostly seem to obtain their declared first or second preference matches in the NRMP matching. By means of extensive simulations, they showed that with $k=k'=5$, match rates and doctor outcomes similar to the NRMP happened. 
% They also proved a theoretical bound.
%, but its conclusions were not as clear-cut as the simulations.

Allman and Ashlagi~\cite{AA23} extended Lee's model by adding a third component to the utilities, the interview value, again a random draw from $[0,1)$. In this model, interviews were determined based on the utility given by the first two components. Then, following the interview, the interview values were added to the utilities, and these new utilities were used to provide preferences over the interviewed partners. We adopt this model in our paper.
Unfortunately, the proofs in Ashlagi et al.\ turned out to be incorrect. These were based on the random graph approach used by Lee. In contrast, our results extend the techniques introduced in \cite{AC23}.

In other recent work, Ashlagi et al.\ \cite{ACRS25} have sought to guarantee matches in the presence of interviews;
in tiered markets a bound of $O(\log^3 n)$ interviews is achieved, in contrast to the $O(1)$ interviews that is our focus.

The impact of short lists on the quality of matches has been studied previously \cite{Arnosti15,KMQ21}; we touch on this issue at the end of the paper.

The engineering of admissions systems for universities and schools has received considerable attention \cite{APR05,APR09,BCCKP19,CEEetal19,RLPC21}, which partly motivates our analysis of this case.

Another line of work seeks to evaluate the use of signaling in stable matching settings \cite{ABKS19,AASY25}.

\paragraph{Roadmap}
In \Cref{sec::model} we define our model and then in \Cref{sec::results} we state our main results.
In \Cref{sec::double-cutDA} we review the double-cut DA, a class of truncated runs of the DA algorithm, which was introduced in \cite{AC23} and is generalized in the current work.
In \Cref{sec::proof-idio-thm} we outline the analysis of the residency setting, and then 
in \Cref{sec::student-school} we briefly explain how the analysis changes for the school choice setting.
In \Cref{sec::extensions}, we explain how our results extend to unequal sized sides (e.g.\ more doctors than hospitals) and discuss how to support generalizations of the utility functions; then, in
\Cref{sec::open-prob} we indicate why the analysis might be extended to the full interview setting as mentioned above and mention an unresolved issue. Next, in \Cref{experiments}, we complement our theoretical results with some experimental results, which indicate that the conclusions from our asymptotic bounds hold for real-world values of $n$, the number of agents. Finally, in \Cref{sec::conc}, we offer some concluding remarks. All omitted proofs can be found in the appendix. 

==> k-props-with-idio.tex <==

\section{The Doctor-Hospital Setting: Sketch of the Analysis}
\label{sec::proof-idio-thm}


To carry out the analysis we discretize the setting, and then to obtain a result for the continuous setting
we take the limit as the discretization tends to 0, similarly to \cite{AC23}.
% In this discretization, if a doctor (resp.\ hospital) has the same utility for two hospitals (resp.\ for two doctors), we do not run the double cut DA.

\begin{claim}
\label{clm::discrete-dist-idio}
For any $\delta>0$, there is a discrete utility space in which
the probability of having any differences
in the preference lists in the original continuous setting and in the discrete setting is at most $\delta$.
\end{claim}
\hide{
\begin{proof}
$z\ge n^3/\delta\kappa$ will be an integer in our construction.

We partition the utility range $[0,3]$ into $3z$ intervals each of length $1/z$.
To do this, we round down each utility to the nearest integer multiple of $1/z$.
Note that for each doctor $d$, the probability that it has the same utility for doctors
$d$ and $d'$ is at most $1/z$: to see this, consider selecting the random utility components
one by one, with the interview value for $d'$ being last; this last choice will create the
utility equality with probability at most $1/z$.
Therefore the probability that a doctor has the same utility for two hospitals is at most
$\tfrac 12 \frac{n}{\kappa}\cdot\big(\frac{n}{\kappa}-1\big)/z$, and so the probability that any doctor has the same utility for two hospitals is at most
$n\cdot \frac{n}{\kappa}\big(\frac{n}{\kappa}-1\big)/2z\le n^3/2z\kappa^2$.

Similarly, the probability that any hospital has the same utility for two doctors is at most
$n^3/2z\kappa$.

Therefore, the settings in which a doctor has the same utility for any pair of hospitals or a hospital has the same utility for any pair of doctors
occur with probability at most $n^3/z\kappa\le \delta$.
\end{proof}
}

We will be repeatedly referring to agents, be it a doctor $d$ or a hospital $h$, with public ratings in an interval $I$. For brevity, we will often write $d\in I$ (or $h\in I$) rather than $r(d)\in I$ (or $r(h)\in I$).

The proof of the theorem will use four different double-cut DAs;
their outcomes are specified in the next four lemmas.
In these lemmas we suppose that $\alpha$ and $g-f$ are chosen so that $\alpha$ is an integer multiple of $g-f$. Also, as the proof proceeds, we will identify some low probability events, \emph{bad events}, for short, collectively denoted by ${\mathcal B}$; collectively, they occur with probability at most
$1/n^c$, for any arbitrary constant $c>0$ (the bounds are a function of $c$ of course).

\begin{lemma}\label{lem::doctors-interval-non-match}
Let $\delta>0$ be an arbitrarily small constant.
Let $I=[f,g)$ be a public rating interval with $g\ge a\alpha$.
Suppose we run the (to be specified) hospital-proposing double-cut DA for interval $I$ using the discretized utilities
from \Cref{clm::discrete-dist-idio}.
Suppose the fraction of unmatched hospitals with public rating in $[g+(a+1)\alpha,1)$ is at most 
$3 \cdot\exp\big(-\alpha k/4(4a+1)\big)$.
Also suppose that event ${\mathcal B}$ does not occur.
Then, with failure probability at most $n^{-(c+2)}$,
the fraction of the doctors in $I$ who fail to match is less than $3\cdot \exp\big(-\frac{\alpha k}{4(4a+1)}\big)$,
if $n\ge2$, $a\ge 5$, $\alpha\cdot\exp\big(\frac{\alpha  k}{4(4a+1)}\big)\ge 3$, and the bounds on $g-f$ from \Cref{clm::hosp-prop-interval-constraints} hold.
\end{lemma}

A similar, but not identical, lemma (\Cref{lem::hospitals-interval-non-match}) for the doctor-proposing double cut DA for intervals $I$ of hospitals is deferred to the appendix.
Its proof is also different in some non-trivial ways.
\hide{
\begin{lemma}\label{lem::hospitals-interval-non-match}
Let $\delta>0$ be an arbitrarily small constant.
Let $I=[f,g)$ be a public rating interval with $g\ge a\alpha$.
Suppose we run the (to be specified) doctor-proposing double-cut DA for interval $I$ using the discretized utilities from in \Cref{clm::discrete-dist-idio}.
Suppose the fraction of unmatched doctors with public rating in $[g+(a+1)\alpha,1)$ is at most 
$3\cdot\exp\big(-\alpha k/4(4a+1)\big)$.
Also suppose that event ${\mathcal B}$ does not occur.
Then, with failure probability at most $n^{-(c+2)}$,
the fraction of the hospitals in $I$ that fail to match
is less than $3\cdot \exp\big(-\frac{\alpha\kappa k}{4(4a+1)}\big)$,
if $n\ge2$, $a\ge 5$, $\alpha\cdot\exp\big(\frac{\alpha k}{4(4a+1)}\big)\ge 3$, and the bounds on $g-f$ from \Cref{clm::doc-prop-interval-constraints} hold.
\end{lemma}
}

%The proof of \Cref{lem::hospitals-interval-non-match} is quite similar to the proof of \Cref{lem::doctors-interval-non-match}, with the roles of the doctors and hospitals being switched. It will be deferred to the appendix.

These two lemmas  are used in a mutual induction with the same value of $\delta$ to justify their assumptions on the numbers of unmatched hospitals and doctors, respectively. They also justify the assumption on the numbers of unmatched hospitals and doctors in the next two lemmas. 
% In order to use these bounds we need to know that the double-cut DA for an interval $I$ of doctors, is over doctors and hospitals with public rating in $[g-\alpha,1)$ and a subset of $[g-a\alpha,1]$, respectively, and similarly for the double-cut DA for an interval $I$ of hospitals.

\begin{lemma}\label{lem::doctors-high-value-match-prob}
Let $\delta>0$ be an arbitrarily small constant.
    Let $d$ be a doctor with public rating at least $a\alpha$.
    Suppose we run the hospital-proposing double-cut DA for doctor $d$ using the discretized utilities
from \Cref{clm::discrete-dist-idio}.
    Suppose the fraction of unmatched hospitals with public rating in $[r(d)+(a+1)\alpha,1)$ is at most $3\exp\big(-\alpha k/4(4a+1)\big)$.
    Also, suppose that event ${\mathcal B}$ does not occur.
    Finally, suppose we run the hospital-proposing double-cut DA for $d$.
     Then the probability that $d$ fails to receive a match for which it has interview value $1-\psibar_d$ or larger is at most $\exp\big(-\frac{k\alpha\psibar_d}{4a+1}\big)$, if both $a\ge 5$ and $\alpha\cdot\exp\big(\alpha k/4(4a+1)\big)\ge 3$.
\end{lemma}
We will use two values of $\psibar_d$: we set it to 1 to obtain the non-match probability, and to
$\alpha$ to obtain a bound on the expected utility which we use in the $\eps$-Nash analysis.

A similar lemma (\Cref{lem::hosp-high-value-match-prob}) for the doctor-proposing double cut DA for hospital $h$ is deferred to the appendix. Again, its proof needs non-trivial changes.

\hide{
\begin{lemma}\label{lem::hosp-high-value-match-prob}
Let $\delta>0$ be an arbitrarily small constant.
    Let $h$ be a hospital with public rating at least $a\alpha$.
    Suppose we run the doctor-proposing double-cut DA for hospital $h$ using the discretized utilities as specified in \Cref{clm::discrete-dist-idio}.
    Suppose the fraction of unmatched doctors with public rating in $[r(d)+(a+1)\alpha,1)$ is at most $3\exp\big(-\alpha k/4(4a+1)\big)$.
    Also, suppose that the event ${\mathcal B}$ does not occur.
    Finally, suppose we run the doctor-proposing double-cut DA for $h$.
     Then the probability that $h$ fails to $\kappa$ matches for which it has interview value $1-\psibar_h$ or larger is at most $\exp\big(-\frac{3k\alpha\psibar_h}{4(4a+1)}\big)$, if $a\ge 5$, $k\ge 4a+1$, and $\alpha\cdot\exp\big(\alpha k/4(4a+1)\big)\ge 3$.
\end{lemma}
}

% The proof of \Cref{lem::hosp-high-value-match-prob} is similar to the proof of \Cref{lem::doctors-high-value-match-prob}. We defer it to the appendix.

We finish up the argument by showing the bounds in these four lemmas apply
to the runs of the double-cut DA with the actual utilities drawn from a continuous range.

\begin{claim}\label{lem::cont-range-bound}
    The bounds of Lemmas \ref{lem::doctors-interval-non-match} and \ref{lem::doctors-high-value-match-prob} and the corresponding lemmas for the hospitals hold in the continuous setting too.
\end{claim}
\hide{
\begin{proof}
 For any given $\delta>0$, by \Cref{clm::discrete-dist-idio}, the actions in the continuous setting and the corresponding discrete setting can differ only when there is a difference in the preferences lists, which occurs with probability at most $\delta$.
 Therefore, by \Cref{lem::doctors-high-value-match-prob}, the probability that a doctor $d$ does not receive a proposal with interview value at least $1-\psibar_d$ is at most $\delta+ \exp\big(-k(\alpha-\delta)\psibar_d /(4a+1)\big)$.
 As this holds for any $\delta>0$, the actual probability is at most $\exp\big(-\alpha k\psibar_d /(4a+1)\big)$.
 Similar arguments apply to the bounds in the remaining three lemmas.
\end{proof}
}


\paragraph{Bad Events ${\mathcal B}$}
These bad events concern the number of agents with ratings in specified public rating intervals (for the sake of brevity, we will say agents in an interval).
We want to limit the analysis to the case where the number of such agents is reasonably close to its expectation. Our analysis will need to assume this for $O(n)$ intervals and unions of intervals.
We defer the details to the appendix.

\hide{
Let $I$ be an interval of public ratings or a union of such intervals of total length $l$.
We will identify two different pairs of bad events to handle the cases $l\ge \alpha$ and $l<\alpha$, respectively.
For the case $l\ge \alpha$, let $\Bhbf(I)$ and $\Bhbm(I)$ be the events that the number of hospitals in $I$ is smaller than $\big(\ell-\frac12 \alpha\big)\cdot \frac{n}{\kappa}$ and more than $\big(\ell+\frac12 \alpha\big)\cdot \frac{n}{\kappa}$, respectively.
For the case $l< \alpha$, let $\Bhsf(I)$ and $\Bhsm(I)$ be the events that the number of hospitals in $I$ is smaller than $\frac 12\ell\cdot \frac{n}{\kappa}$ and more than $2\ell \cdot \frac{n}{\kappa}$, respectively.
(H is for hospital, b for big and s for small $l$, f for too few and m for too many agents).
We define $\Bdbf(I)$, $\Bdbm(I)$, $\Bdsf(I)$ and $\Bdsm(I)$ analogously for doctors (D for doctor), with $n$ replacing $n/\kappa$ in the previous bounds.

We also want to define analogous events for the number of hospitals in $I$ other than a hospital $h$ known to be in $I$. For brevity, we write $\Bhbf(I\setminus h)$ instead of $\Bhbf(I\setminus\{r(h)\})$.
So, for example, if $h\in I$, we define $\Bhbf(I\setminus h)$ to be the event that the number of hospitals in $I$ is less than $\big(\ell-\frac12 \alpha\big)\cdot \big(\frac{n}{\kappa}-1\big)$, and similarly for $\Bhbm(I\setminus h)$, $\Bhsf(I\setminus h)$, $\Bhsm(I\setminus h)$, and likewise for the analogous events concerning doctors. 


\begin{claim}\label{lem::number-agents-in-intervals}
    Suppose $\frac {n}{\ln n}\ge \frac{12(c+2)\kappa \ell}{\alpha^2}$. If $l\ge \alpha$, then  $\Bhbm(I)$ and $\Bhbf(I)$ each occur with probability at most $n^{-(c+2)}$,
    while if $\ell\ge 8(c+2)\kappa\ln n/n$, then $\Bhsm(I)$ and $\Bhsm(I)$ each occur with probability at most $n^{-(c+2)}$.
    
    Similarly, if $\frac {n}{\ln n}\ge \frac{12(c+2)\ell}{\alpha^2}$, and $l\ge \alpha$ then $\Bdbm(I)$ and $\Bdbf(I)$ each occur with probability at most $n^{-(c+2)}$;
    and if $\ell\ge 8(c+2)\ln n/n$, then $\Bdsm(I)$ and $\Bdsf(I)$ each occur with probability at most $n^{-(c+2)}$.

    Analogous bounds hold with $I$ replaced by $I\setminus h$; the one change is that the $n/\kappa$ or $n$ in the relevant bound is replaced by $(n/\kappa)-1$ or $n-1$, respectively.
\end{claim}
\begin{proof}
    The expected number of hospitals in $I$ is $\ell\cdot \frac{n}{\kappa}$.
    By a Chernoff bound, there are more than $\big(\ell+\frac12 \alpha\big)\cdot \frac{n}{\kappa}$ hospitals in $I$ with probability at most $\exp\big(-\frac13\cdot \frac{\alpha^2}{4\ell}\cdot \frac{n}{\kappa}\big)\le n^{-(c+2)}$, if $\frac {n}{\ln n}\ge \frac{12(c+2)\kappa\ell}{\alpha^2}$.
     And by another Chernoff bound,
    there are fewer than $\big[\ell-\frac12\alpha\big]\cdot \frac{n}{\kappa}$ hospitals in $I$ with probability at most $\exp\big(-\frac12\big(1 - \frac {\alpha}{2\ell}\big)^2\ell\cdot \frac{n}{\kappa}\big)\le n^{-(c+2)}$, if $\frac {n}{\ln n}\ge 8(c+2)\kappa l$ (using $\ell\ge \alpha$).
    Similarly, there are more than $2 \ell \cdot\frac n{\kappa}$ hospitals in $I$ with probability at most $\exp\big(-\frac13\ell\cdot \frac n\kappa \big)\le n^{-(c+2)}$, and fewer than $\frac12\ell \cdot\frac n{\kappa}$ hospitals in $I$ with probability at most $\exp\big(-\frac18\ell\cdot\frac n{\kappa}\big)\le n^{-(c+2)}$, if $l\ge 8(c+2)\kappa \ln n/n$.
    \end{proof}

The next corollary shows that, for each doctor and hospital, its cone has a population close to its expectation with high probability.
To make this precise, we introduce the following notation.
Recall that $C(d)$ denotes the cone for doctor $d$; analogously, we let $C(h)$ be the cone for hospital $h$, the
set of doctors with public rating in the range $[r(h)-a\alpha,r(h)+a\alpha)$.
\begin{corollary}\label{cor::cone-population-correct}
    For each doctor $d$ and hospital $h$, the events
    $\Bdbm(C(h))$, $\Bdbf(C(h))$, $\Bhbm(C(d))$, $\Bhbf(C(d))$ each occur with probability at most $n^{-(c+2)}$.
    (Note that the cone for $h$ is an interval of doctors and vice-versa.)
\end{corollary}
\begin{proof}
    It suffices to note that the length of these intervals is typically $2a\alpha$, and at least $a\alpha$ (it can be shorter for the very topmost and bottommost agents), and then apply \Cref{lem::number-agents-in-intervals}.
\end{proof}

In the proofs of Lemmas~\ref{lem::doctors-interval-non-match}--\ref{lem::doctors-high-value-match-prob} we assume that none of these events occur, i.e.\ that all the cones have size fairly close to their expectation.
}

\subsection{Proof of \Cref{lem::doctors-high-value-match-prob}}\label{sec::proof-doc-match-prob}

% We fix the utilities for all edges other than those incident on $d$.

We  use \Cref{lem::hospitals-interval-non-match} along with \Cref{clm::double-cutDA-provides-bounds} to bound the number of not-fully matched hospitals in $[r(d)+\alpha,1)$ in the double-cut DA for $d$.
\begin{claim}\label{clm::matching-bounds-extend}
Let $I=[f,g)\subset [r(d)+(a+1)\alpha,1)$ be an interval of hospitals. Then every hospital that is fully matched in the doctor-proposing double-cut DA for $I$ will be fully matched in the hospital-proposing double-cut DA for $d$. 
\end{claim}
\begin{proof}
    The edges that are used in the double-cut DA for $I$ are to hospitals in the range $[g-\alpha,1)$ (as we will see later).
    The full set $F$ of edges from these hospitals all go to doctors in the range $[g-(a+1)\alpha,1)$.
    Therefore so long as $r(d)$ is in the range $[0,g-(a+1)\alpha)$, the double-cut DA for $d$ includes all of $F$, and additional edges forming a set $F'$.
    Now consider running the hospital-proposing DA with edge set $F'$. By \Cref{clm::double-cutDA-provides-bounds}, the outcome for the hospitals in $I$ on the run with $F'$ is at least as good as the run of the double-cut DA for $I$. But the doctor-proposing DA and the hospital-proposing DA yield the same fully matched hospitals (and doctors). Therefore all the hospitals that are fully matched in the double-cut DA for $I$ are also fully matched in the double-cut DA for $d$.
\end{proof}

\begin{claim}\label{lem::surplus-hosp-prop-one-doc}
    Suppose the following good events  occur: there are at most $[1-r(d)+\frac 32\alpha ]n$ doctors with public rating at least $r(d)-\alpha$ (the expected number is $[1-r(d)+\alpha ]n$ doctors), and there at least $[1-r(d)+(a-\frac32)\alpha] n/\kappa$ hospitals with public rating in the range $[r(d)-a\alpha,r(d)+a\alpha)\cup[r(d)+(a+1)\alpha,1))$ (the expected number is $[1-r(d)+(a-1)\alpha] n/\kappa$ hospitals).
    % $\Bdbm([r(d)-\alpha,1))$ and $\Bhbf([r(d)-a\alpha,r(d)+a\alpha)\cup[r(d)+(a+1)\alpha,1))$, and
    Also suppose that both $a\ge 5$ and $\alpha\cdot\exp\big(\alpha k/4(4a+1)\big)\ge 3$.
    Then the surplus $s\ge\alpha n/\kappa$.
\end{claim}
\begin{proof}
To bound the surplus, we start with the assumed lower bound on the number of available hospitals:
$[1-r(d)+(a-\frac32)\alpha] \frac{n}{\kappa}$.
We then subtract an upper bound given by \Cref{lem::doctors-high-value-match-prob} on the number of hospitals that did not fully match in the range $[r(d)+(a+1)\alpha,1)$, for by \Cref{clm::matching-bounds-extend},
all hospitals in this range that matched for intervals $I$ in this range, also match in the double-cut DA for $d$. We take a disjoint collection of intervals $I$ that cover this range; they contain at most $n/\kappa$ hospitals. Therefore, the number that are not fully matched is at most $\frac{n}{\kappa} \cdot 3\exp\big(-\alpha k/4(4a+1)\big) \le  \alpha \cdot \frac n{\kappa}$, if $\exp\big(- \alpha k/4(4a+1)\big)\le \frac 13\alpha$.
We then determine how many hospitals could be fully matched by the doctors at hand, which is at most $1/\kappa$ times the assumed upper bound on the number of doctors: $\frac1{\kappa}[1-r(d)+\frac 32\alpha ]n$. This yields a surplus of at least
 \hide{
    % As $\Bdbm([r(d)-\alpha,1))$ does not occur, 
    By assumption, the number of doctors with public rating at least $r(d)-\alpha$ is at most $[1-r(d)+\frac 32\alpha ]n$. 
    By the assumption in \Cref{lem::doctors-high-value-match-prob} and by \Cref{clm::matching-bounds-extend}, the number of not-fully matched hospitals in $[r(d)+(a+1)\alpha,1)$ is at most
    $3\frac n{\kappa}\cdot\exp\big(-\alpha\kappa k/4(4a+1)\big)\le  \alpha \cdot \frac n{\kappa}$, if $\exp\big(- \alpha\kappa k/4(4a+1)\big)\le \frac 13\alpha$.
    In addition, some or all of the hospitals in $[r(d)+a\alpha,r(d)+(a+1)\alpha)$ may not be fully matched.
    % As $\Bhbf([r(d)-a\alpha,r(d)+a\alpha)\cup[r(d)+(a+1)\alpha,1))$ does not occur,
    By assumption, the number of hospitals with public rating in $[r(d)-a\alpha,r(d)+a\alpha)\cup[r(d)+(a+1)\alpha,1))$ is at least $[1-r(d)+(a-\frac32)\alpha] n/\kappa$.
    Thus the surplus, the number of not-fully matched available hospitals in $d$'s cone, i.e., hospitals that could propose to $d$, is at least
    }
    \begin{align*}
        \big[1-r(d)+(a-\tfrac32)\alpha\big] \cdot\frac{n}{\kappa} - \big[1-r(d)+\tfrac 32\alpha\big]\cdot\frac{n}{\kappa} -  \alpha \cdot\frac{n}{\kappa}
        \ge \big(a - 4\big)\alpha\cdot \frac{n}{\kappa}\le \alpha \cdot \frac{n}{\kappa},
        ~~~~\text{if $a\ge 5$}.
    \end{align*}
\end{proof}

We put one more (harmless) stop on the hospital proposing double-cut DA in the statement of the lemma: if $d$ receives a proposal that provides
$d$ with interview value $1-\psibar_d$ or larger, we stop the run as the desired outcome has been achieved.
We fix the public ratings of the doctors and hospitals. We also fix all private values and interview values of the doctors other than $d$.
    
We model the possible runs of the double-cut DA using a tree $T$.
As we descend the tree, the maximum utility achievable by each hospital will be decreasing.
At each node $v$, each hospital $h$ has a current maximum possible utility $u(h,v)$, either due to its being tentatively matched with this utility, or having the possibility of achieving this utility, but no larger, due to the remaining random choices; this is called $h$'s \emph{current utility} for short.
In making these random choices, we will allow the hospitals to partially or fully determine some interview values before we determine whether there is an interview.

The nodes and the edges to $v$'s children represent the possible actions by one currently unmatched hospital (if several hospitals could make a proposal or one hospital could make several proposals due to ties in utility values, to avoid ambiguity, a fixed tie-breaking ordering is used; in a subsequent lemma we will impose some mild, but feasible, requirements on the tie-breaking). 
$T$ has two types of nodes. A node is of the first type if it corresponds to a proposal by some hospital $h$ to a doctor $d'\ne d$, where this proposal provides $h$ utility equal to its current possible utility $u(h,v)$.
Due to the tie-breaking, there can be only one such doctor $d'$ at node $v$. 
Reflecting this, there is a single edge descending from $v$ corresponding to making this proposal.
A node $v$ is of the second type if it corresponds to a possible proposal by a hospital $h$ to doctor $d$ providing $h$ utility equal to its current utility $u(h,v)$; below, we write $u=u(h,v)$ for brevity. The following are the possible actions at such a node $v$:
    \begin{itemize}
        \item The choice that $h$ have interview value $u-r(d)$ for $d$ and there is a proposal to $d$ with doctor interview value at least $1-\psibar_d$. We call this a \emph{high-real proposal}. We terminate the DA run at this point, as this achieves the desired outcome. 
        \item The choice that $h$ have interview value $u-r(d)$ and there is a proposal to $d$ with doctor interview value less than $1-\psibar_d$. We call this a \emph{low-real proposal}. 
        We don't allow $h$ to make any further proposals.
        \item The choice that $h$ have interview value $u-r(d)$ but there is no proposal to $d$, because there was no interview (this is a ``no action'' step, but we need to handle it separately). We call this an \emph{imaginary proposal}. Again, we don't allow $h$ to make any further proposals. % (Of course, if the proposal does not exist , then there is no interview value. But, 
        (For the purposes of the analysis, we want to choose the interview value before we determine whether there was an interview.)
        \item ``No action'' (due to the determination that $h$'s remaining interview values are smaller than needed to make a proposal currently; the next node corresponds to $h$ checking if it has a proposal at its next utility value in decreasing order of utilities).
    \end{itemize}
    Let $q(v)$ be the probability that at node $v$ the continuation of the run of the double-cut DA results in zero high-real proposals to doctor $d$. 
    We wish to analyze a corresponding setting with independent proposals, which will have probability
    $\qtilde(v)\ge q(v)$ of zero real proposals at node $v$; $\qtilde$ is designed so that it will be straightforward to upper bound $\qtilde(\treeroot)$.
    
    To define $\qtilde(v)$ we consider the following setup.
    Let $h$'s \emph{residual utility} at node $v$, $u(h,v)$, equal the current utility $u$ minus the minimum utility allowed in the run of the double-cut DA, namely $r(d)+1-\alpha$.
    % , minus the length of the excluded utilities from fixing the utilities w.r.t.\ doctors $d'\ne d$, which is at most $n/z\le \delta$.
    Let $s$ be the minimum surplus over all the possible paths in the computation, assuming no bad events happen.
    Suppose that above node $v$ there have been $x$ low-real proposals and $y$ imaginary proposals to $d$.
    Let $S(v)$ be the set of the $s-x-y$ hospitals with the smallest residual utilities
    among those that have not made a real or imaginary proposal to $d$ already.
    Suppose that among the $|C(d)|-x-y$ hospitals that have not made a real or imaginary proposal to $d$, $k-x$ are chosen uniformly at random. Suppose we then have each of the selected hospitals in $S(v)$ choose its interview value and propose to $d$ if the interview value is at least $1-\alpha$.
Then $\qtilde(v)$ is defined to be the probability that this process results in no high-real proposal to $d$.
In \Cref{clm::fixed-k-stoc-dom-idio},
we will show that $\qtilde(v)\ge q(v)$.
Before proving this claim, we deduce a bound in the $\qtilde$ setting, and therefore in the $q$ setting also, on the probability that $d$ receives no proposal for which $d$ has interview value at least $1-\psibar_d$.

\begin{claim}\label{lem::fail-prob-hospital-prop}
    Let $d$ be a doctor with public rating at least $a\alpha$.
    Suppose $s\ge \frac{\alpha n}{\kappa}$ and that
    there are at most $\frac12(4a+1)\frac{\alpha n}{\kappa}$ hospitals in $C(d)$ (the expected number is $\frac{2a\alpha n}{\kappa}$, except at the ends of the public rating range where it can be as low as $\frac{a\alpha n}{\kappa}$). Then the probability in the $\qtilde$ setting that $d$ receives no proposal for which $d$ has interview value at least $1-\psibar_d$ is at most $\exp\big(-2k\alpha\psibar_d/(4a+1)\big)$.
\end{claim}
\begin{proof}
    For each hospital $h$, its residual utility at the root of $T$ is at least $\alpha$.
    Consider a hospital $h$ in the surplus.
    The probability that $h$ is selected by $d$ is at least $\frac{k}{|C(d)|}\ge \frac{2k\kappa}{(4a+1)\alpha n}$. The probability that $h$ has interview value at least $1-\alpha$, as required by the double-cut DA for $h$ to propose this edge, is $\alpha$,
    and the probability that $d$ has interview value at least $1-\psibar_d$ for $h$ is $\psibar_d$.
    So the probability that there is an edge from $h$ to $d$ that is chosen by the double cut DA and
    that provides $d$ interview value at least $1-\psibar_d$ is at least $\frac{2k\kappa\psibar_d}{(4a+1)n}$.
    Therefore the probability that $d$ receives no such edge is at most
    $\big(1- \frac{2k\kappa\psibar_d}{(4a+1)n}\big)^s\le \exp\big(-\frac{2k\alpha\psibar_d}{4a+1}\big)$,
    as $s\ge \frac{\alpha n}{\kappa}$.
    \hide{
    The expected number of hospitals in $S(\treeroot(T))$ that are selected by $d$ is
    $ks/|C(d)|\ge 2k\frac{\alpha  n}{\kappa}/(4a+1)\frac{\alpha n}{\kappa}= 2k/(4a+1)$.
    If in addition, the hospital has interview value at least $1-\alpha$, as required by the double-cut DA, and $d$ has interview value at least $1-\psibar_d$, the expected number becomes
    $2k\alpha\psibar_d/(4a+1)$.
    By a Chernoff bound, the probability that there are no such hospitals is at most
    $\exp\big(-k\alpha\psibar_d/(4a+1)\big)$. 
    }
\end{proof}

\begin{claim}\label{clm::fixed-k-stoc-dom-idio}
    For every node $v$ in $T$, $\qtilde(v)\ge q(v)$.
\end{claim}
\begin{proof}
We prove the result by an induction from the leaves to the root of tree $T$.

Recall that $u(h,v)$ denotes the residual utility of $h$ at node $v$,
and let $u_1\le u_2\le \ldots\le u_{s-x-y}$ be the $s-x-y$ smallest residual utilities being used to calculate $\tilde{q}(v)$; the hospitals that have already proposed to $h$ are excluded.

\smallskip\noindent
\emph{Base case: a leaf node}\\
At a leaf node $v$ all the random decisions have been made, so either $d$ has received the desired proposal or not. Therefore $q(v)=\qtilde(v)$.

\smallskip\noindent
\emph{Inductive step at an internal node $v$ with one child $w$}\\
Here $q(v)=q(w)$ and $\qtilde(v)=\qtilde(w)$.
So the inductive claim holds trivially.

\smallskip\noindent
\emph{Inductive step at an internal node $v$ with 4 children}\\
Let $h$ be the hospital making a random choice at node $v$.
Let its children be named $\wrh$, corresponding to a real high proposal to doctor $d$, $\wrl$, corresponding to a real low proposal to doctor $d$, 
$\wim$, corresponding to an imaginary proposal to $d$,
and $\wna$, corresponding to ``no action''.
Recall that $d$ has received $x$ low-real and $y$ imaginary proposals prior to reaching node $v$.
Then $\qtilde(v)$ is calculated using $s-x-y$ residual utilities,
$\qtilde(\wna)$ is calculated using $s-x-y$ residual utilities, 
while $\wrl$ and $\wim$ are calculated using $s-x-y-1$ residual utilities,
as in these cases, $h$ makes no further proposals in the run of the double-cut DA;
$\wrh$ is a terminal node as it achieves the desired outcome of a proposal to $d$ with a ``high'' interview value (at least $1-\psibar_h$).
Note that $q(\wrh)=\qtilde(\wrh)=0$.
Finally, in the calculation of $\qtilde(\wna)$, all the residual utilities except at most one are unchanged; the only one that may change is due to the fact that $u(h,\wna)<u(h,v)$. 

Let $p_w$ be the probability that the edge from $v$ to its child $w$ is chosen when at node $v$.
Then $q(v) = \sum_{\text{$w$ a child of $v$}} p_w \cdot q(w)$.
To prove our inductive bound it will suffice to show that
\begin{align}\label{eqn::qtilde-bound-idio}
    \qtilde(v) \ge \sum_{\text{$w$ a child of $v$}} p_w \cdot \qtilde(w).
\end{align}

\smallskip\noindent
\emph{Case 1.} $u(h,v)$ is among the smallest $s-x-y$ residual utilities at node $v$\\
This immediately implies that $u(h,\wna)$ is among the smallest $s-x-y$ residual utilities at $\wna$, as $u(h,w)<u(h,v)$. The residual utilities for the other hospitals are unchanged at every child of $v$.

In this case, we show that \eqref{eqn::qtilde-bound-idio} holds with equality.
To do this we consider the random choices that are made in evaluating $\qtilde(v)$,
by instantiating exactly the randomness needed to select a child $w$ of $v$.

One way to make these random choices is to determine if $h$'s utility for
$d$ equals the utility at node $v$; if so, a further random choice determines if the
proposal is real or imaginary.
If it is real, yet another random choice determines if it is high or low.
At each child, we then make the remaining random choices to determine the probability
of no high-real proposal to $d$. But at each node $w$, this probability
is exactly $\qtilde(w)$, for we are using the same random variables apart from $h$'s
utility which is either the value $u(h,v)$ or a value determined at $\wna$; furthermore, this utility is not used at $v$'s other children.
Thus $\qtilde(v)=\sum_{\text{$w$ a child of $v$}} p_w\cdot \qtilde(w)$ in this case.

\smallskip\noindent
\emph{Case 2}.  $u(h,v)$ is not among the smallest $s-x-y$ residual utilities at node $v$.\\
Because of the rounding of the utilities, this implies that $u(h,\wna)\ge u_{s-x-y}$. All the other
residual utilities are unchanged, and therefore $\qtilde(v)=\qtilde(\wna)$.
Consider the effect of increasing $u_{s-x-y}$ to $u(h,\wna)$. At each child $w\ne \wna$ of $v$, this leaves $\qtilde(w)$ unchanged. However, $\qtilde(v)$ and $\qtilde(\wna)$ are reduced equally,
as the increase to $u_{s-x-y}$ increases the probability that a proposal to $d$ occurs.
Therefore if \eqref{eqn::qtilde-bound-idio} held after this increase, it would have held before the increase.
Now increase $u_{s-x-y}$ further to $u(h,v)$. $\qtilde(v)$ continues decreasing, but all
the $\qtilde(w)$ are unchanged, for $w$ a child of $v$.
When $u_{s-x-y}=u(h,v)$, this becomes an instance of Case 1, at which point \eqref{eqn::qtilde-bound-idio} holds.
We conclude that \eqref{eqn::qtilde-bound-idio} held prior to the increase of $u_{s-x-y}$.
\end{proof}

\hide{
\begin{claim}\label{clm::conditions-hosp-prop-one-doctor}
 The conditions in Claims~\ref{lem::surplus-hosp-prop-one-doc} and~\ref{lem::fail-prob-hospital-prop} amount to the following constraints: $a\ge 5$,  and $\alpha\cdot\exp\big(\alpha\kappa k/4(4a+1)\big)\ge 3$.
 They also exclude events with total probability at most $3n^{-(c+1)}$.
 \end{claim}
}


\hide{
\subsection{Proof of \Cref{lem::hosp-high-value-match-prob}}\label{sec::proof-hosp-match-prob}
 
 This is quite similar to the proof of \Cref{sec::proof-doc-match-prob}, except that the roles of the doctors and hospitals are switched.

We will use the following high-probability lower bound $1-\taubar$ on the private values of the edges selected by each doctor $d$.

\begin{claim}\label{clm::value-of-taubar}
    Let $b>2$ and $c>0$ be constants. Suppose that $\Bhbf(C(d))$ does not occur for any doctor $d$.
    Suppose $\taubar\ge \frac{b(c+2)\ln n} {(a-\frac 12)\frac{\alpha n}{\kappa}}$. Then, for each doctor $d$, with failure probability at most $n^{-(c+2)}$, if $k \le \big(1-\big(\frac 2b\big)^{1/2}\big) \cdot b(c+2)\ln n$,
    $d$ has at least $k$ in-cone edges with private value $1-\taubar$ or larger.
\end{claim}
\begin{proof}
As $\Bhbf(C(d))$ does not occur, the number of hospitals in $d$'s cone is at least $(a-\frac 12)\cdot\frac{\alpha n}{\kappa}$.
    The expected number of $d$'s in-cone edges with private value $1-\taubar$ or larger
    is at least $\taubar$ times the number of hospitals in her cone, i.e.\ $\taubar (a-\tfrac12)\cdot \frac{\alpha n}{\kappa}\ge b(c+2)\ln n$,
    as $\taubar \ge \frac{b\kappa(c+2)\ln n} {(a-\frac12)\alpha n}$.
    Then, by a Chernoff bound, the probability that she
    has fewer than $k$ such edges is at most $\exp\big[-\tfrac b2 (c+2)\ln n \big(1 - \frac k{b(c+2)\ln n}\big)^2\big]
    \le n^{-(c+2)}$, if $k \le \big(1-\big(\frac 2b\big)^{1/2}\big) \cdot b(c+2)\ln n$.
\end{proof}

Going forward, we suppose the event $\Btau$, that some doctor fails to have $k$ edges with private value $1-\taubar$ or larger does not occur.

\begin{claim}\label{lem::surplus-hosp-prop-one-hosp}
    Suppose the following bad events do not occur:
    $\Bhbm([r(h)-\alpha,1))$ and $\Bdbf([r(d)-a\alpha,r(d)+a\alpha)\cup[r(d)+(a+1)\alpha,1))$, and also suppose that both $a\ge 5$ and $\alpha\cdot\exp\big(\alpha k/4(4a+1)\big)\ge 3$.
    Then the surplus $s\ge\alpha n$.
\end{claim}
\begin{proof}
    As $\Bhbm([r(h)-\alpha,1))$ does not occur, the number of hospitals with public rating at least $r(h)-\alpha$ is at most $[1-r(h)+\frac 32\alpha ]\frac{n}{\kappa}$. As $\Bdbf([r(d)-a\alpha,r(d)+a\alpha)\cup[r(d)+(a+1)\alpha,1))$ does not occur,
    the number of doctors with public rating in this range is at least $[1-r(h)+(a-\frac32)\alpha] n$.
    By the assumption in \Cref{lem::doctors-interval-non-match}, the number of unmatched doctors in $[r(h)+(a+1)\alpha,1)$ is at most
    $3n\cdot\exp\big(-\alpha k/4(4a+1)\big)\le  \alpha n$, if $\exp\big(- \alpha k/4(4a+1)\big)\le \frac 13\alpha$.
    Thus the surplus, the number of unmatched available doctors in $h$'s cone, i.e., doctors that could propose to $h$, is at least
    \begin{align*}
        \big[1-r(h)+(a-\tfrac32)\alpha\big] n - \big[1-r(h)+\tfrac 32\alpha\big]n -  \alpha n
        \le \big(a - 4\big)\alpha n\le \alpha n,
    \end{align*}
    if $a\ge 5$.
\end{proof}

As in \Cref{sec::proof-doc-match-prob}, the tree $T$ of possible runs of the double-cut DA has
both real and imaginary proposals. For each edge $(d',h')$ for any doctor $d'$ outside $C(h)$ we fix the utilities for both $d'$ and $h'$.
Also, for each doctor $d$ in $C(h)$, we fix its top $k$ private values, but without specifying which edges these values are attached to.
Now, we are seeking the probability that $h$ receives fewer than $\kappa$ proposals from the doctors in $C(h)$. Again, we obtain the bound by showing that $\qtilde(v) \ge q(v)$ for all nodes $v$ in $T$, and for $\treeroot(T)$ in particular, but the meanings of $q$ and $\qtilde$ are slightly different here.

A node corresponding to an action by a doctor outside $C(h)$ has just one outgoing edge corresponding to its single possible action (using the tie-breaking if needed). For a doctor $d$ in $C(h)$, the set-up is more elaborate. Let $1-\tau_1\ge 1-\tau_2\ge \ldots\ge 1-\tau_k$ be the private values for its $k$ edges; let's name the corresponding proposals $e_1,e_2,\ldots,e_k$. $T$ will have a series of nodes corresponding to deciding in turn, whether each $e_i$ provides $d$ utility equal to its current utility (this is the constraint on the tie-breaking mentioned earlier; we use the private values to order edges that produce equal utility; if there is also a tie in the private values, we use some further arbitrary but fixed rule). For each potential proposal, the decision making proceeds in two steps:
first, whether the proposal has a utility equal to $d$'s current utility value in tree $T$;
note that we have not yet chosen the hospital that receives this proposal. This is a decision based on making a random choice for its interview value. 
For each hospital $h$ for which the current utility is possible for $d$, which we call $d$'s current cone, the probability that $h$ receives this proposal is the same.
In the $q$ setting, we then choose the edge uniformly from the hospitals in $d$'s current cone that she has not already proposed to; in this setting, there are no imaginary proposals.
A doctor stops making proposals either when she has gone through all $k$ of her proposals or she makes a proposal to $h$.
Let $x$ be the number of proposals $h$ has received prior to reaching node $v$.
Then $q(v)$ is the probability that $h$ receives at most $\kappa -x -1$ further proposals in the
computation starting at $v$.

In the $\qtilde$ setting, we keep track of how many proposals a doctor has made.
Again, as soon as a doctor makes a proposal, real or imaginary, to $h$, she stops.
Now, we let $x$ be the number of real proposals to $h$ and $y$ the number of imaginary proposals to $h$.
Let $k(d,v)$ be the number of remaining
proposals for doctor $d$ at node $v$. Also, recall that $u(d,v)$ is her residual probability at node $v$.
To evaluate $\qtilde(v)$, the doctors with the $s-x-y$ smallest products $u(d,v)\cdot k(d,v)$ will attempt to propose; each real proposal will occur with the same probability, which will be no larger than the probability of a proposal in the $q$ setting; the difference in probability will be handled by making proposals imaginary with probability equal to the difference. Now, we make this precise.

We use the same value for the probability that $d$ has a proposal with the current utility $u$ as in the $q$ setting. 
If $d$ is found to have such a proposal, uniformly at random, we choose one of the hospitals in $d$'s current cone that has not already received a proposal from $d$ to receive the proposal; then we choose whether it is real with probability $\tau=1 -\big(1 - \frac {1}{(2a+\frac12)\alpha n}\big)^{k(d,v)}$.
As in \Cref{sec::doc-int-idio-no-match}, $\tildep(\wrl(h))\le p(\wrl(h))$; again, we choose
$\tildep(\wim(h))=p(\wim(h))+[\wrl(h))-\tildep(\wrl(h)]$.


\begin{claim}\label{clm::qtilde-larger-for-intervals-in-doc-prop}
    $\qtilde(v)\ge q(v)$ for all $v$ in $T$.
\end{claim}
\begin{proof}
    The base case argument is unchanged from \Cref{clm::fixed-k-stoc-dom-idio}.

    \smallskip\noindent
    \emph{Case A}. The proposal is to some $h'\ne h$:
    
    Then $v$ has two children $\wrl(h')$, $\wim(h')$, $\wrl$ and $\wim$ for short.
    Here $k(d,w)=k(d,v)-1$ and $u(d,w)<u(d,v)$, for $w=\wrl,\wim$; the variables associated with the other doctors are unchanged. At both children, we seek the probability that $h$ receives at most $\kappa-x-y-1$ proposals. 
    
Also,  $\ptilde(\wrl) \le p(\wrl)$: for the edge is real in the $\qtilde$ setting with probability
$\tau$; this value is computed assuming the cone sizes for all $d\in C(h)$ are as large as possible;
this only reduces the probability of the edge being real.
Then $\ptilde(\wim)=p(\wrl)-\ptilde(\wrl)$.
    
In addition, $\qtilde(\wrl)=\qtilde(\wim)$, for in both settings the doctors have the same $k$ and $u$ values. (One may wonder at this seemingly unnecessarily complex setup; but it is used later in the proof of \Cref{lem::fail-prob-doctor-prop}).

Now, we deduce our result with the help of a little algebra.
\begin{align*}
    \ptilde(\wim)\cdot \qtilde(\wim) + \ptilde(\wrl)\cdot \qtilde(\wrl) 
    & =   [\ptilde(\wim) + \ptilde(\wrl)]\cdot \qtilde(\wrl)\\
    &=p(\wrl)\cdot \qtilde(\wrl)\\
    &\ge p(\wrl)\cdot q(\wrl).
\end{align*}

    \smallskip\noindent
    \emph{Case B}. The proposal is to $h$:
    
    Then $v$ has three children: $\wrl(h)$ and $\wim(h)$ (again $\wrl$ and $\wim$ for short), plus the child $\wna$, corresponding to real and imaginary proposals, and to ``no action''. Note that $\wrl$ is a terminal node, because $h$ has receives a proposal on reaching this node.
    At both $\wim(h)$ and $\wna$ we are seeking the probability of at most $\kappa-x-1$ real proposals to $h$, from respectively the doctors with the smallest $s-x-y-1$ and $s-x-y$ $u$--$k$ products.

     \smallskip\noindent
     \emph{Case 1}. $u(d,v)\cdot k(d,v)$, the proposal probability for $h$ at node $v$, is among the $s-x-y$ smallest proposal probabilities, $u_1k_1\le u_2k_2\le\ldots\le u_{s-x-y}k_{s-x-y}$, at node $v$. \\
     Since only $u(d,w)$ and $k(d,w)$ change (by becoming smaller) at any of $v$'s children $w$, the proposal probability for $d$ continues to be among the $s-x-y$ smallest at the children where it is still in use. 
     $\ptilde(\wna)=p(\wna)$, and as in case A, $\ptilde(\wrl) \le p(\wrl)$ and $\ptilde(\wim)=p(\wrl)-\ptilde(\wrl)$.
     Therefore instantiating the randomness needed to choose an edge to a child of $v$ ensures that $\qtilde(v)=\ptilde(\wim)\cdot \qtilde(\wim) + \ptilde(\wna)\cdot \qtilde(\wna)\ge p(\wim)\cdot \qtilde(\wim) + p(\wna)\cdot \qtilde(\wna) = p(\wna)\cdot\qtilde(\wna)\ge p(\wna)\cdot q(\wna)=q(v)$.

     \smallskip\noindent
     \emph{Case 2}. $u(d,v)\cdot k(d,v)$, the proposal probability for $h$ at node $v$, is not among the $s-x-y$ smallest proposal probabilities at node $v$. \\
     The argument is identical to the Case 2 argument in \Cref{clm::fixed-k-stoc-dom-idio}.
\end{proof}

\begin{claim}\label{lem::fail-prob-doctor-prop}
    Let $h$ be a hospital with public rating at least $a\alpha$.
    Suppose $\Bdbm(C(h))$ does not occur. Then the probability that $h$ receives fewer than $\kappa$ proposals for which $h$ has interview value at least $1-\psibar_h$ is at most $\exp\big(-3\kappa k\alpha\psibar_h/8(4a+1)\big)$, if $\taubar \le \frac14\alpha$ and $k\ge 4a+1$.
\end{claim}
\begin{proof}
    For each doctor $d$, her residual utility at the root of $T$ is at least $\alpha$.
    The expected number of doctors in $S(\treeroot(T))$ that selected $h$ is
    $ks/|C(h)|\ge k\alpha n/(2a+\frac12)\alpha (n/\kappa)= \kappa k/(2a+\frac12)$, as $\Bdbm(C(h))$ does not occur.
    If in addition, the doctor has interview value at least $1-\alpha+\taubar$ and $h$ has interview value at least $1-\psibar_h$, the expected number becomes
    $2\kappa k(\alpha-\taubar)\psibar_h/(4a+1)$.
    By a Chernoff bound, the probability that there are fewer than $\kappa$ such doctors is at most
    $\exp\big(-\frac 12\cdot 2\kappa k(\alpha-\taubar)\psibar_h/(4a+1)\cdot\big[1 -\frac{4a+1}{2k}\big]\big)\le \exp\big(-\kappa k(\alpha-\taubar)\psibar_h/2(4a+1)$, if $k\ge 4a+1$. 
\end{proof}

\begin{claim}\label{clm::conditions-doctor-prop-one-hosp}
 The conditions in Claims~\ref{clm::value-of-taubar}---\ref{lem::fail-prob-doctor-prop} amount to the following constraints: $a\ge 5$, $k\ge 4a+1$, and $\alpha\cdot\exp\big(\alpha k/4(4a+1)\big)\ge 3$.
 They also exclude events with total probability at most $\big(2n+\frac{3n}{\kappa} \big)\cdot n^{-(c+2)}$.
 \end{claim}
}

\subsection{Overview of the Proof of \Cref{lem::doctors-interval-non-match}}
\label{sec::doc-int-idio-no-match}

The participating doctors are those with public rating at least $g-\alpha$.
The participating hospitals are a subset of those with public rating at least $g-a\alpha$, which we specify more fully below. Our goal is to handle the set of doctors in $I$ in the same way as we handled the single doctor $d$ in \Cref{lem::doctors-high-value-match-prob}. The challenge we face is that the stochastic tree dominance argument is going to show, for a suitable bound $r$, the probability that at most $r$ doctors in $I$ receive proposals is upper bounded by the probability of this event for $s$ independent proposals to $I$. However, we need to ensure that each of these proposals is roughly uniform over $I$,
and this need not be true for all the proposals we consider.


% This requires the removal of some hospitals with rating at least $g-a\alpha$.

To achieve this near uniformity, we start by excluding all hospitals with public rating in the range $[f+a\alpha,g+a\alpha)$, for these are the hospitals that are in cone for some but not all the doctors in $I$. We note that
the hospitals in the range $L\triangleq [g-a\alpha,f+a\alpha)$ are in-cone for all doctors in $I$.

Next, we remove any hospital in $L$ that has two or more edges to doctors in $I$ (typically, most hospitals in this range have no such edges), for the first proposal to $I$ from such hospitals would not be uniform over $I$.
In addition, the doctors $d$ incident on these edges are removed, as are the
hospitals which are neighbors of removed doctors.
Let $I'$ and $L'$ be the resulting sets of doctors and hospitals, respectively.
We note that the second set of removed hospitals each had only one edge to doctors in $I$,
and therefore the doctors in $I'$ each have all their $k$ edges incident on hospitals in $L'$.
In \Cref{clm::hosp-removal-lots-edges} we show that $|I'|\ge |I|\big[1-\exp\big(-\alpha k/4(4a+1)\big)\big]$ with high probability.
% Let $\Bcol$ be the event that more than $|I|\exp\big(-\alpha k/4(4a+1)\big)$ edges collide. Going forward, we assume that $\Bcol$ does not occur.

\hide{
\begin{claim}\label{clm::hosp-removal-lots-edges}
Suppose that the following events do not occur: $\Bdsf(I)$ and $\Bhbf(C(d))$ for all $d\in I$.
Then at most $|I|\exp\big(-\alpha k/4(4a+1)\big)$ hospitals are removed because they have 2 or more edges to doctors in $I$, 
at most $|I|\exp\big(-\alpha k/4(4a+1)\big)$ doctors are incident on the removed edges, and at most $|I|k\exp\big(-\alpha k/4(4a+1)\big)$ hospitals and edges incident on $I$ are removed, with failure probability at most $n^{-(c+2)}$, if\\ $2(c+2)\exp\big(\alpha k/4(4a+1)\big)\cdot \frac{\ln n}{n} \le g-f \le 2(a-\frac12)\alpha\exp\big(-\alpha k/4(4a+1)\big)/(e^2k^2\kappa)$.
\end{claim}
\begin{proof}
  We begin by giving a bound the number of edges from $I$ that collide, i.e., that have the same hospital as an endpoint.
  As $\Bhbf(C(d))$ does not occur for any $d\in I$, $|C(d)| \ge (a-\frac12)\alpha n/\kappa$ for each
  $d\in I$. For brevity we let $m$ denote $(a-\frac12)\alpha n/\kappa$.
  The probability that an edge from $I$ collides with any of the other edges out of $I$ is at most
  $\frac{(|I|-1)k}{m}\le \frac{|I|k}{m}=\frac{|I|k\kappa}{(a-\frac12)\alpha n}$. To give a high probability bound on the number of colliding edges
  we use stochastic dominance: we consider $|I|k$ 0/1 random variables which are 1 with probability
  $\frac{|I|k\kappa}{(a-\frac12)\alpha n}$. Their sum has expectation bounded by $b=\frac{|I|^2k^2\kappa}{(a-\frac12)\alpha n}$. Hence, by a Chernoff bound, the probability that the sum is greater than $s=|I|\exp\big(-\alpha k/4(4a+1)\big)$ is at most
  \begin{align*}
      \Big(\frac {e^{(s/b) -1}}{(s/b)^{s/b}}\Big)^{b}
      \le \Big(\frac{eb}{s}\Big)^{s} 
      = \Big(\frac{e|I|k^2\kappa\exp\big(\alpha k/4(4a+1)\big)}{(a-\frac 12) \alpha n}\Big)^{|I|\exp(-\alpha k/4(4a+1))}.
  \end{align*}
  This probability is maximized when $|I|$ is as small as possible, and as $\Bdsf(I)$ does not occur,
  this is when $|I|=\frac 12(g-f)n$.
  Then the probability is bounded by $n^{-(c+2)}$
  if $g-f\ge 2(c+2)\exp(\alpha k/4(4a+1))\cdot \frac{\ln n}{n}$ (which causes the exponent in the above expression to be at least $(c+2)\ln n)$, and $g-f \le 2(a-\frac12)\alpha\exp\big(-\alpha k/4(4a+1)\big)/(e^2k^2\kappa)$ (which causes the base term to be at most $1/e$).
  
  By stochastic dominance, $|I|\exp\big(-\alpha k/4(4a+1)\big)$ is also a bound on the number of edges that collide, and hence the
  number of hospitals with two or more edges into $I$ and the number of doctors incident on colliding edges. Therefore, in total, at most $|I|k\exp\big(-\alpha k/4(4a+1)\big)$ edges and hospitals are removed.
\end{proof}
}


We partially exclude some additional hospitals so as to ensure that they have a roughly equal probability of proposing to any doctor in $I'$ throughout the run of the double-cut DA.
In particular, for each doctor $d'\in I'$, if the hospital obtains a utility in the range
$[r(d')+1-\alpha,r(d')+1)$, we want the utility to be in the smaller range
$\cap_{d\in I'}[r(d)+1-\alpha,r(d)+1)=[g+1-\alpha,f+1)$.
To achieve this, we terminate the run of any of these hospitals which obtains a utility in the range
$([r(d)+1-\alpha,r(d)+1) \subset \big([f-\alpha,g-\alpha)\cup [f+1,g+1)\big)\cap([r(d)+1-\alpha,r(d)+1)$ for any doctor $d$ in $I'$ (note that $f\le r(d)<g$), right before they make such a proposal.



The rest of the argument will be similar to the one for \Cref{lem::doctors-high-value-match-prob}.
       For this result we are only seeking to ensure matches, and not that the doctors achieve high interview values. 
       %Still, we want the hospitals to make lots of ``real'' proposals to the doctors in $I'$ so as to ensure most of these doctors are matched; this makes the structure of the analysis somewhat similar to that in the prior lemma.  %We let $r+1$ be the desired number of real proposals; we specify $r$ later.
%
To this end, we fix $I'$ and the utilities for all doctors outside of $I'$.
We will be seeking to analyze the double-cut DA as if $I'$ was a single doctor that makes $k|I'|$ proposals.
The reason this does not cause difficulties is that because of the above exclusions 
% assuming $\Bcol$ does not occur, then 
every edge from a doctor in $I'$ to a hospital in $\cap_{d\in I} C(d)$ is to a distinct hospital.

\hide{
The nodes and edges in the tree $T$ of possible computations in the run of the double cut DA need to be redefined. Now we partition proposals according to whether they go to a doctor outside $I'$ or to a doctor in $I'$. As before, a node corresponding to a proposal to $d\notin I'$ will have a single child.
Proposals to doctors in $I'$ can be real or imaginary, but we no longer distinguish high-real and low-real proposals. Again, the need for imaginary proposals is due to selecting $h$'s utility before determining whether there is an edge from $I'$ to $h$.

Following this, we redefine $q(v)$ and $\qtilde(v)$, as follows.
We let $x$ denote the number of doctors in $I'$ who receive actual or real proposals before the computation reaches node $v$.
Each time a proposal is made to a doctor $d$ in $I'$, she might as well remove the remaining $k-1$ edges to $d$ as they will not cause any new doctors to receive a proposal.
This results in the removal of $k$ hospitals: the one making the real proposal, and the $k-1$ others with edges to $d$.
Next, we let $y$ denote the number of imaginary proposals to doctors in $I'$ who have not received a real proposal when node $v$ is reached. Again, we will stop the computation of the proposing hospital following any imaginary proposal to a doctor in $I'$. So at node $v$, $kx+y$ hospitals will have had their runs stopped. (The reason for the slightly convoluted definition of $y$ is that the $kx$ term may include some imaginary proposals.)
        
        Then $q(v)$ is defined to be the probability that at node $v$ the continuation of the run of the double-cut DA results in at most $r-x$ additional real proposals to doctors in $I$. As before, let $h$'s \emph{residual utility} at node $v$, $u(h,v)$, equal the current utility $u$ minus the minimum allowed utility in this run of the double cut utility, namely $u-(g+1-\alpha)$, minus the maximum utility range lost due to the elimination of equal utilities, namely at most $n/z<\delta$. Let $s$ be the minimum surplus over all the possible paths in the computation assuming no bad events occur.
    Let $S(v)$ be the set of the $s-x-y$ hospitals with the smallest residual utilities
    among those which have not made a real or imaginary proposal to a doctor in $I$ before reaching $v$.
    
    To define $\qtilde(v)$ we consider the following setup. 
    Suppose that the $s-kx-y$ hospitals with the smallest residual utilities independently attempt to make a proposal, real or imaginary, with probability corresponding to their residual utility. Suppose that, for each proposal, we then select whether it is real with probability $\tau =1 -\big(1-\frac 1{(2a+\frac12)\alpha n/\kappa}\big)^{k(|I'|-x)}$, where $|I'|$ is the number of doctors in $I'$ and $(2a+\frac 12)\alpha n/\kappa$ is an upper bound on the number of hospitals in $\cap_{d\in I} C(d)$, the intersection of the cones for $d\in I$, assuming $\Bhbm(C(d))$ does not occur for any $d\in I$. 
Then $\qtilde(v)$ is defined to be the probability that this process results in proposals to at most $r-x$ more doctors in $I'$.  
}

\hide{
\begin{claim}\label{clm::qtilde-bound-for-hosp-doc-int}
    $\qtilde(v)\ge q(v)$ for all $v$ in $T$.
\end{claim}
\begin{proof}
The proof that $\qtilde(v)\ge q(v)$ for all nodes $v$ is similar to the proof in \Cref{lem::doctors-high-value-match-prob}. There are three significant changes.
We no longer distinguish low-real and high-real proposals; rather than determining the probability of zero high-real proposals, we want to determine the probability of at most $r$ real proposals to distinct doctors in $I'$.
The second change is related: rather than a node $v$ having the four children $\wrh$,
$\wrl$, $\wim$, and $\wna$, corresponding to high-real, low-real, and imaginary proposals to $d$, and to ``no action'',
it will have children $\wrl(d)$, $\wim(d)$ for each $d\in I'$, corresponding to real and imaginary proposals to $d\in I'$, and it will also have a child  $\wna$ corresponding to ``no action''. At these children, the goal will be to bound the probability that the number of doctors in $I'$ receiving real proposals is bounded by, respectively, $r-1$, $r$, and $r$. 
The third change is that the probabilities of the paths in $T$ with $q$ and $\qtilde$ will differ.
But at the root, the probabilities sum to 1 in both cases, so having $\qtilde(\treeroot)\ge q(\treeroot)$ allows us to proceed as before.

The base case, the case of a node with a single child, and case 2 are unchanged.
We give a new proof for the remaining case, namely case 1.

\smallskip\noindent
\emph{Case 1.} $u(h,v)$ is among the smallest $s-kx-y$ residual utilities at node $v$\\
This immediately implies that $u(h,\wna)$ is among the smallest $s-kx-y$ residual utilities at $\wna$, as $u(h,\wna)<u(h,v)$, for the residual utilities for the other hospitals are unchanged at $\wna$; we also note that they are unchanged at the other children.

Again, we consider the random choices that are made in evaluating $\qtilde(v)$,
by instantiating exactly the randomness needed to select a child $w$ of $v$.
As before, $\qtilde(v)=\sum_{\text{$w$ a child of $v$}} \ptilde(w)\cdot \qtilde(w)$,
where $\ptilde(w)$ is the probability that the edge to $w$ is taken.

Now, $\ptilde(\wna)=p(\wna)$ as this probability depends only on the decrease in $h$'s current utility.
Also, for all $d\in I'$, $\ptilde(\wrl(d)) \le p(\wrl(d))$: for the edge is real in the $\qtilde$ setting with probability
$\tau$; this value is computed assuming the cone sizes for all $d\in I'$ are as large as possible;
this only reduces the probability of the edge being real.
Therefore, we can define $\ptilde(\wim(d))=p(\wim(d))+p(\wrl(d))-\ptilde(\wrl(d))$ (for on all the paths to nodes $\wim(d)$, $h$'s computation is terminated, which implies that the subtrees at each node
$\wim(d)$ are isomorphic,  meaning that all that matters is the total probability weight assigned to these trees, and not how the probability weight is distributed among them, or equivalently, among
the edges to the nodes $\wim(d)$).

In addition, $\qtilde(\wrl(d))\le \qtilde(\wim(d))$. To see this, note that the bad event captured by
$\qtilde(\wrl(d))$ is having proposals to $r-(x+1)$ or fewer doctors in $I'$ and the bad event captured by
$\qtilde(\wim(d))$ is having proposals to $r-x$ or fewer doctors in $I'$. But $\wim(d)$ has all the proposers
present in $\wrl(d)$ plus up to another $k$ in addition, who have edges to the same one doctor $d'$ in $I'$. So whenever the random choices result in at most $r-(x+1)$ doctors receiving proposals at $\wrl(d)$, the same random choices at $\wim(d)$ result in at most $r-(x+1)$ doctors receiving proposals plus, in addition, $d$' possibly receiving  one or more proposals, for a total of at most $r-x$ doctors
receiving proposals.

Now, we deduce our result with the help of a little algebra.
\begin{align*}
    &\sum_{d\in I'}\big[\ptilde(\wim(d))\cdot \qtilde(\wim(d)) + \ptilde(\wrl(d))\cdot \qtilde(\wrl(d)) \big]\\
    &\hspace*{0.3in} =   \sum_{d\in I'}\big[p(\wim(d))\qtilde(\wim(d)) + p(\wrl(d))\qtilde(\wrl(d))\big] + \big[\ptilde(\wim(d))-p(\wim(d))\big]\cdot \big[\qtilde(\wim(d))-\qtilde(\wrl(d))\big]\\
    &\hspace*{0.3in} \ge \sum_{d\in I'}\big[p(\wrl(d))q(\wrl(d)) + p(\wim(d))q(\wim(d))\big].
\end{align*}
\end{proof}
}

We defer to the appendix the claims that the surplus $s\ge \alpha n/\kappa$, the probability that the number of unmatched doctors is more than
    $3|I|\cdot \exp\big(-\frac{\alpha k}{4(4a+1)}\big)$ is at most $n^{-(c+2)}$,
    and that a suitably defined $\qtilde$ and $T$ satisfy $\qtilde(v)\ge q(v)$ for all
    nodes $v\in T$.

\hide{
\begin{claim}\label{qtilde-bound-at-root-hosp-to-doc-int}
Let $I=[f,g)$, and suppose that $s\ge \alpha n/\kappa$, 
$6\exp\big(\frac{\alpha k}{4(4a+1)}\big) \cdot (c+2)\frac{\ln n}{n} \le g-f \le \min\big\{ \frac {(2a+\frac12)\alpha}{4\kappa k},~ \frac {\alpha}{2}\big\}$.
Also, suppose that the following events do not occur: $\Bcol$, $\Bdsf(I)$, and $\Bdsm(I)$.
Then the probability that the number of unmatched doctors is more than
    $3|I|\cdot \exp\big(-\frac{\alpha k}{4(4a+1)}\big)$ is at most $n^{-(c+2)}$.
\end{claim}
\begin{proof}
We seek to identify as small an $r$ as possible such that $\qtilde(\treeroot(T))\le n^{-(c+2)}$,
for we can then deduce that $q(\treeroot(T))\le n^{-(c+2)}$ for this value of $r$.
The remainder of the analysis concerns $\qtilde(\treeroot(T))$.

In the $\qtilde(\treeroot(T))$ setting, $s\ge \alpha n/\kappa$ hospitals each seek to propose to some unspecified doctor in $I'$ with probability at least
\begin{align*}
[\alpha-(g-f)]\cdot \Big[1-\big(1-\frac 1{(2a+\frac12)\alpha n/\kappa}\big)^{|I'|\cdot k}\Big]
& \ge \frac{\alpha}{2}\cdot \frac {|I'| k}{(2a+\frac12)\alpha n/\kappa}
     - \frac{\alpha}{2}\cdot \Big(\frac {|I'| k}{2(2a+\frac12)\alpha n/\kappa}\Big)^2\\
& \ge \frac{\alpha}{4}\cdot \frac {|I'| k}{(2a+\frac12)\alpha n/\kappa},
\end{align*}
using $g-f\le \frac {\alpha}{2}$ and $\frac {|I'| k}{(2a+\frac12)\alpha n/\kappa}\le \frac 12$;
as $\Bdsm(I)$ does not occur, $|I'|\le|I|\le 2(g-f)n$, and then the latter condition holds if $\frac{2(g-f)\kappa k}{(2a+\frac12)\alpha}\le \frac 12$.

Thus the expected number of proposals to a single doctor $d$ in $I'$ is at least
$\frac{\alpha k}{2(4a+1)}$.
By a Chernoff bound, $d$ receives no proposals with probability at most
$\exp\big(-\frac12 \frac{\alpha k}{2(4a+1)} \big)$.
Let $X_d$ be the 0/1 random variable that equals 1 if $d$ receives no proposals.
The $X_h$ are negatively correlated and therefore we can apply Chernoff bounds to their sum.
In expectation, the sum of the $X_h$ is at most
$|I'|\cdot \exp\big(-\frac{\alpha k}{4(4a+1)}\big)$, and by a Chernoff bound, it is more than
$2|I'|\cdot \exp\big(-\frac{\alpha k}{4(4a+1)}\big)$
with probability at most $\exp\big(-\frac 23 |I'|\cdot \exp\big(-\frac{\alpha k}{4(4a+1)}\big)\big)\le n^{-(c+2)}$, if $|I'| \ge \frac 32 \exp\big(\frac{\alpha k}{4(4a+1)}\big) \cdot (c+2)\ln n$.
If $\Bcol$ and $\Bdsf(I)$ do not occur, and if $\exp\big(-\alpha k/4(4a+1)\big)\le \frac12$, then $|I'|\ge |I|\big[1-\exp\big(-\alpha k/4(4a+1)\big)\big]\ge \frac 12|I|\ge \frac 14 (g-f)\frac{n}{\kappa}$;
then $g-f \ge 6\exp\big(\frac{\alpha k}{4(4a+1)}\big) \cdot (c+2)\frac{\ln n}{n}$ suffices.  

On setting $r=2|I'|\cdot \exp\big(-\frac{\alpha k}{4(4a+1)}\big)$, we deduce that at most
$2|I'|\exp\big(-\frac{\alpha k}{4(4a+1)}\big)$ doctors in $|I'|$ are unmatched, with failure probability
at most $n^{-(c+2)}$. As $\Bcol$ does not occur, we know that $|I|-|I'| \le |I|\exp\big(-\frac{\alpha k}{4(4a+1)}\big)$, from which our result follows.
\end{proof}

For the next claim, the following additional notation will be helpful.
$J=[g+(a+1)\alpha,1)\cup [g-a\alpha,f+a\alpha)$ is the set of participating hospitals excluding those in $[g+a\alpha,g+(a+1)\alpha)$,
and $K=[g-\alpha,1)\setminus I$ is the set of participating doctors excluding those in $I$.

\begin{claim}\label{clm::surplus-interval-hosp-prop}
    Suppose that none of the following events occur: 
    $\Bdsm(I)$, $\Bhbf(J)$, $\Bhbm(K)$ (defined in the appendix).
    Then the surplus $s\ge \alpha n/\kappa$, if $\alpha\cdot\exp\big(\alpha k/4(4a+1)\big)\ge 3$,
    $g-f\le \frac32 a\alpha/\kappa k$, 
    and $a\ge 5$.
\end{claim}
\begin{proof}
We need to consider two cases, depending on whether the span of the cone for some doctor in $I$  overlaps the range $[1-\alpha,1)$, or in other words whether or not $g\le 1-(a+1)\alpha$.
\\
    \emph{Case 1}. $g\le 1-(a+1)\alpha$.\\
        As $\Bhbf(J)$ does not occur, $J$ contains at least $\big[1-g-(a+1)\alpha)+(2a\alpha- [g-f]) -\frac 12\alpha\big]\cdot \frac{n}{\kappa}= \big[(1-g) +(a-\frac32)\alpha -(g-f)\big]\cdot \frac{n}{\kappa}$ hospitals.
        By assumption, at most a fraction $3\cdot \exp\big(-\frac{\alpha k}{4(4a+1)}\big)$ of the hospitals in $[g+(a+1)\alpha,1)$ are not fully matched.
        % (strictly, the fraction in a minimal set of intervals covering $[g+a\alpha,1)$).
        By \Cref{clm::hosp-removal-lots-edges}, the number of hospitals that are eliminated is at most $|I|k\exp\big(-\alpha k/4(4a+1)\big)\le 2(g-f)kn\exp\big(-\alpha k/4(4a+1)\big)$, as $\Bdsm(I)$ does not occur; we want this to be bounded by $3a\alpha \frac{n}{\kappa}\exp\big(-\alpha k/4(4a+1)\big)$, which holds
        if $g-f\le \frac32 a\alpha/\kappa k$.
        Then, the number of eliminated hospitals in the intervals
        $[g-a\alpha,f+a\alpha)\cup[g+(a+1)\alpha,1)$ is at most $[1-(g-a\alpha)]\frac{n}{\kappa}\cdot 3\exp\big(-\alpha k/4(4a+1)\big)\le \alpha \frac{n}{\kappa}$, if $3\le \alpha \exp\big(\alpha k/4(4a+1)\big)$.
        
        As $\Bdbm(K)$ does not occur, there are at most $[1-g+\frac32\alpha-(g-f)]n$ participating doctors outside of $I$.
        Therefore, the number of fully matched hospitals in $[g-a\alpha,f+a\alpha)$ is at least 
    $\Big(\big[1-g)+(a-\frac 32)\alpha- (g-f)\big]- \alpha -\big[1-g+\frac32\alpha-(g-f)\big]\Big)\cdot \frac{n}{\kappa}\ge (a-4)\frac{\alpha n}{\kappa}\ge \frac{\alpha n}{\kappa}$.
            \\
    \emph{Case 2}. $g> 1-(a+1)\alpha$.\\
    As in Case 1, $K$ contains at most $\big[1-g+\frac32\alpha-(g-f)\big]n\le \big[(a+\frac52)\alpha -(g-f)\big]n$ doctors.
     Now, $J=[g-a\alpha,f+a\alpha)$.
    Similarly to Case 1, the number of hospitals in $[g-a\alpha,f+a\alpha)$ that are available for matching
    is at least $\big[(2a-\frac32)\alpha-(g-f)\big]\cdot\frac {n}{\kappa}$.
    So the surplus is at least
    $\big(\big[(2a-\frac52)\alpha-(g-f)\big] - \big[(a+\frac32)\alpha -(g-f)\big] \big)\cdot\frac {n}{\kappa}
    \ge (a-4)\frac {\alpha n}{\kappa}\ge \frac {\alpha n}{\kappa}$.
    \end{proof}
    }

\hide{\begin{claim}\label{clm::hosp-prop-interval-constraints}
    The conditions in Claims~\ref{clm::hosp-removal-lots-edges}--\Cref{clm::surplus-interval-hosp-prop} amount to the following constraints:
    \begin{align*}
        \alpha\cdot \exp\Big(\frac {\alpha k}{4(4a+1)}\Big)&\ge 3~~~~(\Cref{clm::surplus-interval-hosp-prop})\\
        a&\ge 5~~~~(\Cref{clm::surplus-interval-hosp-prop})
   %     n&\ge \frac {e(|I|k\kappa)^2}{2\tildec[(a-\frac12)\alpha]^2}~~~~(\Cref{clm::hosp-removal-lots-edges})
    \end{align*}
    and several constraints on $g-f$, namely:
    \begin{align*}
       & 
        6(c+2)\exp\Big(\frac{\alpha k}{4(4a+1)}\Big)\cdot\frac{\ln n}{n}
        \le g-f
        \le \min\Big\{\frac{(2a-1)\alpha\cdot\exp\big(-\frac{\alpha k}{4(4a+1)}\big)}{(ek)^2\kappa},~\frac{\alpha}{2},~\frac{(4a+1)\alpha}{8\kappa k},~\frac{3a\alpha}{2\kappa k}\Big\}\\
       & \hspace*{2in}(\text{resp.\ Claims \ref{clm::hosp-removal-lots-edges} and \ref{qtilde-bound-at-root-hosp-to-doc-int}, \ref{clm::hosp-removal-lots-edges}, \ref{qtilde-bound-at-root-hosp-to-doc-int}, \ref{qtilde-bound-at-root-hosp-to-doc-int}, \ref{clm::surplus-interval-hosp-prop}}).
    \end{align*}
    In addition, over the whole induction, they exclude events with total probability at most $\big( \frac{6}{g-f} + \frac{n}{\kappa}\big)\cdot n^{-(c+2)}$.
\end{claim}
\begin{proof}
By inspection, 
the excluded events in \Cref{clm::hosp-removal-lots-edges} have probability at most $\big(\frac{n}{g-f}+\frac{n}{\kappa}\big)\cdot n^{-(c+2)}$ and it has failure probability at most $\frac{1}{g-f}\cdot n^{-(c+2)}$;
the additional excluded events in \Cref{qtilde-bound-at-root-hosp-to-doc-int} have probability at most
$\frac{1}{g-f}\cdot n^{-(c+2)}$ and this claim has failure probability at most $\frac {1}{g-f}\cdot n^{-(c+2)}$;  
the additional excluded events in \Cref{clm::surplus-interval-hosp-prop} have probability at most $\frac{2}{g-f} \cdot n^{-(c+2)}$. The bound on the probability of excluded events follows readily.
\end{proof}
}





\hide{
\subsection{Proof of \Cref{lem::hospitals-interval-non-match}}

$I=[f,g)$ is an interval of hospitals here. We define $L=[g-a\alpha,f+a\alpha)$ to be the interval of doctors that are in-cone for all hospitals in $I$. We want to ensure that there are a sufficient number
of potential proposals from $L$ that are uniform over $I$ w.r.t.\ the interview values. Suppose that we guarantee, with failure probability at most $n^{-(c+2)}$, that the doctors' proposals all have private value at least $1-\taubar$ (which we bound in \Cref{clm::value-of-taubar}, below) and utility at least $f+2-\alpha$. This yields a set $P$ of $[\alpha-\taubar-(g-f)]\cdot|L|$ such proposals in expectation, and at least
$\frac12 [\alpha-\taubar-(g-f)]\cdot|L|$ with high probability. Then we will seek to count how many hospitals in $I$ receive at least $\kappa$ proposals from the proposals in $P$ and show that this count is sufficiently large with
high probability. Similarly to the hospital removal in \Cref{sec::doc-int-idio-no-match}, we will remove all doctors that have two or more edges to hospitals in $I$.
The next lemma bounds the number of removed doctors.

\begin{claim}\label{clm::doc-removal-lots-edges}
Suppose that the following events do not occur: $\Bhsf(I)$, $\Bhsm(I)$, $\Bdbm(L)$, $\Bdbf(L)$, and $\Bhbf(C(d))$ for all $d$ in $L$.
Then at most $|L|\exp\big(-\alpha k/4(4a+1)\big)$ doctors are removed because they have two or more edges to hospitals in $I$, 
with failure probability at most $n^{-(c+2)}$, if 
$2(c+2)\exp\big(\alpha k/4(4a+1)\big)\cdot \frac{\ln n}{n}\le (g-f)\le \frac{4(a-\frac12)^2\alpha }{(2a+\frac12)\cdot(e\kappa k)^2}\cdot\exp\big(-\alpha k/4(4a+1)\big)$.
% and $(a-\frac12)\alpha \exp\big(-\alpha k/4(4a+1)\big)\ge (c+2)\cdot \frac{\ln n}{n}$.
\end{claim}
\begin{proof}
Let $d$ be a doctor in $L$, the intersection of the cones for hospitals in $I$.
The probability that an edge from $d$ is to a hospital in $I$ is at most $|I|/[(a-\frac12)\cdot(\alpha n/\kappa)]$, as $\Bhbf(C(d))$ does not occur for any doctor in $I$'s cone. Therefore the probability that $d$ has two or more edges to $I$ is at most
$\frac12 k^2 \cdot \Big[\frac{|I|}{(a-\frac12)\cdot(\alpha n/\kappa)}\Big]^2$.
% $\le 2\Big[\frac{k(g-f)\kappa}{(a-\frac12)\alpha}\Big]^2$, as $\Bdsm(I)$ does not occur.

Therefore the expected number of doctors with two or more edges to $I$ is at most 
$\frac12|L| \cdot \Big[\frac{k|I|\kappa}{(a-\frac12)\alpha n}\Big]^2$.
Note that $|L|\le (2a+\frac12)\alpha n$, as $\Bdbm(L)$ does not occur.
By a Chernoff bound, there are more than $|I|\exp\big(-\alpha k/4(4a+1)\big)$ such doctors with probability at most 
\begin{align*}
    \Big[\frac{(2a+\frac12)e|I|(\kappa k)^2\exp\big(\alpha k/4(4a+1)\big)}{2(a-\frac12)^2\alpha n}\Big]^{|I|\exp\big(-\alpha k/4(4a+1)\big)}.
    \end{align*}
    This is maximized when $|I|$ is as small as possible, i.e.\ $\frac12 (g-f)\frac{n}{\kappa}$, as $\Bhsf(I)$ does not occur; so it is at most
\begin{align*}
    \Big[\frac{(2a+\frac12)e[(g-f)(\kappa k)^2\exp\big(\alpha k/4(4a+1)\big)}{4(a-\frac12)^2\alpha}\Big]^{\frac12 (g-f) n\exp\big(-\alpha k/4(4a+1)\big)}.
\end{align*}
This is bounded by $n^{-(c+2)}$ if
$(g-f)\le \frac{4(a-\frac12)^2\alpha }{(2a+\frac12)\cdot(e\kappa k)^2}\cdot\exp\big(-\alpha k/4(4a+1)\big)$ and $g-f\ge 2(c+2)\exp\big(\alpha k/4(4a+1)\big)\cdot \frac{\ln n}{n}$.

Finally, we need $|I|\exp\big(-\alpha k/4(4a+1)\big)\le |L|\exp\big(-\alpha k/4(4a+1)\big)$.
Assuming $\Bhsm(I)$ and $\Bdbf(L)$ do not occur, it suffices that
$2(g-f)n\ge (a-\frac12)\alpha n$, i.e.\ $g-f\le (2a-1)\alpha$, and this is subsumed by the first lower bound on $g-f$.
\end{proof}
Let $L'$ be the set of doctors remaining after the removals from $L$, and left
$\Bdrem$ be the event that more than $|L|\exp\big(-\alpha k/4(4a+1)\big)/(e^2 \kappa)$ doctors are removed for any of the intervals $L$ that occur in the analysis.
Going forward, we suppose that $\Bdrem$ does not occur.

We suppose the event $\Btau$, that some doctor fails to have $k$ edges with private value $1-\taubar$ or larger does not occur, as specified in \Cref{clm::value-of-taubar}.

The proof that $\qtilde(v)\ge q(v)$ needs some modifications.
Again the possible runs of the double-cut DA will use some additional stops.
Doctors with two or more edges to $I$ are eliminated.
Of the remaining doctors with a single edge to $I$, if it provides utility in the range
$[f+2-\alpha,g+2-\alpha)\cup [f+2-\taubar,g+2)$ we do not include the proposal to $I$ in our count of proposals. This ensures that for the remaining doctors with a proposal to $I$, the receiving
hospital is uniformly distributed over $I$.

As in \Cref{sec::doc-int-idio-no-match}, the tree $T$ of possible runs of the double-cut DA has
both real and imaginary proposals. For each doctor $d$ outside $L'$ we fix the utilities.
Also, for each doctor $d$ in $L'$, we fix its top $k$ value utilities, but without specifying which edges these values are attached to.
Now, we are seeking the probability that the doctors in $L'$ make at most $r$ proposals to hospitals in $I$ for an $r$ to be specified later; in addition, we want to show that $\qtilde(v) \ge q(v)$ for all nodes $v$ in $T$, and for $\treeroot(T)$ in particular.

A node corresponding to an action by a doctor outside $L'$ has just one outgoing edge corresponding to its single possible action. For a doctor $d$ in $L'$, we proceed as in \Cref{sec::proof-hosp-match-prob}.
We consider the edges out of $d$ one at a time.
the decision making corresponding to one edge proceeds in two steps:
first, whether it has a utility equal to $d$'s current utility value in tree $T$. This is a decision based on making a random choice for its interview value. For each possible destination of this edge, this occurs with the same probability. 
In the $q$ setting, we then choose the edge uniformly from the hospitals in $d$'s current cone that she has not already proposed to; in this setting, there are no imaginary proposals.
A doctor stops making proposals either when she has gone through all $k$ of her proposals or she makes a proposal to a hospital in $I$.

In the $\qtilde$ setting, we keep track of how many proposals a doctor has made.
Again, as soon as a doctor makes a proposal, real or imaginary, to a hospital in $I$, she stops.
We keep track of how many proposals a doctor has made; let $k(d,v)$ be the number of remaining
proposals for doctor $d$ at node $v$. Also, recall that $u(d,v)$ is her residual probability at node $v$.
the doctors with the smallest products $u(d,v)\cdot k(d,v)$ will attempt to propose; each real proposal will occur with the same probability, which will be no larger than the probability of a proposal in the $q$ setting; the difference in probability will be handled by making proposals imaginary with probability equal to the difference. Now, we make this precise.

We use the same value for the probability that $d$ has a proposal with the current utility $u$ as in the $q$ setting. 
If $d$ is determined to have such a proposal, uniformly at random, we choose one of the hospitals in $d$'s current cone that has not already received a proposal from $d$ to receive the proposal; then we choose whether it is real with probability $\tau=1 -\big(1 - \frac {1}{(2a+\frac12)\alpha n}\big)^{k(d,v)}$.
As in \Cref{sec::doc-int-idio-no-match}, $\tildep(\wrl(h))\le p(\wrl(h)$; again, we choose
$\tildep(\wim(h))=p(\wim(h))+[\wrl(h))-\tildep(\wrl(h)]$.

Again, let $x$ be the number of hospitals in $I'$ that have received real proposals.
At node $v$, we will be seeking the probability that at most an additional $r-x$ real proposals are made to hospitals in $I'$.

\begin{claim}\label{clm::qtilde-larger-for-intervals-in-hosp-prop}
    $\qtilde(v)\ge q(v)$ for all $v$ in $T$.
\end{claim}
\begin{proof}
    The base case argument and case 2 are unchanged from \Cref{clm::qtilde-bound-for-hosp-doc-int}.

    \smallskip\noindent
    The proposal is to some $h\notin I'$\\
    Then $v$ has two children $\wrl$, $\wim$.
    Here $k(d,w)=k(d,v)-1$ and $u(d,w)<u(d,v)$, for $w=\wrl,\wim$; the variables associated with the other doctors are unchanged. At both children, we still seek the probability that at most $r-x$ more real proposals are made to hospitals in $I$. As in \Cref{sec::doc-int-idio-no-match}, 
    $\ptilde(\wrl)\le p(\wrl)$ and $\qtilde(\wrl)\ge \qtilde(\wim)$. It follows that $ p(\wrl)\cdot \qtilde(\wrl) + p(\wim)\cdot \qtilde(\wim)\ge \ptilde(\wrl)\cdot \qtilde(\wrl) + \ptilde(\wim)\cdot \qtilde(\wim)$, proving the inductive hypothesis in this case.

    \smallskip\noindent
    The proposal is to some $h\in I'$\\
    Then $v$ has two children $\wrl(h)$ and $\wim(h)$, for each $h\in I'$, plus the child $\wna$.

     \smallskip\noindent
     \emph{Case 1}. $u(d,v)\cdot k(d,v)$, the proposal probability for $h\in I'$ at node $v$, is among the $s-x-y$ smallest proposal probabilities, $u_1k_1\le uk_2\le\ldots\le u_{s-x-y}k_{s-x-y}$, at node $v$. \\
     Since only $u(d,w)$ and $k(d,w)$ change (by becoming smaller) at any of $v$'s children $w$, the proposal probability for $d$ continues to be among the $s-x-y$ smallest at the children where it is still in use. Therefore instantiating the randomness needed to choose to edge to a child of $v$ ensures that $\qtilde(v)= \sum_{\text{$w$ a child of $v$}} \ptilde(w)\cdot \qtilde(w)\ge \sum_{\text{$w$ a child of $v$}} p(w)\cdot \qtilde(w)$, as for each pair of nodes $\wrl(h)$ and $\wim(h)$, we have $ p(\wrl)\cdot \qtilde(\wrl) + p(\wim)\cdot \qtilde(\wim)\ge +\ptilde(\wrl)\cdot \qtilde(\wrl) + \ptilde(\wim)\cdot \qtilde(\wim)$, and $\ptilde(\wna)=p(\wna)$.
\end{proof}





For the next claim, which bounds the surplus, the following additional notation will be helpful.
$J=[g+(a+1)\alpha,1)\cup [g-a\alpha,f+a\alpha)$ is the set of participating doctors minus those in $[g+a\alpha,g+(a+1)\alpha)$,
and $K=[g-\alpha,1)\setminus I$ is the set of participating hospitals excluding those in $I$.
   
\begin{claim}\label{clm::surplus-interval-doc-prop}
Suppose that neither of the following events occurs: $\Bdbf(J)$, $\Bhbm(K)$.
    Then the surplus $s\ge \alpha n$, if $\alpha\cdot\exp\big(\alpha k/4(4a+1)\big)\ge 3$, and $a\ge 5$.
\end{claim}
\begin{proof}
We need to consider two cases, depending on whether the span of the cone for some doctor in $I$ has  overlaps the range $[1-\alpha,1)$.
\\
    \emph{Case 1}. $g\le 1-(a+1)\alpha$.\\
        As $\Bdbf(J)$ does not occur, $J$ contains at least $\big[1-g-(a+1)\alpha)+(2a\alpha- [g-f]) -\frac 12\alpha\big]n= \big[(1-g) +(a-\frac32)\alpha -(g-f)\big]n$ doctors.
        By assumption, at most a fraction $3\cdot \exp\big(-\frac{\alpha k}{4(4a+1)}\big)$ of the doctors in $[g+(a+1)\alpha,1)$ are not fully matched.
        % (strictly, the fraction in a minimal set of intervals covering $[g+a\alpha,1)$).
        By \Cref{clm::doc-removal-lots-edges}, the number of doctors in $L$ that are eliminated is at most $|L|\exp\big(-\alpha k/4(4a+1)\big)$.

        Thus the number of doctors remaining is at least $\big[(1-g) +(a-\frac32)\alpha -(g-f)\big]n\cdot \big[1 -3\cdot \exp\big(-\frac{\alpha k}{4(4a+1)}\big)\big] \ge \big[(1-g) +(a-\frac52)\alpha -(g-f)\big]n$, as $\exp\big(-\alpha k/4(4a+1)\big)\le \frac 13 \alpha$.
              
        As $\Bhbm(K)$ does not occur, there are at most $[1-g+\frac52\alpha-(g-f)]\frac{n}{\kappa}$ participating hospitals outside of $I$.
        Therefore, the surplus, the number of doctors in $[g-a\alpha,f+a\alpha)$ not matched to $K$,
        is at least 
    $\big(\big[1-g)+(a-\frac32)\alpha-(g-f)\big] -\big[1-g+\frac52\alpha-(g-f)\big]\big)n\ge (a-4)\alpha n\ge \alpha n$.
            \\
    \emph{Case 2}. $g> 1-a\alpha$.\\
    As in Case 1, $K$ contains at most $\big[1-g+\frac52\alpha-(g-f)\big]n\le \big[(a+\frac52)\alpha -(g-f)\big]\cdot \frac{n}{\kappa}$ hospitals.
     Now, $J=[g-a\alpha,f+a\alpha)$.
    Similarly to Case 1, the number of doctors in $[g-a\alpha,f+a\alpha)$ that are available for matching
    is at least $\big[(2a-\frac32)\alpha-(g-f)\big]n$.
    So the surplus is at least
    $\big(\big[(2a-\frac52)\alpha-(g-f)\big] - \big[(a+\frac32)\alpha -(g-f)\big] \big)\cdot\frac {n}{\kappa}
    \ge (a-4)\frac \alpha n\ge \alpha n$.
\end{proof}

\begin{claim}\label{qtilde-bound-at-root-doc-to-hosp-int}
Let $I=[f,g)$, and suppose that $s\ge \alpha n$, 
$g-f \ge 3\exp\big(\frac{\alpha\kappa k}{4(4a+1)}\big) \cdot (c+2)\frac{\ln n}{n}$,
$g-f+\taubar\le \frac {\alpha}{2}$, $\alpha k\ge 8(4a+1)$, and $\frac {\kappa k}{(2a+\frac12)\alpha n}\le 1$.
Also, suppose that $\Bhsf(I)$ not occur.
Then the probability that the number of not fully matched hospitals is more than
    $3|I|\cdot \exp\big(-\frac{\alpha\kappa k}{4(4a+1)}\big)$ is at most $2n^{-(c+2)}$.
\end{claim}
\begin{proof}
We seek to identify as small an $r$ as possible such that $\qtilde(\treeroot(T))\le n^{-(c+2)}$,
for we can then deduce that $q(\treeroot(T))\le n^{-(c+2)}$ for this value of $r$.

In the $\qtilde(\treeroot(T))$ setting, $s\ge \alpha n$ doctors each seek to propose to an arbitrary  hospital $h$ in $I$ with probability at least
\begin{align*}
[\alpha-(g-f)-\taubar]\cdot \Big[1-\big(1-\frac {1}{(2a+\frac12)\alpha n/\kappa}\big)^{k}\Big]
& \ge \frac{\alpha}{2}\cdot \frac {\kappa k}{(2a+\frac12)\alpha n}
     - \frac{\alpha}{4}\cdot \Big(\frac {\kappa k}{(2a+\frac12)\alpha n}\Big)^2\\
& \ge \frac{\alpha}{2}\cdot \frac {\kappa k}{(4a+1)\alpha n},
\end{align*}
using $g-f+\taubar\le \frac {\alpha}{2}$ and $\frac {\kappa k}{(2a+\frac12)\alpha n}\le 1$.

In expectation, the hospitals in $I$ receives at least $|I|\cdot\frac{\alpha\kappa k}{2(4a+1)}$ proposals. 
By a Chernoff bound, $I$ receives fewer than $\frac 12 |I|\cdot\frac{\alpha\kappa k}{2(4a+1)}$ proposals with probability at most
$\exp\big(- \frac{|I|\alpha\kappa k}{16(4a+1)} \big)\le n^{-(c+2)}$,
if $|I|\alpha\kappa k \ge 16(4a+1)\cdot(c+2)\ln n$. 
As $\Bhsf(I)$ does not occur, $|I|\ge \frac 12 (g-f)\frac{n}{\kappa}$,
and so $g-f\ge \frac{32(4a+1)}{\alpha k}\cdot(c+2)\frac {\ln n}{n}$ suffices.
We set $r+1=  |I|\cdot\frac{\alpha\kappa k}{4(4a+1)}$.
So we know there are this many proposals to $I$ in run of the double-cut DA with failure probability at most $n^{-(c+2)}$,
and furthermore each proposal is uniform over $I$.
We now analyze how many hospitals in $I$ receive fewer than $\kappa$ proposals.

Let $X_h$ be the 0/1 random variable that equals 1 if $h$ receives fewer than $\kappa$ proposals.
The $X_h$ are negatively correlated and therefore we can apply Chernoff bounds to their sum.
In expectation, the sum of the $X_h$ is at most
$|I|\cdot \exp\big(-\frac{\alpha\kappa k}{4(4a+1)}\big)$, and by a Chernoff bound, it is more than
$2|I|\cdot \exp\big(-\frac{\alpha\kappa k}{4(4a+1)}\big)$
with probability at most $\exp\big(-\frac 23 |I|\cdot \exp\big(-\frac{\alpha\kappa k}{4(4a+1)}\big)\le n^{-(c+2)}$, if $|I| \ge \frac 32 \exp\big(\frac{\alpha\kappa k}{4(4a+1)}\big) \cdot (c+2)\ln n$.
As $\Bhsf(I)$ does not occur, $|I|\ge \frac 12 (g-f)\frac{n}{\kappa}$,
so $g-f \ge 3\exp\big(\frac{\alpha\kappa k}{4(4a+1)}\big) \cdot (c+2)\frac{\kappa\ln n}{n}$ suffices.

Finally, looking at the two lower bounds on $g-f$, the second one dominates so long as $\alpha k\ge 8(4a+1)$.
\end{proof}

\begin{claim}\label{clm::doc-prop-interval-constraints}
    The conditions in Claims~\ref{clm::doc-removal-lots-edges}--\Cref{qtilde-bound-at-root-doc-to-hosp-int} amount to the following constraints:
    \begin{align*}
        \alpha\cdot \exp\Big(\frac {\alpha\kappa k}{4(4a+1)}\Big)&\ge 3~~~~(\Cref{clm::surplus-interval-doc-prop})\\
        a&\ge 5~~~~(\Cref{clm::surplus-interval-doc-prop})\\
        \taubar &\ge \frac{b\kappa}{(a-\frac12)\alpha}\cdot(c+2)\cdot\frac {\ln n}{n}~~~~(\Cref{clm::value-of-taubar})\\
        b& >2~~~~(\Cref{clm::value-of-taubar})\\
        k &\le \Big[1 -\Big(\frac 2b\Big)^{1/2}\Big]\cdot b(c+2)\ln n~~~~(\Cref{clm::value-of-taubar})\\
        \alpha n &\ge \frac{\kappa k}{2a+\frac12}~~~~(\Cref{qtilde-bound-at-root-doc-to-hosp-int})\\
        \alpha k &\ge 8(4a+1)~~~~(\Cref{qtilde-bound-at-root-doc-to-hosp-int})
    \end{align*}
    and several constraints on $g-f$, namely:
    \begin{align*}
       & 
        3\exp\Big(\frac{\alpha\kappa k}{4(4a+1)}\Big)\cdot(c+2)\cdot\frac{\ln n}{n}
        \le g-f ~~~~(\text{Claims \ref{clm::doc-removal-lots-edges} and \ref{qtilde-bound-at-root-doc-to-hosp-int}})\\
        &\hspace*{1in}\le \min\Big\{\frac{\alpha}{2}-\taubar,
        ~\frac{(2a-1)^2\alpha\cdot\exp\big(-\frac{(\alpha k}{4(4a+1)}\big)}{(2a+\frac12)\cdot(e\kappa k)^2} \Big\}\\
       & \hspace*{2in}(\text{resp.\ Claims \ref{qtilde-bound-at-root-doc-to-hosp-int}, \ref{clm::doc-removal-lots-edges}}).
    \end{align*}
    In addition, over the whole induction, they exclude events with total probability at most $\big(2n+ \frac{10}{g-f}\big)\cdot n^{-(c+2)}$.
\end{claim}
\begin{proof}
    By inspection, 
the excluded events in \Cref{clm::doc-removal-lots-edges} have probability at most $\big(n+\frac{4}{g-f}\big)\cdot n^{-(c+2)}$ and it has failure probability at most $\frac{1}{g-f}\cdot n^{-(c+2)}$;
there are no additional excluded events in \Cref{clm::value-of-taubar} and it has failure probability at most $n\cdot n^{-(c+2)}$;
the additional excluded events in \Cref{clm::surplus-interval-doc-prop} have probability at most
$\frac{2}{g-f}\cdot n^{-(c+2)}$ and this claim has failure probability at most $\frac {1}{g-f}\cdot n^{-(c+2)}$; 
there are no additional excluded events in \Cref{qtilde-bound-at-root-doc-to-hosp-int} and this claim has failure probability at most $\frac {2}{g-f}\cdot n^{-(c+2)}$;  
 The bound on the probability of excluded events follows readily.
\end{proof}
}

\hide{
\subsection{The Outcome for the bottommost Agents}\label{sec:bottom-agent-outcomes-idio-case}

Consider running the doctor-proposing DA, for now excluding the bottommost doctors, i.e.\ those with
public rating less than $a\alpha$. Furthermore, let's start by cutting at hospital public rating
$(2a-1)\alpha$. From the prior analysis, we know that all but a small fraction of the hospitals
with public rating $2a\alpha$ or larger are fully matched (see \Cref{lem::hospitals-interval-non-match}).
Now continue the run of DA, cutting at hospital public rating $a\alpha$. This ensures that all but a small fraction of the doctors with public rating $2a\alpha$ or larger are matched, as we justify below.

The behavior of the currently unmatched doctors with public rating less than $2a\alpha$ somewhat resembles what happens in the classic random permutation setting, but the match rate is not completely uniform; the higher rated doctors will be more successful on average.

\begin{claim}\label{clm::match-rate-near-bottom-doctors}
    In the partial run of the doctor-proposing DA described above, with failure probability at most $n^{-(c+2)}$, at most ... fraction of the doctors with public rating at least $2a\alpha$ remain unmatched.
\end{claim}
\begin{proof}
    Consider the runs of the double-cut hospital proposing DA for the interval including public rating $2a\alpha$ and all higher intervals. By \Cref{lem::doctors-interval-non-match}, at most ... of these doctors remain unmatched. If we expand this run of the hospital proposing DA to include all doctors with public rating at least $a\alpha$, meaning that the cut value is reduced to $a\alpha$, this maintains a match for all doctors that were previously matched, although who they were matched to could change. The set of edges in this partial run of DA is the same set of edges as is being used in the run described in the statement of the claim. As the hospital-proposing DA yields the worst outcome for the doctors among all stable matchings, it implies that the run of the doctor-proposing DA on this set of edges has at least as many doctors matched (actually, it is the same number).
\end{proof}

Approximately, after the partial run of the doctor-proposing DA, the number of unmatched doctors in the range $[a\alpha,2a\alpha)$ equals the number of available hospital places in the same range (up to a factor of $\frac 32a\alpha n$ due to the unmatched doctors above this range, and the possible disparities between the actual and expected number of hospitals and doctors in this range).
}

\subsection{The $\eps$-Nash Equilibrium for all but the Bottommost Doctors}
\label{sec::idio-eps-Nash}

We begin by identifying sufficient conditions to satisfy the constraints in Claims~\ref{clm::conditions-hosp-prop-one-doctor}, \ref{clm::conditions-doctor-prop-one-hosp},
\ref{clm::hosp-prop-interval-constraints}, and \ref{clm::doc-prop-interval-constraints}.

\begin{claim}\label{clm::final-cstrnts-idio}
    With $\delta=0$ and $\alpha=\big(\frac{4(4a+1)\ln k}{k}\big)^{1/2}$, $a=5$, and $b=3$ the following constraints suffice: 
\begin{align*}
                \Omega(1)&\le k \le \frac 12(c+2)\ln n \\
         \frac{n}{\ln n} &=\Omega\Big(\frac{(c+2)k^{2.5}\kappa}{(\ln k)^{1/2}}\exp\big(\Omega\big( (k\ln k)^{1/2}\big)\big)\Big).
    \end{align*}
\end{claim}

\hide{
\begin{claim}\label{clm::idio-constraint-summary}
With $\delta=0$,
    the constraints in Claims~\ref{clm::conditions-hosp-prop-one-doctor}, \ref{clm::conditions-doctor-prop-one-hosp}, \ref{clm::hosp-prop-interval-constraints}, and \ref{clm::doc-prop-interval-constraints} are all satisfied if
    \begin{align}
        a&\ge 5 \notag\\
        b &\ge 3 \notag\\
        3&\le \alpha\cdot\exp\Big(\frac{\alpha k}{4(4a+1)}\Big) \label{eqn::alpha-cstrnt}\\
         \frac{2\sqrt{a}}{e}&\le k \le \Big[1 -\Big(\frac 2b\Big)^{1/2}\Big]\cdot b(c+2)\ln n \notag\\
         \frac{n}{\ln n}& \ge\frac{2b(c+2)\kappa\exp\big(\frac{\alpha\kappa k}{2(4a+1)}\big)}{9(a-\frac12)}. \notag
    \end{align}
\end{claim}
\begin{proof}
We set $\taubar = \frac{b(c+2)\kappa \ln n}{(a-\frac12)\alpha n}$,
and $\frac14\alpha \ge \taubar$,
which yields the constraint $\alpha^2\ge \frac{2b(c+2)\kappa}{(a-\frac12)}\cdot\frac{\ln n}{n}$,
which is subsumed by the first bound on $n/\ln n$ on taking $b=3$ and $\alpha=\big([2a+\frac12] \ln k/k\big)^{1/2}$, if $\frac{n}{\ln n} \ge \frac{2b(c+2)\kappa\exp\big(\frac{\alpha\kappa k}{2(4a+1)}\big)}{9(a-\frac12)}$.
Looking at the upper bound on $g-f$ in \Cref{clm::hosp-prop-interval-constraints}, we see that the first term, $\frac{(2a-1)\alpha\cdot\exp\big(-\frac{\alpha k}{4(4a+1)}\big)}{(ek)^2\kappa}$, is the smallest,
if $k^2\ge \frac{2(2a-1)\exp\big(-\frac{\alpha k}{4(4a+1)}\big)}{e^2\kappa}$; $k\ge 2\sqrt{a}/e$ suffices. Similarly, in \Cref{clm::doc-prop-interval-constraints}, 
the second term in the upper bound on $g-f$, $\frac{(2a-1)^2\alpha\cdot\exp\big(-\frac{\alpha k}{4(4a+1)}\big)}{(2a+\frac12)\cdot(e\kappa k)^2}$, is the smaller,
if $k^2 \ge \frac{4(2a-1)^2\exp\big(-\frac{\alpha k}{4(4a+1)}\big)}{e^2(4a+1)\kappa^2}$;
again $k\ge 2\sqrt{a}/e$ suffices.
Finally, the condition $n \ge \frac {2\kappa k}{(4a+1)\alpha}$ is subsumed by the condition on $n/\ln n$.
\end{proof}
}

\begin{claim}\label{clm::prob-B}
Let ${\mathcal B}$ denote the bad events excluded in Claims~\ref{clm::conditions-hosp-prop-one-doctor}, \ref{clm::conditions-doctor-prop-one-hosp}, \ref{clm::hosp-prop-interval-constraints}, \ref{clm::doc-prop-interval-constraints}.
The probability that ${\mathcal B}$ occurs is at most $12n^{-(c+1)}$.
\end{claim}
\hide{\begin{proof}
    Summing the probabilities of the bad events in these four claims gives a bound of
    $\big(7n+\frac{15}{g-f}+\frac 3n\kappa\big)n^{(-c+2)}\le 11n^{(-c+1)}$, if $g-f\le n/15$.
    \rnote{There may be double counting here. I have not checked.}
\end{proof}
}

Next, we show that for a non-bottommost student, a student with public rating at least $a\alpha$,
changing strategies will not significantly improve her outcome in expectation.


\begin{claim}\label{lem::typical-student-eps-nash}
Suppose the constraints in \Cref{clm::final-cstrnts-idio} hold.
    Let $d$ be a doctor with public rating at least $a\alpha$, and let $\alpha=\big(\frac{4(4a+1)\ln k}{k}\big)^{1/2}$.
        In expectation, ex-ante, $d$ could improve her utility by at most 
        $O(\alpha)=O((\ln k/k)^{1/2})$, if $k\ln k\ge \big(\frac83\big)^2\cdot\frac{4a+1}{\kappa^2}$.
\end{claim}
\begin{proof} (Sketch.)~
Basically, there are two ways in which a doctor could gain expected $O(\alpha)$ utility in principle (but it is not clear such changes in strategy would lead to actual gains).
First, by changing a bid in cone, this might improve the public rating component of the match utility
by up to $2a\alpha$. Second, by changing bids so as to avoid matches with low interview values,
she might improve the match utility when this happens by $O(1)$; but as \Cref{lem::hosp-high-value-match-prob} shows, this is a somewhat uncommon event, with probability at most $\alpha$, yielding an expected gain of $O(\alpha)$. The other gains, from better results when ${\mathcal B}$ occurs and improvements in the private value, are small in comparison. The full proof can be found in the appendix.
\end{proof}




This concludes the proof of \Cref{thm::eps-nash-idio-large-cap}.





==> no-idio-old-text.tex <==

\hide{
In this setting, we suppose there are $n$ students applying to $n/\kappa$ schools,
each of which has $\kappa$ places, which we will also refer to as their \emph{capacity}.

Each student will select $k$ schools to which to apply. The matches will be made by running the
student-proposing DA. The students and schools will order their preference lists based on utilities which we specify next.

Each school and each student has a public rating, a uniform random draw from $[0,1)$. 
The schools will all use the same ordering of students based on the students' public ratings.
There are two common ways in which these arise: due to a lottery, used in multiple school districts in America,
or based on a common entrance exam, used in multiple national university systems, for example in China.

In addition, each student has a private (idiosyncratic) value for each school, again a uniform random draw from $[0,1)$.
Each student will select $k$ schools based on the school's public rating and her private values; we specify exactly how a little later. The student will then collect additional information about these $k$ schools, and obtain a further valuation, also a uniform random draw from $[0,1)$; we call this the interview value.
A student's utility for a particular school is the sum of these three values: the school's public rating, and her private and interview values for the school. She then orders the $k$ chosen schools based on her utilities for these schools.

A stu{\bf d}ent $d$ selects schools according to the following rule. (We use the notation $d$ for schools as later we will be analyzing the doctor-hospital setting, and doctors will be roughly analogous to students.) First, $d$ only considers schools with public ratings in the range $[r(d)-a\alpha,r(d)+a\alpha)$, where $r(d)$ is $d$'s public rating and $a$ and $\alpha$ are parameters we specify later.
We call this range $d$'s \emph{cone}, and denote it by $C(d)$.
Among these schools she selects those with the $k$ largest private values.
Note that because the private values are uniform random draws, we can think of this selection as a uniform random selection of $k$ schools from her cone.

We will show that the outcome, when running the student-proposing DA, is an $\eps$-Nash equilibrium for all but the bottommost students (bottommmost w.r.t.\ their public ratings), with this property unaffected by whether or not the bottommost students follow the recommended strategy.

\begin{theorem} %\label{thm::eps-nash-no-idio-large-cap}
    Suppose that there are $n$ students and $n/\kappa$ schools each with capacity $\kappa$, for $n$ sufficiently large.
    Suppose further that $a = \frac 72$ and 
    $\alpha =2\cdot\frac {4a+1}{k}\cdot\max\big\{1, \frac{(c+2)\ln n}{\kappa}\big\}$.
    Then the outcome when following the specified application process is an $\eps$-Nash equilibrium for all students with public rating at least $a\alpha$, regardless of the strategy that the remaining students use, where $\eps=O\big(\max\big\{\frac 1k,\frac{\ln n}{k\kappa}\big\}\big)$.
\end{theorem}

To carry out the analysis, we will identify some low probability events, \emph{bad events}, for short, denote ${\cal B}$. The remainder of the analysis assumes these bad events do not occur.

This theorem will use three different double-cut DAs to obtain its bounds.
Their outcomes are specified in the next three lemmas.

\begin{lemma}\label{lem::students-interval-non-match}
Let $I=[f,g)$ be a public rating interval.
Suppose the fraction of unmatched schools with public rating in $[g+\alpha,1)$ is at most 
$\alpha \exp\big(-\alpha k/(2a-\frac 12)\big)$ \rnote{may need to modify.}
Also suppose that the event ${\cal B}$ does not occur.
Then the probability that at least $\alpha n \exp\big(-\alpha k/(2a-\frac 12)\big)$ students with public rating in $I$ fail to match
is at most $n^{-(c+2)}$,
if $\alpha n \ge 3(c+2)\ln n \cdot\exp\big(\alpha k/(2a-\frac12)\big)$.
\rnote{Redo prob bound and conditions.}
\end{lemma}

\begin{lemma}\label{lem::schools-interval-non-match}
Let $I=[f,g)$ be a public rating interval.
Suppose the fraction of unmatched schools with public rating in $[g+\alpha,1)$ is at most 
$\alpha \exp\big(-\alpha k/(2a-\frac 12)\big)$ \rnote{may need to modify.}
Also suppose that the event ${\cal B}$ does not occur.
Then the probability that at least $\alpha \cdot \frac n{\kappa} \cdot \exp\big(-\alpha k/(2a-\frac 12)\big)$ schools with public rating in $I$ fail to match
is at most $n^{-(c+2)}$,
if $\alpha \frac n{\kappa} \ge 3(c+2)\ln n \cdot\exp\big(\alpha k/(2a-\frac12)\big)$.
\rnote{Redo prob bound and conditions.}
\end{lemma}

These two lemmas are used in a mutual induction to justify their assumptions on the numbers of unmatched schools and students, respectively. The bound in \Cref{lem::doctors-interval-non-match} also justifies the assumption on the number of unmatched schools in the next lemma.

\begin{lemma}\label{lem::students-high-value-match-prob}
    Let $d$ be a student with public rating at least $a\alpha$.
    Suppose the fraction of unmatched schools with public rating in $[r(d)+a\alpha,1)$ is at most 
$\alpha \exp\big(-\alpha k/(2a-\frac 12)\big)$ \rnote{may need to modify.}
    Also, suppose that the event ${\cal B}$ does not occur.
    Finally, suppose we run the school-proposing double-cut DA for $d$.
     Then the probability that $d$ fails to receive a match with interview value $1-\psibar_d$ or larger is at most $\exp\big(-k\frac{\psibar_d(a-1)}{2a+\frac12}\big)$.\rnote{may need to modify}
\end{lemma}



\paragraph{Bad Events ${\cal B}$}
These bad events concern the number of agents with ratings in specified public rating intervals (for the sake of brevity, we will say agents in an interval).
We want to limit the analysis to the case where the number of such agents is reasonably close to its expectation. Our analysis will need to assume this for $O(n)$ intervals and unions of intervals.

Let $I$ be an interval of public ratings or a union of such intervals of total length $l$.
We will identify two different pairs of bad events to handle the cases $l\ge \alpha$ and $l<\alpha$, respectively.
For the case $l\ge \alpha$, let $\Bhbf(I)$ and $\Bhbm(I)$ be the events that the number of schools in $I$ are less than $\big(\ell-\frac12 \alpha\big)\cdot \frac{n}{\kappa}$ and  more than $\big(\ell+\frac12 \alpha\big)\cdot \frac{n}{\kappa}$, respectively.
For the case $l< \alpha$, let $\Bhsf(I)$ and $\Bhsm(I)$ be the events that the number of schools in $I$ is less than $\frac 12\ell\cdot \frac{n}{\kappa}$ and more than $2\ell \cdot \frac{n}{\kappa}$, respectively.
(H is for hospital or (high)-school, b for big and s for small $l$, f for too few and m for too many agents).
We define $\Bdbf(I)$, $\Bdbm(I)$, $\Bdsf(I)$ and $\Bdsm(I)$ analogously for students (D for doctor or stu{\bf d}ent), with $n$ replacing $n/\kappa$ in the previous bounds.

We also want to define analogous events for the number of schools in $I$ other than a school $h$ known to be in $I$. For brevity, we write $\Bhbf(I\setminus h)$ instead of $\Bhbf(I\setminus\{r(h)\})$.
So, for example, if $h\in I$, we define $\Bhbf(I\setminus h)$ to be the event that the number of schools in $I$ is less than $\big(\ell-\frac12 \alpha\big)\cdot \big(\frac{n}{\kappa}-1\big)$, and similarly for $\Bhbm(I\setminus h)$, $\Bhsf(I\setminus h)$, $\Bhsm(I\setminus h)$, and likewise for the analogous events concerning doctors. 


\begin{lemma}%\label{lem::number-agents-in-intervals}
    Suppose $\frac {n}{\ln n}\ge \frac{12(c+2)\kappa \ell}{\alpha^2}$. Then $\Bhbm(I)$ occurs with probability at most $n^{-(c+2)}$, and if in addition $\ell\ge a\alpha$, then $\Bhbf(I)$ also occurs with probability at most $n^{-(c+2)}$.
    Finally, if $\ell\ge 8(c+2)\kappa\ln n/n$, then $\Bhsm(I)$ and $\Bhsm(I)$ each occur with probability at most $n^{-(c+2)}$.
    
    Similarly, if $\frac {n}{\ln n}\ge \frac{12(c+2)\ell}{\alpha^2}$, then $\Bdbm(I)$ occurs with probability at most $n^{-(c+2)}$;
    if in addition $\ell \ge a\alpha$, then $\Bdbf(I)$ also occurs with probability at most $n^{-(c+2)}$;
    finally, if $\ell\ge 8(c+2)\ln n/n$, then $\Bdsm(I)$ and $\Bdsf(I)$ each occur with probability at most $n^{-(c+2)}$.

    Analogous bounds hold with $I$ replaced by $I\setminus h$; the one change is that the $n/\kappa$ or $n$ in the relevant bound is replaced by $(n/\kappa)-1$ or $n-1$, respectively.
\end{lemma}
\begin{proof}
    The expected number of schools in $I$ is $\ell\cdot \frac{n}{\kappa}$.
    By a Chernoff bound, there are more than $\big(\ell+\frac12 \alpha\big)\cdot \frac{n}{\kappa}$ schools in $I$ with probability at most $\exp\big(-\frac13\cdot \frac{\alpha^2}{4\ell}\cdot \frac{n}{\kappa}\big)\le n^{-(c+2)}$, if $\frac {n}{\ln n}\ge \frac{12(c+2)\kappa\ell}{\alpha^2}$.
     And by another Chernoff bound,
    there are fewer than $\big[\ell-\frac12\alpha\big]\cdot \frac{n}{\kappa}$ schools in $I$ with probability at most $\exp\big(-\frac12\big(1 - \frac {\alpha}{2\ell}\big)^2\ell\cdot \frac{n}{\kappa}\big)\le n^{-(c+2)}$, if $\frac {n}{\ln n}\ge 8(c+2)\kappa\cdot \frac{a}{(2a-1)^2\alpha}$ (using $\ell\ge a\alpha$).
    Similarly, there are more than $2 \ell \cdot\frac n{\kappa}$ schools in $I$ with probability at most $\exp\big(-\frac13\ell\cdot \frac n\kappa \big)\le n^{-(c+2)}$, and fewer than $\frac12\ell \cdot\frac n{\kappa}$ schools in $I$ with probability at most $\exp\big(-\frac18\ell\cdot\frac n{\kappa}\big)\le n^{-(c+2)}$, if $l\ge 8(c+2)\kappa \ln n/n$.
    \end{proof}

The next corollary shows that, for each student and school, its cone has a population close to its expectation with high probability.
To make this precise, we introduce the following notation.
Recall that $C(d)$ denotes the cone for student $d$; analogously, we let $C(h)$ be the cone for school $h$, the
set of students with public rating in the range $[r(h)-a\alpha,r(h)+a\alpha)$.
\begin{corollary}%\label{cor::cone-population-correct}
    For each student $d$ and school $h$, the events
    $\Bdbm(C(h))$, $\Bdbf(C(h))$, $\Bhbm(C(d))$, $\Bhbf(C(d))$ each occur with probability at most $n^{-(c+2)}$.
    (Note that the cone for $h$ is an interval of doctors and vice-versa.)
\end{corollary}
\begin{proof}
    It suffices to note that the length of these intervals is typically $2a\alpha$, and at least $a\alpha$ (it can be shorter for the very topmost and bottommost agents), and then apply \Cref{lem::number-agents-in-intervals}.
\end{proof}
We assume going forward that none of these events occur, i.e.\ that all the cones have size fairly close to their expectation.

\subsection{Proof of \cref{lem::students-high-value-match-prob}}\label{sec::proof-doc-match-prob-no-idio}

For the purposes of this analysis, we discretize the setting, and then to obtain a result for the continuous setting
we take the limit as the discretization tends to 0, similar to what was done in \cite{AgarwalCole2023}.
In this discretization, if a student (resp.\ school) has the same utility for two schools (resp.\ for two students), we do not run the double cut DA.

\begin{claim}
\label{clm::discrete-dist}
For any $\delta>0$, there is a discrete utility space in which
the probability of having any differences
in the sequence of actions in the school-proposing DA in the original continuous setting and in the discrete setting is at most $\delta$.
\end{claim}
\begin{proof}
$z\ge n^3/2\delta\kappa^2+\frac {n^2}{2z}$ will be an integer in our construction.
We partition the range $[0,3]$ into $3z$ intervals each of length $1/z$.
To do this, we round down each utility to the nearest integer multiple of $1/z$.
Note that for each school $h$, the range of utilities it can provide to a student is given by $[r(h),r(h)+2]$;
on rounding, this creates at most $1+2/z$ possible utilities, each one occurring with probability
at most $1/z$ (to see this consider the random choice of the interview value). Therefore the probability that a student has the same utility for two schools is at most
$\tfrac 12 n(n-1)/z$, and so the probability that any student has the same utility for two schools is at most
$n\cdot n/\kappa\cdot(n/\kappa-1)/2z\le n^3/2z\kappa^2$.

Similarly, the probability that any school has the same utility for two students is at most
$\frac{n(n-1)}{2} \cdot \frac 1z \le \frac{n^2}{2z}$, 
for these utilities are simply the students public ratings.

We set aside all settings in which a student has the same utility for any pair of schools or a school has the same utility for any pair of students.

Recall that in the run of school-proposing double-cut DA, each school repeatedly makes her next highest utility proposal. 
We view this as happening as follows. For each successive discrete utility value, school $h$ has the following choices.

i. $h$ selects some student 
to propose to (among the students $h$ has not yet proposed to); or 

ii. $h$ takes ``no action''. This corresponds 
to $d$ making no proposal achieving the current utility.

Every run of DA in the continuous setting that does not have a hospital selecting two students over the course of a single
utility interval of length $z$ will result in the identical run in the discrete setting in terms of the order in which each
school proposes to the students.
\end{proof}

\begin{lemma}
    The surplus $s\ge\alpha n/\kappa$ if the following bad events do not occur:
    $\Bdbm([r(d)-\alpha,1))$ and $\Bhbf([r(d)-a\alpha,1]$, and if both $a\ge \frac 52$ and $\exp\big(-\alpha k/(2a-\frac 12)\big)\le \frac 12$.
\end{lemma}
\begin{proof}
    As $\Bdbm([r(d)-\alpha,1))$ does not occur, the number of students with public rating at least $r(d)-\alpha$ is at most $[1+\frac 32\alpha -r(d)]n$. As $\Bhbf([r(d)-a\alpha,1]$ does not occur,
    the number of schools with public rating at least $r(d)-a\alpha$ is at least $[1-r(d)+(a-\frac12)\alpha] n/\kappa$.
    By the assumption in \Cref{lem::students-high-value-match-prob}, the number of unmatched schools above $d$'s cone is at most
    $\alpha \frac n{\kappa}\exp\big(-\alpha k/(2a-\frac 12)\big)\le \frac 12 \alpha n$, if $\exp\big(-\alpha k/(2a-\frac 12)\big)\le \frac 12$.
    Thus the surplus, the number of not-fully matched available schools, i.e., schools that could propose to $d$, is at least
    \begin{align*}
        \big[1-r(d)+(a-\tfrac12)\alpha\big] \cdot\frac{n}{\kappa} - \big[1+\tfrac 32\alpha -r(d)\big]\cdot\frac{n}{\kappa} - \tfrac 12 \alpha \cdot\frac{n}{\kappa}
        \le \big(a - \tfrac 52\big)\alpha\cdot \frac{n}{\kappa}\le \alpha \cdot \frac{n}{\kappa},
    \end{align*}
    if $a\ge \frac 52$.
\end{proof}

We build a tree $T$ to represent the possible runs of the double-cut DA.
Each node corresponds to an action by a particular school $h$ at its current utility $u$: the action consists of $h$ doing one of the following:
\begin{itemize}
    \item $h$ proposes to some student $d$.
    \item $h$ makes no proposal with the present utility $u$.
    \end{itemize}
At the children of the current node $h$'s utility will be reduced to $u-z$ and the utility of all other schools will be unchanged.

Let $q(v)$ be the probability that at node $v$ the continuation of the run of the double-cut DA results in no proposal to student $d$. Let $h$'s \emph{residual probability} at node $v$, $p(d,v)$, be the probability that $h'$ proposes to student $d$ in the computation starting at node $v$ if it has not already done so. Let $s$ be the minimum value of the surplus over all the possible paths in the computation.
Finally, let $\qtilde(v)$ be the probability
then if the $s-x$ schools with the smallest residual probabilities propose independently to $d$ with their residual probabilities, it results in no proposal to $d$. In \Cref{clm::fixed-k-stoc-dom},
we will show that $\qtilde(v)\ge q(v)$.
Before proving this claim, we deduce a bound on the probability that $d$ receives no proposal.

\begin{lemma}\label{lem::fail-prob-school-prop}
    Let $d$ be a doctor with public rating at least $a\alpha$.
    Suppose ${\cal B}$ does not occur. Then the probability that $d$ receives no proposal is at most
\end{lemma}
\begin{proof}
    As 
    \end{proof}


\subsection{Applying The Double Cut DA}\label{sec::double-cut-DA-no-idio}

We use both school-proposing and student-proposing double-cut DAs in this analysis. Next, we review how a double-cut DA proceeds. Suppose we want to show that school $h$ has a high probability of receiving a proposal (or $\kappa$ proposals in the event we want to show it is fully matched). The run of DA will have the following participants: all schools with public rating at least $r(h)-\alpha$, and all students with public rating at least $r(h)-a\alpha$.
We run the student-proposing DA, but with the following stopping rules for each student:
whenever a student would make a proposal with utility less than $r(h)-a\alpha+2$ she stops without making this proposal;
also, if she is about to propose to $h$ she makes this proposal and stops. 

The analysis of the school match will exclude the low probability event that there are too many unmatched students, and the analysis of the student match will exclude the low probability event that there are schools which are not fully matched. To avoid circularity, we will use an inductive argument, with the inductive hypothesis being that these bounds apply to increasingly long intervals of schools and students descending from the schools and students with the highest public ratings.

\hide{
The point of this set-up is to ensure there are considerably more students that school places available in this run of DA,
which we call the (student) \emph{surplus}.
Students who do not match with a school other than $h$ are the ones in the surplus.
Each of these students either runs through all their proposals allowed by the double-cut DA, or proposes to $h$ (or both).
One detail in calculating the surplus is that we need to subtract the number of students above $h$'s cone who remain unmatched, which is why we want a high-probability bound on this number.
}

First, we observe that for each school $h$ the outcome in the student-proposing DA is at least as good as the outcome in the double-cut DA for $h$, and a similar claim for students.

\begin{lemma}\label{lem::DA-better-than-double-cut-no-idio}
    Let $h$ be a school. The outcome for $h$ in the standard student-proposing DA is at least as good as the outcome in the double-cut DA for $h$. Similarly, let $d$ be a student. Her outcome in the run of the standard student-proposing DA (yes, we mean student-proposing) is at least as good as her outcome in the school-proposing double-cut DA for $d$.
\end{lemma}
\begin{proof}
   Because every student who proposed to $h$ in the double-cut DA prefers it to schools with a lower public rating
   (due to the cut at utility $r(h)+2-a\alpha$),
    adding additional schools does not affect the proposals $h$ receives. And adding additional students can only improve the proposals $h$ receives. So $h$'s outcome in the full student-proposing DA is only better than its outcome in the double-cut DA for $h$.

    Similarly, for each student $d$, her outcome in the standard school-proposing DA is at least as good as her outcome in the double-cut DA for $d$. But the school-proposing DA produces the worst outcome for $d$ and the school-proposing DA produces the best outcome among all stable matchings involving this set of edges,
    implying the second claim in the lemma.
\end{proof}

\subsubsection{Upper Bounds on the Probability that Students Fail to Match}\label{sec::prob-student-match}

Let ${\cal B}_i^h$ be the event that the $i$th school in public rating order is not fully matched, and let ${\cal C}_j^h= \cup_{i=1}^j {\cal B}_i^h$, be the event that any of the top $j$ schools are not fully matched.
For the analogous event for students we partition the students into intervals $(x,y]$ of exactly $\frac12 \alpha n$ students, for suitable values of $x$ and $y$.
Let ${\cal B}^d_u(I)$ be the event that the interval $I$ of students defined by their public ratings has at least $\alpha n \exp\big(-k \frac{a-1}{2a+\frac12}\big)$ unmatched students;
and let ${\cal C}_j^d= \cup_{i=1}^j {\cal B}_i^d$, be the event that any of the top $j$ intervals has too many unmatched students.

\Cref{lem::students-high-value-match-prob} below concerns the match probability for a student. We will assume inductively that all the schools above her cone are fully matched, i.e.\ the relevant $B_i^h$ do not occur.

\begin{lemma} %\label{lem::students-high-value-match-prob}
    Let $d$ be a student with public rating at least $a\alpha$.
    Suppose each school above $d$'s cone is fully matched.
    Suppose we run the school-proposing double-cut DA for $d$.
    Suppose also that $\Bhf(I)$ does not occur, where $I=[r(d)-a\alpha,1)$, 
    i.e.\ that there are not too few schools in the interval $I$, that $\Bdm(J)$ does not occur,
    where $J=(r(d),1)$, i.e., that there are not too many students above $d$, and that $\Bhf(C(d))$ does not occur, 
    meaning that there are not too few schools in $d$'s cone.
    Then $d$ fails to receive a match with probability at most
    $\exp\big(-k\cdot\frac {a-1}{2a+\frac12} \big)$.
\end{lemma}
\begin{proof}
    The school-proposing double-cut DA has a cut at $d$ and uses schools with public rating
    at least $r(d)-a\alpha$. The surplus in this setting is defined to be the number of schools
    that end up with fewer than $\kappa$ matches.
    
    As $\Bhf(I)$ does not occur, the number of participating schools is at least
    $\big(1-r(d)+(a-\frac 12)\alpha\big) n/\kappa$,  by \Cref{lem::number-agents-in-intervals}.
    Similarly, as $\Bdm(J)$ does not occur, the number of participating students is at most
    $\big(1-r(d)+\frac 12 \alpha\big)n$.
    Finally, by assumption, all the schools above $d$'s cone are fully matched.
    Therefore, the surplus $s$ is at least 
    $\big(1-r(d)+(a-\frac 12)\alpha\big) n/\kappa - \big(1-r(d)+\frac 12 \alpha\big)n/\kappa \ge (a-1)\alpha n/\kappa$.
    
    Now let's calculate the probability that none of $d$'s edges go to the surplus schools.
    As $B_m^h(C(d))$ does not occur, there are at most $(2a+\frac 12 a)\alpha n/\kappa$ schools in $d$'s cone.
    So the probability is upper bounded by:
    \begin{align*}
        \Big(1 - \frac{(a-1)\alpha n/\kappa} {(2a+\frac 12 a)\alpha n/\kappa}  \Big)^k \le \exp\Big(-k\frac {a-1}{2a+\frac12}\Big).
    \end{align*}
\end{proof}

Next, we obtain a high-probability upper bound on the number of students who fail to match.
We will be seeking to show that most of the students in a non-bottommost interval of exactly $\frac 12\alpha n$ students are matched with high probability.
We use an argument similar to that in \Cref{lem::students-high-value-match-prob}.
We want to apply a Chernoff bound, but the difficulty we face is that the outcomes in the previous lemma may not be independent.

\begin{lemma}\label{lem::students-interval-non-match}
Let $I=(x,y]$ an interval containing exactly $\frac 12 \alpha n$ students.
Let $J=(y+a\alpha,1]$ and $K=(y,1]$.
Suppose that neither $\Bhf(J)$ nor $\Bhm(K)$  occurs,
and also, for every student $d\in I$, $\Bhf(C(d))$ does not occur (i.e.\ there are enough schools in its cone);
in addition, if $d$'s public rating $z$ is at least $1-a\alpha$, suppose that $\Bdm([z.1))$ does not occur.
Finally, suppose that every school in $J$ is fully matched.
Then the probability that at least $\alpha n \exp\big(-k\cdot \frac{a-2}{2a-\frac 12}\big)$ students fail to match
is at most $n^{-(c+2)}$,
if $n \ge 3(c+2)\ln n \cdot\exp\big(k\cdot \frac{(a-2)} {(2a-\frac12)}\big)/\alpha$.
\end{lemma}
\begin{proof}
    Consider running the student-proposing DA with the students proposing in public rating order.
    Note that once a student $d$ gets matched to a school it remains matched to that school, as any subsequent student is less preferred.
    To determine the probability that a student fails to match, we compute a lower bound on how many schools in its cone are not fully matched. Let $\nd$ be the number of schools in $d$'s cone.
       \\
    \emph{Case 1}. $y\le 1-a\alpha$ (so $d$ has a cone of length $2a\alpha$).\\
        As $\Bhf(J)$ does not occur, $J$ contains at least $(1-y)n-(a+\frac 12) \alpha n/\kappa$ schools;
    and as $\Bhm(K)$ does not occur, $K$ contains at most $(1-y)n+\frac12\alpha n$ students.
    As the schools in $J$ are fully matched, necessarily by students in $K$, the number of students in $K$ not matched to $J$ is at most $(a+1)\alpha n$ students.
    There are fewer than $\frac 12 \alpha n$ students in $I$ above $d$.
    Therefore the number of schools in $C(d)$ that are fully matched is at most
    $[(a+1)\alpha n+\frac 12 \alpha n]/\kappa = (a+\frac32)\alpha n/\kappa$.
        \\
    \emph{Case 2}. $y> 1-a\alpha$ and $d$ has public rating at most $1-a\alpha$.\\
    As in Case 1, $K$ contains at most $(1-y)n+\frac12\alpha n$ students, and
    there are fewer than $\frac 12 \alpha n$ students in $I$ above $d$.
    Therefore the number of schools in $C(d)$ that are fully matched is at most
     $\big[(1-y) +\frac12)\alpha \big]n/\kappa +\frac 12 \alpha n/\kappa  \le (a+1)\alpha n/\kappa$, as $y>1-a\alpha$.
     \\
     \emph{Case 3}. $y> 1-a\alpha$ and $d$ has public rating greater than $1-a\alpha$.\\
     As $\Bdm([z,1))$ does not occur,
     there are at most $[(1-z)+\frac 12 \alpha]n$ students above $d$.
     Therefore the number of schools in $C(d)$ that are fully matched is at most 
     $[(1-z)+\frac 12 \alpha]n/\kappa$. 

     In the first two cases, as $\Bhf(C(d))$ does not occur, by \Cref{lem::number-agents-in-intervals}, $\nd \ge (2a-\frac12)\alpha n/\kappa$. Also, the number of schools in $C(d)$ that are matched is at most $(a+\frac32)\alpha n/\kappa$,
     and therefore the probability that $d$ fails to match is at most 
     $\big(\frac{(a+\frac32)\alpha n/\kappa}{\nd}\big)^k\le \big(\frac{a+\frac32}{2a-\frac 12}\big)^k
     \le \exp\big(-k\frac{a-2}{2a-\frac12}\big)$.
     In the third case, as $\Bhf(C(d))$ does not occur, $\nd\ge [(1-z) +(a-\frac 12)\alpha]n$.
     Therefore the probability that $d$ fails to match is at most 
     $\big(\frac{[(1-z) \frac 12\alpha]n}{(1-z+(a-\frac12)\alpha}\big)^k\le \big(\frac{(a+\frac12\alpha)+\frac12\alpha}{(a+\frac12\alpha)+(a-\frac12)\alpha}\big)^k=\big(\frac{a+1}{2a} \big)^k\le \exp\big(-k\frac{a-2}{2a-\frac12}$.
     
    This bound holds regardless of what happens to the students in $I$ above $d$; therefore we can apply a Chernoff bound.
    The expected number of students in $I$ that do not match is at most
    $\frac12 \alpha n\exp\big(-k\cdot \frac{(a-2)} {(2a-\frac12)}\big)$ and therefore the probability that more than
    $2\alpha n\exp\big(-k\cdot \frac{(a-2)} {(2a-\frac12)}\big)$ students fail to match is at most
    $\exp\big(-\frac 13 \alpha n\exp\big(-k\cdot \frac{(a-2)} {(2a-\frac12)}\big) \le n^{-(c+2)}$,
    if $n \ge 3(c+2)\ln n \exp\big(k\cdot \frac{(a-2)} {(2a-\frac12)}\big)/\alpha$.
\end{proof}

For one of the intervals $I$ in \Cref{lem::students-interval-non-match}, let ${\cal B}_{\text{int}}(I)$ to be the event that at least $\alpha n \exp\big(-k\cdot \frac{a-2}{2a-\frac 12}\big)$ students in $I$ fail to match.

\hide{
We will be seeking to show that most of the students in an non-bottommost interval $I=(x,x+\ell]$ are matched with high probability.
To this end, we modify the set of participants in the double-cut DA we use. It will be the school-proposing DA.
We use the following range of schools: all the schools
in the interval $(x-a\alpha,1]$, except that we exclude the schools that can propose to some but all
of the students in $I$. More precisely, let $J=(x+\ell-a\alpha,x+a\alpha)$, the schools for which all of $I$ is in their cone, and $K=(x+\ell+a\alpha,1]$, the schools whose cones are completely above $I$, and let $L=(x,1]$, the students
in $I$ and above.
we include the schools with public rating in the range $J \cup K$,
and the  students in $L$.
To ensure exactly this set of students participate, we cut at utility $x+1$ for the schools.
We call this the double-cut DA for (interval) I.


\begin{claim}\label{clm::students-interval-non-match}
Let $I=(x,x+\ell]$ be a public rating interval for students, and let $J$, $K$, and $L$ be as defined above.
Let $\nI$ be the number of students in $I$ and let
${\cal B}_{\text{int}}(I)$ to be the event that at least $\frac 12\nI \alpha$ students
in $I$ fail to match.
Suppose none of ${\cal B}_f^h(J)$, ${\cal B}_f^h(K)$, ${\cal B}_f^d(L\setminus I)$, nor ${\cal B}_v^d(I)$ occur,
and also, for every student $d\in I$, ${\cal B}_m^h(C(d))$ does not occur (i.e.\ there are not too many schools in its cone).
Suppose also that
\begin{itemize}
    \item $\ell= \frac{8(c+2)\ln n}{n}\cdot\exp\big(\frac k{2a+\frac 12}\big)$.
    \item $\ell \le \frac 12 \alpha$.
    \item $k\ge 2a + \frac 12$.
    \item $a\ge 3$.
    \item $= \ge\frac{2k^2\ell}{(2a + \frac12 )\alpha}$. (This is really a condition on $n$.)
    \item $\alpha\ge 4e\exp\big(-k/[2a+\frac12]\big)$.
\end{itemize}
Then, in a run of the school-proposing double-cut DA for $I$, ${\cal B}_{\text{int}}(I)$ occurs with probability at most $n^{-(c+2)}$.
\end{claim}
\begin{proof}
By assumption, ${\cal B}_v^d(I)$ does not occur. As $E[\nI]=\ell n$, we have
$\frac 12\ell n\le \nI \le 2\ell$.

As ${\cal B}_f^h(J)$, ${\cal B}_f^h(K)$, and ${\cal B}_f^d(L\setminus I)$ do not not occur, the surplus $s$ is at least 
the number of schools in $J\cup K$ minus $1/\kappa$ times the number of students in $L\setminus I$.
So $s \ge \big([1-x-\ell-(a+\frac12) \alpha] + [(2a-\frac 12)\alpha-\ell] - [1-x-\ell+\frac 12 \alpha]\big)n/\kappa =[(a-\frac32)\alpha -\ell]n/\kappa\ge \alpha n/\kappa$, as $\ell\le \frac {\alpha}2$ and $a\ge 3$.

Let $S$ denote the set of schools in the surplus. 
We want to determine how many of the edges to $S$ go to a school receiving two or more edges.
Clearly, at most $k\nI$ schools in $S$ can receive edges from $I$.
We can think of this as a process which, for each student, randomly throws each of her $k$ edges to a set of bins of size at most
$(2a+\frac 12)\alpha n/\kappa$ (because ${\cal B}_m^h(C(d))$ does not occur), and this set includes $s$ bins that correspond to the $s$ schools in $S$.
Let's imagine having each student in turn make $k$ throws of edges. Now, let's consider the $k$ throws by the $i$th student in $I$.
The probability that a throw is to a not fully filled school in $S$ is at least $\frac{[s - k(i-1)/\kappa]}{(2a + \frac12)\alpha n/\kappa}
=\frac{[\alpha n - k(i-1)]/\kappa}{\alpha n (2a + \frac12)/\kappa}$, 
and therefore the probability that this student has no edges to a single-edge recipient in $S$ is at most
$\big(1-\frac{\alpha n - k(i-1)}{\alpha n (2a + \frac12)} \big)^k
\le \exp\big(-k\cdot\frac{\alpha n - k(i-1)}{\alpha n (2a + \frac12)}\big)$.
These probability bounds are independent as they do not depend on the outcomes for the earlier students, and so we
can apply a Chernoff bound.
The expected number of students with no such edges is at most $\nI$ times this probability,
and the probability that there are more than $2\nI\cdot \exp\big(-k\frac{\alpha n - k(i-1)}{\alpha n (2a + \frac12)}\big)$ such students is at most
$\exp\Big(-\frac 13\nI \cdot\exp\big(-k\cdot\frac{\alpha n - k(i-1)}{\alpha n (2a + \frac12)}\big)\Big)
\le \exp\Big(-\frac 13\nI \cdot\exp\big(-k\cdot\frac{\alpha n}{\alpha n (2a + \frac12)}\big)\Big)$.
Recall that $\nI \ge \frac 12\ell n$.
Therefore the probability bound is at most 
$\exp\Big(-\frac 16\ell n \cdot\exp\big(-\frac{k}{2a + \frac 12}\big)\Big)\le n^{-(c+2)}$.
Also, $\nI \le 2\ell n$, and as $i\le \nI$, the term $\frac{k^2(i-1)}{\alpha n (2a + \frac12)}
\le \frac{2k^2 \ell}{\alpha n (2a + \frac12)}\le 1$.
Therefore the number of students is at most
$2\nI\cdot\exp\big(1-k/[2a+\frac 12]\big)$.
As $\alpha\ge 4e\exp\big(-k/[2a+\frac12]\big)$, this is at most $\frac 12 \nI \alpha$ students.

The overall failure probability bound is at most $n^{-(c+2)}$.
\end{proof}
}

\subsubsection{Upper Bound on the Probability that Schools Fail to Match}\label{prob-school-unmatched}

In this section, we will show that all the schools with public rating at least $a\alpha$ are fully matched with high probability.


Let ${\cal B}_{\operatorname{eq}}$ be the event that some student has the same utility for a pair of schools.
By \Cref{clm::discrete-dist}, ${\cal B}_{\operatorname{eq}}$ occurs with probability at most $\delta$.

For the next lemma, we need to introduce two additional parameters, $\taubar$ and $\psibar$. 
We will be considering proposals with private value at least $1-\overline{\tau}$ and interview value at least $1-\overline{\psi}$, where $\taubar+\psibar \le \alpha$. This ensures that if we are running a double-cut DA for
a school $h$ with cutoff $r(h)+2-\alpha$, then any such proposal to $h$ will survive the cutoff.

\begin{lemma}\label{lem::value-of-taubar}
    Let $b>2$ and $c>0$ be constants.
    Suppose $\taubar\ge \frac{b\kappa(c+2)\ln n} {(2a-\frac 12)\alpha n}$. Then, with failure probability at most $n^{-(c+2)}$, if $k \le \big(1-\big(\frac 2b\big)^{1/2}\big) \cdot (c+2)\ln n$,
    each student has at least $k$ in-cone edges with private value $1-\taubar$ or larger.
\end{lemma}
\begin{proof}
    Let $d$ be a student. The expected number of $d$'s in-cone edges with private value $1-\taubar$ or larger
    is at least $\taubar$ times the number of schools in her cone, i.e.\ $\taubar (2a-\tfrac12)\alpha n/\kappa\ge b(c+2)\ln n$,
    as $\taubar \ge \frac{b\kappa(c+2)\ln n} {(2a-\frac12)\alpha n}$.
    Then, by a Chernoff bound, the probability that she
    has fewer than $k$ such edges is at most $\exp\big[-\tfrac b2 (c+2)\ln n \big(1 - \frac k{b(c+2)\ln n}\big)^2\big]
    \le n^{-(c+2)}$, if $k \le \big(1-\big(\frac 2b\big)^{1/2}\big) \cdot (c+2)\ln n$.
\end{proof}
Let ${\cal B}_{\taubar}$ be the event that some student has fewer than $k$ in-cone edges with private value $1-\taubar$ or larger. \Cref{lem::value-of-taubar} shows that ${\cal B}_{\taubar}$ occurs with probability at most $n^{-(c+2)}$.

Now we show that in the discrete setting, if neither ${\cal B}_{\taubar}$ nor ${\cal B}_{\text{eq}}$ occur, then each school will receive $\kappa$ proposals with high probability.

\begin{lemma}\label{lem::high-cap-men-outcome}
Suppose that none of ${\cal B}_{\taubar}$, ${\cal B}_{\text{eq}}$, nor $B^h_m(C(d))$ occur, for any student $d$ in $h$'s cone. Suppose also that $\taubar+\psibar \le \alpha$.
Suppose we run the student-proposing double-cut DA for school $h$ with utility cut
$r(h)+2-\alpha$.
Suppose further that each school has capacity $\kappa$, the surplus $s\ge \alpha n$ (the surplus is the number of students who are in $h$'s cone and which end up either proposing to $h$ or being unmatched), and
both $\kappa k\psibar \ge 8(2a+\frac12)\cdot(c+2)\ln n$ and $k\psibar\ge 2(2a+\frac12)$.
Then, with failure probability at most $n^{-(c+2)}$, each school $h$ with public rating at least $a\alpha$
received $\kappa$ matches, i.e.\ is fully matched.
\end{lemma}
\begin{proof}
We build a tree $T$ to represent the possible runs of the double-cut DA, but now nodes will have high degree.
Each node corresponds to an action by a particular student at her current utility: the action consists of her doing one of the following:
\begin{itemize}
    \item She proposes to some school $h'$.
    \item She makes no proposal with the present utility $u$.
    \end{itemize}
Let $q(v)$ be the probability that at node $v$ the continuation of the run of the double-cut DA results in at most $r=\kappa-1$ proposals to school $h$, including the proposals made to $h$ before reaching node $v$. Let $d$'s \emph{residual probability} at node $v$, $p(d,v)$, be the probability that $d$ proposes to school $h$ in the computation starting at node $v$ if she has not already done so. Let $s$ be the minimum surplus over all the possible paths in the computation.
Finally, let $\qtilde(v)$ be the probability that if $x$ students have already proposed to $h$,
then if the $s-x$ students with the smallest residual probabilities propose independently to $h$ with their residual probabilities, it results in at most $r$ proposals to $h$. In \Cref{clm::fixed-k-stoc-dom},
we will show that $\qtilde(v)\ge q(v)$.

Therefore, the probability that $s$ students independently attempting to propose to $h$ at the root $z$ of $T$ produce fewer than $\kappa$ proposals
is an upper bound on the probability that the double-cut DA results in fewer than $\kappa$ proposals to $h$.

But at the root $z$ each of these students $d$ has probability at least $\frac {k}{(2a+\frac12)\alpha n/\kappa}\cdot\psibar$ of proposing to $h$, as by assumption $\Bhm(C(d))$ does not occur.
In expectation, they produce at least $s\cdot \frac {k}{(2a+\frac12)\alpha n/\kappa}\cdot\psibar\ge \frac {k\psibar\kappa}{2a+\frac12}$ proposals, as $s\ge \alpha n$ by assumption.
By a Chernoff bound, they produce fewer than $\kappa$ proposals with probability
at most $\exp\big(-\frac12 \cdot \frac{k\kappa\psibar}{2a + \frac 12} \cdot\big[1 - \frac {(2a+\frac 12)}{k\psibar}\big]^2\big)$.
As $k\psibar \ge 2(2a+\frac 12)$, the probability is at most
$\exp\big(-\frac12 \cdot \frac{k\kappa\psibar}{2a + \frac 12} \cdot \frac 14\big)$,
and as $k\kappa\psibar \ge 2\cdot(2a+\frac 12)\cdot (c+2)\ln n$, this probability in turn is at most $n^{-(c+2)}$.
\end{proof}

Next, we show that in the setting of \Cref{lem::high-cap-men-outcome} the surplus is at most $\alpha n$.

\begin{lemma}\label{lem::students-surplus-no-idio}
Suppose we run the student-proposing double-cut DA for $h$ with the conditions specified in \Cref{lem::high-cap-men-outcome}.
Let $I_1=(r(h)-\alpha,1])$, $I_2=(r(h)-a\alpha,1]$, and $J_i=(1-i\ell,1-(i-1)\ell)$, for every $i$ with
$1-i\ell$ above $h$'s cone.
Suppose also that none of $\Bhm(I_1)$, $\Bdf(I_2)$, or ${\cal B}_\text{int}(J_i)$ occur, for these values of $i$. 
Finally, suppose that $a\ge \frac 72$.
Then the surplus $s\ge \alpha n$.
\end{lemma}
\begin{proof}
    As $\Bhm(r(h)-\alpha,1])$ does not occur, the number of schools with public value at least $r(h)-\alpha$ is at most
    $[1+\frac 32\alpha-r(h)]n$. Likewise, as $\Bdf(r(h)-a\alpha,1])$ does not occur, the number of students with public value at least $r(h)-a\alpha$ is at least
    $[1-r(h) +(a-\frac12)\alpha]n$.
    As ${\cal B}_\text{int}(J_i)$ does not occur, by \Cref{lclm::students-interval-non-match},
    the number of unmatched students above $h$'s cone is at most $ne^{k\psi/2a}\le \frac 12\alpha n$.
    Thus the surplus is at least 
    \begin{align*}
        \big[1+\tfrac 32\alpha-r(h)\big]n - \big[1-r(h) +(a-\tfrac12)\big]\alpha - \tfrac12\alpha n  \ge (a-\tfrac52)\alpha n \ge \alpha n.
    \end{align*}
    \end{proof}

The following claim completes the proof of \Cref{lem::high-cap-men-outcome}.

\begin{claim}\label{clm::fixed-k-stoc-dom}
    For every node $v$ in $T$, $\qtilde(v)\ge q(v)$.
\end{claim}
\begin{proof}
We prove the result by an induction from the leaves to the root of tree $T$.

\smallskip\noindent
\emph{Base case: a leaf node}\\
At a leaf node $v$ all the random decisions have been made, so each student has either proposed to $h$ or not. This results
in either at least $r$ proposals to $h$ or fewer than $r$ proposals; in the first case, $q(v)=1=\qtilde(v)$ and in the second case $q(v)=0=\qtilde(v)$.

\smallskip\noindent
\emph{Inductive step at internal node $v$}\\
Let $d$ be the student making a random choice at node $v$.
Suppose $h$ has been proposed to $x$ times prior to reaching node $v$.
Then $\qtilde(v)$ is calculated using $s-x$ residual probabilities,
and for each child $u$ of $v$, $\qtilde(u)$ is calculated using $s-x$ residual probabilities, with the exception of the child $\overline{u}$ corresponding to a proposal to school $h$, where $\qtilde(\overline{u})$ is calculated using $s-x-1$ residual probabilities. Furthermore, in the calculation of $\qtilde(u)$, all the residual probabilities except at most one are unchanged; the only one that may change is due to the fact that $p(d,v)>p(d,u)$ at each node $u\ne \overline{u}$.

\smallskip\noindent
\emph{Case 1.} $p(d,v)$ is among the smallest $s-x$ residual probabilities at node $v$, and $p(d,u)$ is among the smallest $s-x$ residual probabilities at each child $u\ne \overline{u}$ of $v$.\\
One way to make the random choices involved in evaluating $\qtilde(v)$ is to determine if $d$'s utility for
$h$ equals the utility at node $v$; then, the probability that the remaining
$s-x-1$ residual probabilities at node $v$ generate at most $r-x-1$ proposals to $h$ is given by $\qtilde(\overline{u})$;
otherwise, at any child $u\ne \overline{u}$ of $v$, the probability that the $s-x$ residual probabilities generate at most $r-x$ proposals to $h$ is given by $\qtilde(u)$.
Thus $\qtilde(v)=\sum_{\text{$u$ a child of $v$}} p_u\cdot \qtilde(u)$, where $p_u$ is the probability that the edge to $u$ is followed.
As $q(v)=\sum_{\text{$u$ a child of $v$}} p_u\cdot q(u)$, it follows by induction that $\qtilde(v)\ge q(v)$ in this case.

\smallskip\noindent
\emph{Case 2}.  $p(d,v)$ is not among the smallest $s-x$ residual probabilities at node $v$, and $p(d,u)$ is not among the smallest $s-x$ residual probabilities at any child $u\ne \overline{u}$ of $v$.\\
At every child $u\ne \overline{u}$ of $v$, $\qtilde(u)=\qtilde(v)$, as these probabilities are being computed
using the same residual probabilities.
At node $v$, let $p_1\le p_2\le \ldots\le p_{s-x}$ be the residual probabilities being used to calculate
$\qtilde(v)$, the probability that at most $r-x$ proposals to $h$ are made. 
$\qtilde(\overline{u})$ is the probability that at most $r-x-1$ proposals to $h$ occur with the residual probabilities $p_1\le p_2\le \ldots\le p_{s-x-1}$.
This is smaller than $\qtilde(v)$ for even if $r-x$ proposals to $h$ occurred at $\overline{u}$,
with the same $s-x-1$ random decisions at node $v$, the probability $p_{s-x}$ choice at node $v$ could
result in another ``no proposal'', yielding a total of $r-x$ proposals.

So in this case
$\qtilde(v)>\sum_{\text{$u$ a child of $v$}} p_u\cdot \qtilde(u)$, but $q(v)=\sum_{\text{$u$ a child of $v$}} p_u\cdot q(u)$ still, and again by induction, $\qtilde(v)\ge q(v)$.

\smallskip\noindent
\emph{Case 3}.  $p(d,v)$ is not among the smallest $s-x$ residual probabilities at node $v$, but for at least one child $u\ne \overline{u}$ of $v$, $p(d,u)$ is among the smallest $s-x$ residual probabilities at $u$.\\
The difficulty we face is that if $p(d,u)<p_{s-x}$, then $\qtilde(u)>\qtilde(v)$, while
$\qtilde(\overline{u})<\qtilde(v)$, and if $p(d,u)>p_{s-x}$, then $\qtilde(u)<\qtilde(v)$.
So it would seem that to show
$\qtilde(v)\ge\sum_{\text{$u$ a child of $v$}} p_u\cdot \qtilde(u)$, and then by induction deduce that
$\qtilde(v)\ge q(v)$, we would need to know something about the relative sizes of the various $p_u$.
However, we will sidestep this obstacle by means of the following reduction.

What we need to show is that
\begin{align} %\label{eqn::tree-dom-holds}
    \sum_{\text{$u$ a child of $v$}} p_u\cdot\qtilde(v)\ge\sum_{\text{$u$ a child of $v$}} p_u\cdot \qtilde(u).
\end{align}
Let's first remove the nodes $u$ for which $\qtilde(v)= \qtilde(u)$, i.e.\ the nodes $u$ for which $p(d,u)$ is not among the smallest $s-x$ residual probabilities.
This subtracts equal amounts from both sides of \eqref{eqn::tree-dom-holds}.

Now, let's increase $p_{s-x}$ until it is equal to $p(d,v)$.
This leaves the remaining $\qtilde(u)$ unchanged, as their smallest residual probabilities are unchanged.
However, it reduces $\qtilde(v)$ as the residual probability $p_{s-x}$ which is used in its evaluation is being increased.
But at this point we can switch $p(d,v)$ and the increased $p_{s-x}$, putting us in Case 1.
Now \eqref{eqn::tree-dom-holds} holds for node $v$ and its remaining children; undoing the increase in $p_{s-x}$
only increases $\qtilde(v)$ and therefore \eqref{eqn::tree-dom-holds} continues to hold.

Finally, undoing the change from the previous paragraph continues to maintain \eqref{eqn::tree-dom-holds}.
\end{proof}

\subsection{The $\eps$-Nash Equilibrium}\label{sec::eps-Nash}

We begin by bounding the probability that any of the bad events occur. Let $\cal B$ be the union of these events.

\begin{lemma}\label{lem-bad-events}
    The probability that $\cal B$ occurs, namely any of the bad events excluded in Lemmas~\ref{lem::students-high-value-match-prob}--\ref{lem::students-surplus-no-idio}, is at most $n^{-(c+1)}(4 + 3/\kappa+(a+\frac12)\alpha)+(1+8/\alpha)n^{-(c+2)}$.
\end{lemma}
\begin{proof}
    For each student with public rating at least $a\alpha$,
    \Cref{lem::students-high-value-match-prob} excludes three events each with probability at most $n^{-(c+2)}$, for a total probability of at most $3n^{-(c+1)}$.
    For each of up to $n/\frac 12 \alpha n = 2/\alpha$ intervals of $\alpha n /2$ students, \Cref{clm::students-interval-non-match} excludes two events,
    with a total probability of at most $4n^{-(c+2)}/\alpha$. In addition, it excludes the event ${\cal B}_m^d(C(d))$ for every student $d$, but these events have already been counted as they are excluded in \Cref{lem::students-high-value-match-prob}.
    Finally, it excludes the event ${\cal B}_m^d([z,1))$ for every student with public rating $z\ge 1-a\alpha$.
    By excluding ${\cal B}_m^d([1-a\alpha,1))$, this ensures excluding another $1+(a+\frac12)\alpha n$ events each having probability $n^{-(c+2)}$ suffices.
    Also, adding in the probability for ${\cal B}_{\text{int}}(I)$, for each interval $I$, contributes another $2n^{-(c+2)}/\alpha$ probability.
    By \Cref{lem::value-of-taubar}, excluding ${\cal B}_{\taubar}$ costs at most $n^{-(c+1)}$.
    The failure probability in \Cref{lem::high-cap-men-outcome}, summed over all schools, is at most
    $n^{-(c+1)}/\kappa$.
    \Cref{lem::students-surplus-no-idio} adds two bad events per school, with total probability at most
    $2n^{-(c+1)}/\kappa$, and a further $2/\alpha$ bad events, one for each  interval of $\alpha n/2$ students,
    with total probability at most $2n^{-(c+2)}/\alpha$.
    
   This is a total probability of at most $n^{-(c+1)}(4 + 3/\kappa+(a+\frac12)\alpha)+(1+8/\alpha)n^{-(c+2)}$.
\end{proof}

Next, we show that for a non-bottommost student, a student with public rating at least $a\alpha$,
changing strategies will not significantly improve her outcome in expectation.

\begin{lemma}\label{lem::typical-student-eps-nash}
    Let $d$ be a student with public rating at least $a\alpha$.
        In expectation, ex-ante, $d$ could improve her utility by at most $3n^{-(c+1)} (5+ 3/\kappa)+ 6n^{-(c+2)}/\alpha + 2a\alpha+\frac52\exp\big(-k\cdot\frac {a-1}{2a+\frac12}\big)$.
\end{lemma}
\begin{proof}
If $\cal B$ occurs, $d$ could improve her outcome by at most 3 units of utility; by \Cref{lem-bad-events}, $\cal B$ occurs with probability at most $n^{-(c+1)} (5+ 3/\kappa)+ 6n^{-(c+2)}/\alpha$.
Otherwise, if the recommended strategies are followed, any school $h$ above $d$'s cone will only match to students above $d$; these matches will be preferred to a possible match with $d$, as $h$'s preferences are based only on the students' public ratings.
  By assumption, all the schools above $d$'s cone are fully matched.
  Therefore these schools would reject a proposal from $d$.
  
  If a student changes her strategy to make a different proposal in-cone, if she were already matched, ex-ante her utility would increase in expectation by at most $2a\alpha$, the potential gain from an improved public rating for her partner.
  If she were not already matched, her expected gain would be at most $r(w)+\frac32\le \frac 52$; by \Cref{lem::students-high-value-match-prob}, this occurs with probability at most $\cdot\exp\big(-k\cdot\frac {a-1}{2a+\frac12}\big)$.
  
  Finally, if she switches strategies to make a proposal below her cone, if she were giving up an in-cone match, in expectation her gain would be at most $\taubar\le \alpha$,
  and if she was replacing a non-match, her gain would be at most $\frac 52$; again, a non-match occurs with probability at most $\exp\big(-k\cdot\frac {a-1}{2a+\frac12}\big)$.
\end{proof}
\noindent
\emph{Comment}. This is not to imply that there is a strategy that enables this size of improvement.
We conjecture that the possible expected improvement is in fact $O(\exp(-O(k))$.

The strategies of the bottommost students do not affect the bounds on the gains of higher up students, so it does not have a broader impact whether they follow the designated strategy or not. The only potential impact is on the schools with public rating in the interval $[a\alpha, 2a\alpha)$, for which the claim that they are fully matched may no longer hold.
But this has no impact on the students with public rating at least $a\alpha$.
It also means that if the modeling of these bottommost students is not particularly accurate, it does not affect the results for the remaining students.

\paragraph{Setting the parameters}
We have imposed the following conditions in Lemmas \ref{lem::number-agents-in-intervals}--\ref{lem::students-surplus-no-idio}.

    
\begin{itemize}    
   \item $b>2$, $c>0$ (\Cref{lem::value-of-taubar}).
   \item $a\ge \frac 72$ (\Cref{lem::students-surplus-no-idio})
   \item $\frac {n}{\ln n}\ge \frac{12(c+2)\kappa}{\alpha^2}$ (\Cref{lem::number-agents-in-intervals}).
   \item  $\frac {n}{\ln n} \ge 3(c+2) \cdot\exp\big(k\cdot \frac{(a-2)} {(2a-\frac12)}\big)/\alpha$ (\Cref{clm::students-interval-non-match}).
   \item $\frac {n}{\ln n}  \ge (c+2)\cdot \frac 2{\alpha \psibar \big(1 - \frac {\kappa}{s\psibar}\big)^2}$ (\Cref{lem::high-cap-men-outcome}) and $s\ge \alpha n$ (\Cref{lem::students-surplus-no-idio}).
   \item $\frac {n}{\ln n} \ge \frac{b(c+2)\kappa} {(2a-\frac 12)\alpha \taubar}$ (\Cref{lem::value-of-taubar}).
   \item $\ln n \ge \frac{k}{\big(1-\big(\frac 2b\big)^{1/2}\big) \cdot (c+2)}$ (\Cref{lem::value-of-taubar}).   
   \item $k\psibar \ge 2\cdot(2a+\frac 12)$ (\Cref{lem::high-cap-men-outcome}).
   \item $\kappa k\psibar \ge 2\cdot(2a+\frac 12)\cdot(c+2)\ln n$ (\Cref{lem::high-cap-men-outcome}).
   \item $\alpha \ge \psibar+\taubar$ (\Cref{lem::high-cap-men-outcome}).
\end{itemize}

We would like to minimize the $\eps$ implied by \Cref{lem::typical-student-eps-nash}.
First, we set $c=\ln 9/\ln n$; this makes the first term in the deviation improvement be at most
$1/n$.
For simplicity, we set $b=3$ and $a = \frac 72$.
The second term, which is the most significant term, calls for minimizing $\alpha$.
To this end, for simplicity, we set $\taubar=\psibar=\frac12\alpha$
and $\psibar=\frac {4a+1}{k}\cdot\max\big\{1, \frac{(c+2)\ln n}{\kappa}\big\}$.
Then it suffices to set $n$ large enough to satisfy the remaining conditions.
This yields an $\eps=O\big(\max\big\{\frac 1k,\frac{\ln n}{k\kappa}\big\}\big)$, albeit with a somewhat large
constant multiplier (but simulations suggest the actual constant is considerably smaller).
\rnote{Can we do this?}
}


\hide{
Still, we give a bound on the match probabilities for the bottommost students and deduce bounds on their expected gains.
For this final lemma, we need to exclude one more bad event, namely that the number of bottommost schools, those with public rank $a\alpha$ or less, is at least $(a-\frac 12)\alpha n/\kappa$; this has failure probability at most
$n^{-(c+2)}$. Call this event ${\cal B}_b$.

\begin{lemma}\label{lem::bottom-students-gains}
Suppose neither $\cal B$ nor ${\cal B}_b$ occur.
    Let $d_i$ be the student with the $i$th smallest public rating. If $i\ge (2a+\frac 12)\alpha n/k$ her probability of failing to match
    is at most $\exp\big(-ki/(2a+\frac 12)\alpha n\big)$, and if $i<(2a+\frac 12)\alpha n/k$, her probability of matching is still $\Theta(1)$, if $n\ge \frac{16(c+2)k \cdot e^{1+1/k}} {\alpha (a + \frac 12)}$.
\end{lemma}
\begin{proof}
    Suppose we run the student-proposing DA, allowing each student in turn to propose, continuing until she matches
    or goes through all $k$ of her proposals. Consider what happens when student $d_i$ makes her proposals. Given that the schools above her cone are fully matched, it must be
    that there are at least $i$ unmatched school places in $d_i$'s cone, and hence at least $i/\kappa$ schools with one or more places available; as her private values provide a uniform
    random selection among the schools in her cone, at most $(2a+\frac12)\alpha n/\kappa$ schools,
    the probability that she fails to match is at most
   $\big(1 - \frac {i/\kappa}{(2a+\frac 12)\alpha n/\kappa}\big)^k \le \exp\big(-\frac{ki}{(2a+\frac 12)\alpha n}\big)$.

    \rnote{The following part is not right. It needs an analysis that obtains the distribution of space in the schools. This may not be worth the trouble.}
    To get a $\Theta(1)$ bound for $i<(2a+\frac 12)\alpha n/k$, we argue as follows.
    Suppose there are no more than $(a-\frac 12)\alpha n/k$ unmatched students remaining.
    As ${\cal B}_b$ does not occur, $d_i$'s cone contains at least $(a-\frac 12)\alpha n/\kappa$ schools.
    Then $d_i$ fails to match with probability at least $(1-\frac 1k))^k\ge e^{-(1+1/2k)}$, for $k\ge 2$.
    If there are at most $\frac 12 (a-\frac 12)\alpha n/k$ unmatched students when the number of available school places is first reduced to  $(a-\frac 12)\alpha n/k$, then at least $\frac 12 (a-\frac 12)\alpha n/k$ remain unfilled.
    Otherwise, in expectation at least $e^{-(1+1/2k)}\cdot \frac 12 (a-\frac 12)\alpha n/k$ students and therefore school places
    remain unmatched, and by a Chernoff bound, the probability that fewer than $\frac 14 e^{-(1+1/2k)}\cdot (a-\frac 12)\alpha n/k$ students (and school places) remain unmatched is at most 
    $\exp(-\frac 1{16} e^{-(1+1/2k)}\cdot (a-\frac 12)\alpha n/k)\le n^{-(c+2)}$, if $n\ge \frac{16(c+2)ke^{1+1/k}}{\alpha (a + \frac 12)}$.
\end{proof}
}

==> preliminaries.tex <==
\section{Preliminaries}

\pj{Lee's model, the idiosyncracies and the metrics we use --- match rate, men's / women's loss, eps bayes nash equilibria definition.} \\

\pj{definition of aligned man/woman. Definition of ``cone" given an $\alpha$ value. what does it mean to match ``in-cone" ... Definiton of M[i..j] and W[i..j]}

\pj{probably need to state that assume wherever necessary that $n\alpha$ is an integer}

\pj{which values of $\lambda$ we focus on.}

Let $m_i$ denote the $i^{th}$ man in decreasing order of public ratings and let $\ratem{i}$ be the public rating of this man. The $\alpha$-cone if $m_i$ is the set of women with public ratings in range $[\ratem{i} - a\alpha, \ratem{i} + a\alpha]$. The $\alpha$-cone of $w_i$ is defined similarly.

==> rebuttal.tex <==
Thank you for your careful reading and thoughtful feedback.
We comment on the questions that have been raised and related points.

What happens when the school-proposing/hospital-proposing DA is used: The results hold unchanged in the model in which doctors choose the interviews, because all the bounds follow by considering runs of both the doctor-proposing and the hospital-proposing double-cut DA. 

Possible changes to the utilities:

i. At present, the private values have a small effect on the matches, as the private values for the interviewing doctors are all close to 1 (recall they are the top $\kappa k$ in-cone private values). One would have to increase the weights significantly for there to be an effect, which we believe would be to increase the cone size, so that the weighted range of private values and public rankings remain similar.

ii. Allowing non-uniform draws, or more generally, utilities that are functions of the public ratings, private and interview values. We believe the results would be similar, with the exponent of the match rate depending on the degree of non-uniformity. One part of the analysis needs the expected number and the actual number of agents in a public rating interval to be similar. With bounded rates of change of the utilities w.r.t. the public ratings, this will continue to hold. And for the tree stochastic dominance, we believe it suffices to have rates of change for the doctors' utilities w.r.t. each of the private and interview values being within constant factors of each other, and similarly for the hospitals.

iii. Different hospitals having different capacities: discussed below.

Differing numbers of interview requests: We would want these differing numbers to be an outcome of the setting. We note that this occurs naturally in the model in which doctors request interview and hospitals each grant $\kappa k$ interviews. 

The lack of an $\epsilon$-Nash bound for the bottommost agents: We strongly suspect that an $\epsilon'$ bound applies to the doctors, where $\epsilon'>\epsilon$, but is still quite small. The reason is that the only way these doctors could significantly improve their outcome is by substantially increasing their match rate, supposing it is somewhat low. But we believe their match rate is already quite high, as indicated by our simulation results. 

One could also seek to extend the $\epsilon$-Nash bound to the hospitals. Then we would need to specify the utility of a capacity $\kappa$ hospital: one natural measure is the sum of the utilities derived from each of its matches.  Since hospitals can only manipulate the ordering of the proposals they receive, and we can show for all but the bottommost that they have only expected $O(\epsilon)$ loss, this bounds their possible utility gain.

\pj{Truncation can still help them right?} \rjc{This just leads to better in-cone matches, so within the $\epsilon$ bound. What it could do is hurt the doctors.}

Takeaway:
Doctors/students should spread their applications over a suitable public value based cone. This could be useful advice for naive users who might otherwise misunderstand the advice to list choices in order of preference.

Why this $\epsilon$-Nash equilibrium: Our view is that we are analyzing a natural strategy, which turns out to have an $\epsilon$-Nash outcome for all but possibly the bottommost agents.

Interview scheduling: We view this as fully distributed. The doctors select the hospitals where they interview based on their utilities. Granted there is no enforcement of the $k$ interview bound per doctor, nor of the requirement that hospitals interview all applicants.

Relevance to EC: Multiple papers on stable matching have appeared in each recent EC, including the best student paper in EC'16. The paper whose model is the starting point for our work, by Allman and Ashlagi (EC'25 PC co-chair) appeared in EC'23.

[Continued from above] iii. Different hospitals having different capacities: We believe the current analysis can accommodate this with some modest changes. The most important is that doctors would need to select hospitals in proportion to their capacities. One way to do this would be for each doctor to order her private values as follows: suppose she has private value $1-\delta_i$ for hospital $h_i$ with capacity $\kappa_i$. Then she would choose the $k$ hospitals that maximize the values $1 - \frac{\delta_i}{\kappa_i}$.

Finally, we comment on the graphs in Figure 2. The whiskers in these graphs are less informative than we intended; we will remove them.

==> stoc-dom.tex <==
\subsection{The double cut DA}

Let $m$ be a man with public score $v=v(m)$. In the double-cut DA for $m$ only the women with public utility
greater than $v-a \alpha$ make proposals, furthermore they are limited to proposals which provide them utility
greater than $c(m)\triangleq \lambda(v-\mu)+(1-\lambda)$, where $\mu= k/(2a\alpha n)$. Recall that we set $\alpha =e^{-\beta k}$, for a suitable $\beta>0$.
\pj{Fix notation and relate k and alpha here!}

\begin{lemma}\label{lem::stoc-dom}
Let $m$ be an arbitrary man with public score at least $v-\mu$.
If none of ${\cal B}_1$--${\cal B}_3$ occur, then, in the woman proposing double-cut DA for $m$,
with probability at least $1- e^{-\beta k}$,
 $m$ receives at least one proposal from a woman in or above his cone.
\end{lemma}
\begin{proof}
We would like to argue that each of the women in the surplus will make a proposal to $m$ with independent probability at least $\mu$. For then the probability that $m$ receives no proposal would be at most
$(1-\mu)^s\le e^{-\mu s}$. If ${\cal B}_1$--${\cal B}_3$ do not occur, then $s\ge b\alpha n$, where $b= $, and as
$\mu = ke^{\beta k}/2an$, this yields a probability of at most $e^{-bk/2a}=e^{-\beta k}$.

However, the random choices of the values for $m$ by the women in the surplus need not be independent, as the choice of one woman can affect whether another woman is even in the surplus. Nonetheless, we show that the actual probability of $m$ receiving a proposal
is only higher than what would be achieved in the above independent random choices scenario.

We prove this bound holds regardless of the private values of the women for men other than $m$, and of the men other than $m$ for all the women. So let's fix all these private values. We start by eliminating the zero probability events that a woman has the same private value for any two men, or that a man has the same private value for any two women. Clearly, these zero probability events are not going to affect our final bound on the probability that $m$ receives no proposal.

It will be helpful to define a tree $T$ which will represent the possible computations of the double-cut DA. 
These computations depend only on $m$'s private values and on the private values of the women for $m$.
Each random choice of these private values defines a computation path. To make these paths unique, whenever two or more women could make a proposal, we let the one with lower rank proceed.

Let's consider the actions of a single woman $w$. Suppose $w$'s utilities for the men other than $m$, which are above the cut at $c(m)$, are $u_1>u_2>\ldots>u_s$. On each computation path $P$, there will be a subsequence of up to $2s+1$ nodes corresponding to $w$'s actions; let $x_1,x_2,x_3,x_4,\ldots x_{2r+1}$ be the node names on path $P$, where $r\le s$ (as we shall see, on each path there are an odd number of nodes corresponding to $w$'s actions); note that the value of $r$ may be path dependent.
Node $x_{2i}$ corresponds to making a proposal to the man for which $w$ has utility $u_i$.
Node $x_{2i+1}$ corresponds to the random choice of whether $w$'s private value for $m$ is in the range
$(\max\{u_{i+1},c(m)\},u_{i})$ or not (we take $u_0$ to be $\lambda v+(1-\lambda)$ and $u_{s+1}$ to be 0); the first choice corresponds to $w$ proposing to $m$ at this point in the current run of the double-cut DA, and the second choice corresponds to $w$ having a smaller private value for $m$, and to taking
no action (i.e.\ making no proposal) for this range of private values.
There will be one edge descending from $x_{2i}$ going to the node representing the next action in this run of DA; there is always an edge, for at the very least this woman has not yet proposed to $m$, and therefore still has a random choice of whether to do so or not.
Similarly, there will be two edges descending from $x_{2i+1}$, corresponding respectively to the proposal to $m$ and the no action move, again going to the next actions in these two runs or to a terminal leaf node in the case of no further actions being possible.

We associate a probability with each path $P$ in $T$, namely the probability that $P$ is traversed as a function of the random choices of the private values. This probability is also associated with the leaf at the end of $P$.
We then give each internal node a probability equal to the sum of the probabilities of its children; this is also the sum of the probabilities of the paths going through the node.

Each path $P$ either has a proposal to $m$ or not. We now calculate, for each node, the probability that the continuation of the run of DA from that node will result in not making a proposal to $m$.
We call this the blocking probability.
For leaf nodes, clearly this probability is either 1 or 0. 
For an internal node, the blocking probability is simply a weighted combination of the probabilities for its children.
Specifically, let $x$ be an internal node.

\smallskip
\noindent
{\bf Case 1}. $x$ has a single child $y$.\\
Let $p_x$ and $p_y$ be the blocking probabilities for nodes $x$ and $y$.
Clearly, $p_x=p_y$, as the proposal made at node $x$ is to a man other than $m$.

\smallskip\noindent
{\bf Case 2}. $x$ has two children, $y$ and $z$.\\
Let $p_x$, $p_y$, and $p_z$ be the blocking probabilities for nodes $x$, $y$, and $z$, respectively.
Suppose edge $(x,y)$ is traversed with probability $\pl$ and edge $(x,z)$ with probability $\pr=1-\pl$.
Suppose further that edge $(x,y)$ corresponds to making a proposal to $m$ and $(x,z)$ to ``no action''.
Note that $p_y=0$.
Then $p_x=\pr\cdot p_z$.

\smallskip

We define the \emph{idealized blocking probability} $q_x$ at a node $x$ in $T$ as follows.
If $m$ is proposed to at some node above $x$ then $q_x=0$.
Otherwise, we proceed as follows.
Suppose that at node $x$ the remaining range of utility for woman $w$ is one of $[0,u)$ or $[0,u]$.
We define $w$ to have blocking probability $c(m)/u$ at node $x$ (note that $c(m)\le u$).
To calculate $q_x$,
we start with the set of all the women participating in the double-cut DA for $m$.
We then remove those women who propose to some man other than $m$ on every path through $x$ (the men proposed to need not be the same on every path). For the remaining women, we take the $s$ women with the largest blocking probabilities, breaking ties arbitrarily
(note that there are at least $s$ women remaining as in this case there have been no proposals to $m$).
Let the blocking probabilities at node $x$ for these women be $o_1^x,o_2^x,\ldots,o_s^x$.
The idealized blocking probability $q_x$ at node $x$ is defined to be $\prod_{1\le i\le s} o_i^x$.


\begin{claim}
    For all $x\in T$, $p(x)\le q(x)$.
\end{claim}
\begin{proof}
We show the result by an induction from the leaves to the root of $T$.

At a leaf $x$, if $p_x=0$, this is because $m$ had received a proposal, and therefore $q_x=0$ also.
While if $p_x=1$, then $m$ has not received any proposals, and therefore all the non-removed women have blocking probability 1, implying $q_x=1$.

Now, let's consider an internal node.

\smallskip
\noindent
{\bf Case 1}. $x$ has a single child $y$.\\
As the sets of paths through $x$ and through $y$ are identical, it must be that
$q_x= q_y$, and as $p_x=p_y$ in this case, the inductive claim follows.

\smallskip\noindent
{\bf Case 2}. $x$ has two children, $y$ and $z$.\\
If there is a proposal to $m$ on the path to $x$ then $p_x=0=q_x$ and the result is immediate.
Otherwise, $p_x=\pr\cdot p_z$ (as observed in the previous Case 2 above).
Suppose that at node $z$, $q_z=\prod_{1\le i\le s} o_i^z$, and further $o_1^z\ge o_2^z\ge\ldots\ge o_s^z$.
Let $w$ be the woman making the random choice at node $x$ of whether to propose to $m$ at this point.
Let $o_w^x$ be the blocking probability for $w$ at node $x$, and $o_w^z$ be her blocking probability at node $z$
(necessarily, $o_w^x<o_w^z$).
Finally, suppose that $w$'s possible utility range at $x$ is $[0,u)$ and at $y$ it is $[0,u-\Delta u]$.
Note that $o_w^x =\frac{c(m)}{u}$ and $o_w^z=\frac{c(m)}{u-\Delta u}$.

\smallskip\noindent
{\bf Case 2.1}. $o_w^x\ge o_s^z$.\\
Suppose $w$ is the $j$th woman in the product $\prod_{1\le i\le s} o_i^x$.
Then,
\begin{align*}
q_x & =o_w^x \cdot \prod_{1\le i\le s, i\ne j} o_i^x \\
    &= o_w^x\cdot \prod_{1\le i\le s, i\ne j} o_i^z \\
    &= \frac{c(m)}{u} \cdot \prod_{1\le i\le s, i\ne j} o_i^z\\
    &= \frac{u-\Delta u}{u} \cdot \frac{c(m)}{u-\Delta u} \cdot \prod_{1\le i\le s, i\ne j} o_i^z\\
    &= \pr \cdot o_w^z \cdot \prod_{1\le i\le s, i\ne j} o_i^z\\
    & = \pr q_z
    \ge \pr p_z
     = p_x.
\end{align*}

\smallskip\noindent
{\bf Case 2.2}. $o_w^z< o_s^z$.\\
Then,
\begin{align*}
q_x & =\prod_{1\le i\le s} o_i^x 
     = \prod_{1\le i\le s} o_i^z 
     =p_z
     \ge \pr p_z 
     = p_x.
\end{align*}

\smallskip\noindent
{\bf Case 2.3}. $o_w^x< o_s^z\le o_w^z$.\\
Let $o_1^x\ge o_2^x\ge \ldots \ge o_s^x$.
Then, using the indices to name the same women w.r.t.\ the product at node $z$, we have
\begin{align*}
q_x & = \prod_{1\le i\le s} o_i^x 
      > o_w^x \cdot \prod_{1\le i\le s-1} o_i^x 
      = \pr \cdot o_w^z \cdot \prod_{1\le i\le s-1} o_i^z 
      = \pr \cdot q_z 
      \ge \pr \cdot p_z
      =p_x.
\end{align*}
\end{proof}

\end{proof}

\newpage

\rnote{This will be a complete rewrite.}

\begin{def}\label{def::threshold-strategy}
Given a threshold $\tau\in [0,1]$, a threshold strategy for the women in the woman-proposing DA has her proposing to a man $m$ only if her private value for $m$ is greater than $1-\tau$.
\hide{ 
and an analogous threshold $\mu\in[0,1]$ for the men, 
has a man rejecting any proposal with private value $1-\mu$ or less, again in the woman-proposing DA. \pj{I think men do not have such a threshold, we only focus on these edges ($1 - \mu$) in the analysis to guarantee that in the woman proposing DA, men receive a "good quality" proposal.} \rnote{Yes, you are right.}
Similar definitions apply to the man-proposing DA. 
}
\end{def}

\begin{def}\label{def::cone}
    The $\alpha$-cone for woman $w$ is the set of men with public rating in the
    range $(r_w - a\alpha, r_w + a\alpha)$, where $a>1$ is a suitable constant, and $\alpha\in(0,1)$.
\end{def}

\begin{def}\label{k-thresh}
    The $k$-threshold strategy in the women proposing DA has $\tau = \tfrac{k} {2a\alpha n}$.
    This ensures that when the cone's range is fully contained in $[0,1]$, the expected number of men in $w$'s cone 
    will be equal to $k$. 
\end{def}

\begin{def}\label{def::top-k}
   A top-$k$ strategy for the women in the woman-proposing DA has an individual threshold $\tau_w$ for each woman $w$, chosen so that the set of men for which $w$ has private value greater than $1-\tau_w$
   contains exactly $k$ men;
   if there are fewer than $k$ men in her cone, the threshold is set to 1.
\end{def}

\paragraph{Outline of the analysis} 
We seek to analyze a setting in which women request interviews, and then the woman-proposing DA is run on the
interview edges. Our analyses will consider runs of both the woman-proposing and man-proposing DA on these edges in order to obtain useful bounds, but in the end it is the outcome of woman-proposing DA that we seek to characterize.

Our analyses are all based on the double-cut DA, introduced by Agarwal and Cole. We describe the woman-proposing version with respect to a man $m$ with public rating $r_m$. The double-cut DA is simply a truncated run of the standard DA algorithm. More specifically, we allow only those women with public rating more than $r_m - a\alpha$ to participate, i.e.\ those women in or above $m$'s $\alpha$-cone. Furthermore, a woman stops as soon as her next proposal would be either to $m$ or have a utility of
$c(m) \triangleq\lambda r_m + (1-\lambda)\cdot (1-\tau)$ or less; this is the double-cut.



We seek to analyze the setting in which each woman's proposals are in her cone. However, we will need to begin by considering a setting in which proposals to any man are possible, but in-cone proposals are preferred, on both sides. To achieve this, we modify the utilities as follows.
%
\begin{equation*}
    U_i(m_j) = \begin{cases}
    \ratem{j} + \sw{i}{j} + 2 ~~~~ \text{if } m_j \in M[\ratew{i} - a\alpha, \ratew{i} + a\alpha] \\
    \ratem{j} + \sw{i}{j} ~~~~~~~~~ \text{otherwise} \\
    \end{cases}
\end{equation*}
and
\begin{equation*}
    V_i(w_j) = \begin{cases}
    \ratew{j} + \sm{i}{j} + 2 ~~~~ \text{if } w_j \in W[\ratem{i} - a\alpha, \ratem{i} + a\alpha] \\
    \ratew{j} + \sm{i}{j} ~~~~~~~~~ \text{otherwise} \\
    \end{cases}
\end{equation*}


To introduce our techniques in a relatively simple setting, we start by considering the setting in which men consider only the public values of the women in calculating their utilities (or equivalently, all their private values are equal to 0).
We will show that in this setting, the probability that a man with public rating at least $a\alpha$ remains unmatched is at most
$e^{-\beta k}$, for a suitable constant $\beta>0$.
We will show the same bound for the women with value at least $a\alpha$ (the proof is slightly different).
%We then show that in expectation there are few out-of-cone matches, which allows us to deduce similar bounds when all proposals are in-cone.
We then extend the result to bound the number of unmatched men in an interval covering a range of $2a \alpha$.
We conclude this case by extending the result to the top-$k$ strategy.

Next, we extend the result to the case that the men do take account of their private values. Similar bounds hold. \pj{bounds should be slighly worse.. atleast based on the previous analysis.} \rnote{Agreed.}

We continue by considering the case in which each man has capacity $c>1$, meaning that it wants to match with $c$ women. We are particularly interested in the case that $ck=\Omega(\ln n)$, for it will turn out that in this case all the men with public rating at least $a\alpha$ will be fully matched. The analogous statement does not hold for the women. 

After this, we consider the interview model introduced in Allman and Ashlagi. We show that similar bounds apply here too.

Finally, we consider a setting in which women have two public ratings $r_w$ and $s_w$, and each man $m$'s utility for every woman $w$ is given by $\lambda_m r_w + (1-\lambda_m) s_w$, where $\lambda_m\in (0,1)$ is a man specific parameter. In this model a women knows how each man rates her, and therefore can figure out which men rate her relatively highly, which allows her to more effectively target her proposals. \rnote{Add informal statement of results; not sure what they are yet.}

\subsection{Setting with No private Values for the Men}

\subsubsection{The Threshold Strategy Bound}

\begin{lemma} \label{lem::men-no-match-prob-thresh-str}
   Let $m$ be a man with public rating at least $a\alpha$. In the double-cut DA, the probability that $m$ remains unmatched is at most $e^{-s\tau}$.
\end{lemma}
%
\begin{proof}
    We prove the bound holds regardless of the private values of the women for men other than $m$, and of the men other than $m$ for all the women (actually, the men's private values don't matter in this proof) \pj{I think it eventually will---when we talk about the eps bayes nash equilibrium} \rnote{Agreed; but that's not this lemma.}. So let's fix all these private values, which we call \emph{fixing all but $m$}. We start by eliminating the zero probability events that a woman has the same private value for any two men, or that a man has the same private value for any two women. Clearly, these zero probability events are not going to affect our final bound on the probability that $m$ receives no proposal.

    We form a tree to represent the computation with no proposals to $m$ and the computations that end with a single proposal to $m$ (we terminate any run as soon as there is a proposal to $m$.) This tree has a path $P$ which represents the no-proposal run, and single edges leaving this path, which represent the alternate computations in which $m$ receives a proposal.
    
    There are two types of nodes on $P$. Those that represent a proposal by some woman to a man other than $m$, and those that represent branch points at which either there is a proposal to $m$ or no proposal is made at that point.
    To make this a little more precise, let's consider the subsequence of nodes corresponding to the actions of a woman $w$.
    Let $w$'s utilities for the men other than $m$, which are above the cut at $c(m)$, be $u_{w1}>u_{w2}>\ldots>u_{wr}>c(m)$ \pj{should be $u_{m1} \cdots$}. Let $x_{w1},x_{w2},x_{w3},x_{w4},\ldots x_{w,2r+1}$ be the subsequence of nodes on path $P$ corresponding to $w$'s possible actions.
    Node $x_{w,2i}$ corresponds to making a proposal to the man for which $w$ has utility $u_i$.
    Node $x_{w,2i+1}$ corresponds to the random choice of whether $w$'s private value for $m$ is in the range
    $(u_{w,i+1},u_{wi})$ or not (we take $u_{w0}$ to be $\lambda r_w+(1-\lambda)$ \pj{should be 1 ?}\rnote{times 1?} and $u_{w,r+1}$ to be $\lambda r_w+(1-\lambda)\cdot (1-\tau)$ \pj{should be 0?} \rnote{no; this is the bottom of the range which produces an edge.}); the first choice corresponds to $w$ proposing to $m$ at this point in the current run of the double-cut DA, and the second choice corresponds to $w$ having a smaller private value for $m$, and to taking
    no action (i.e.\ making no proposal to $m$) for this range of private values.
    The second choice, no-action, is what is represented on path $P$.
    To make $P$ unambiguous, whenever two or more women could make a proposal, we let the one with lower public rating proceed. 
    
    At the end of the run represented by path $P$ at least $s$ women end up unmatched; recall that $s$ denotes the surplus. We let $S$ denote the set of these $s$ or more women. 

    Now, we determine the probability that $P$ occurs as a function of the women's choices of private value for $m$.
    Let $\delta_{wi}=u_{wi}-u_{w,i-1}$, for $1\le i\le r+1$.
    Note that for all $w\in S$, $\sum_{1\le h\le r+1} \delta_{wh} = \tau$.
Conditioned on reaching node $x_{w,2i-1}$, the probability of reaching node $x_{w,2i}$, 
i.e.\ of $w$ making no proposal to $m$ with utility in the range $(u_{w,i-1},u_{w,i})$ is given by
\begin{align*}
   \frac{1- \sum_{h=1}^i\delta_{wh}} {1- \sum_{h=1}^{i-1}\delta_{wh}}.
\end{align*}

It follows that fixing all but $m$, the probability of having no proposals to $m$ is given by 
\begin{align}\label{eqn::bound-man-no-match}
\prod_{w\in S,1\le i\le r+1} \frac {1- \sum_{h=1}^i\delta_{wh}} {1- \sum_{h=1}^{i-1}\delta_{wh}} 
     \le \prod_{w\in S} \Big[ 1- \sum_{h=1}^{r+1}\delta_{wh} \Big]
    \le \big(1 - \tau\big)^s
     \le \exp\big(-s\tau\big).
\end{align}
\end{proof}

\begin{corollary}\label{cor::thresh-str-bound-men}
    If neither ${\cal B}_1$ nor ${\cal B}_2$ happen, then in the woman-proposing double cut DA a man $m$ with public rating at least $a\alpha$ remains unmatched with probability at most $e^{-\beta k}$, where $\beta = \tfrac {b\lambda k}{2a(1-\lambda)}$.
\end{corollary}
\begin{proof}
 If neither ${\cal B}_1$ nor ${\cal B}_2$ happen, then $s\ge b\alpha n$.
 Now $\tau = \tfrac{\lambda k} {(1-\lambda)2a\alpha n}$, and so
 $s\tau \ge \tfrac {b\lambda k}{2a(1-\lambda)}= \beta k$.
 The result now follows from \Cref{lem::men-no-match-prob-thresh-str}.
\end{proof}

\begin{corollary}\label{cor::thresh-str-bound-men-fullDA}
    If neither ${\cal B}_1$ nor ${\cal B}_2$ happen, then in the woman-proposing DA a man $m$ with public rating at least $a\alpha$ remains unmatched with probability at most $e^{-\beta k}$, where $\beta = \tfrac {b\lambda k}{2a(1-\lambda)}$.
\end{corollary}
\begin{proof}
    In the full DA, there are more proposals from more women, meaning that each man only does better than in the double-cut DA.
\end{proof}

Next, we determine the probability that a woman remains unmatched.
\begin{lemma} \label{lem::women-no-match-prob-thresh-str}
   Let $w$ be a woman with public rating at least $a\alpha$. In the man-proposing double-cut DA, using the edges chosen by the women's threshold strategy, the probability that $w$ remains unmatched is at most $e^{-s\tau}$.
\end{lemma}
%
\begin{proof}
  The proof is largely the same as for \Cref{lem::men-no-match-prob-thresh-str}.
  Here, we allow only those men with public rating more than $r_m-a\alpha$ to participate, i.e.\ those men in or above $w$'s $\alpha$-cone. Furthermore, a man stops as soon as his next proposal would be either to $w$ or to a woman below $w$ (who would necessarily provide a smaller utility than $w$); this is the double-cut.
  The structure of the path $P$ is somewhat simpler here. For each man $m$, there is a subsequence of nodes corresponding to his proposals to women above $w$ in public rank order, and for the $s$ men that remain unmatched, a final node corresponding to his possible proposal to $w$.
  There is such a proposal with probability $\tau$; this is the event that $w$ had a high enough private value for this edge. Again, let $S$ denote the set of unmatched men.
  Now the probability that path $P$ occurs is given by
  \begin{align*}
      \prod_{n\in S} (1-\tau) \le e^{-\tau s}.
  \end{align*}
\end{proof}

The next corollary follows in a similar way to the bound for the men.
\begin{corollary}\label{cor::thresh-str-bound-men-fullDA}
    If neither ${\cal B}_1$ nor ${\cal B}_2$ happen, then in the woman-proposing DA a woman $w$ with public rating at least $a\alpha$ remains unmatched with probability at most $e^{-\beta k}$, where $\beta = \tfrac {b\lambda k}{2a(1-\lambda)}$.
\end{corollary}
\begin{proof}
    The bound holds for the man-proposing DA in the same way as the bound on the men in the women-proposing DA.
    But the same men and women are matched in the runs of both the man and the woman-proposing DA, so the bound applies
    to the woman-proposing DA also.
\end{proof}

Now, we bound the number of out-of-cone matches.

\begin{lemma}
    The probability that a given man or woman has an out-of-cone match is at most
    $\frac { k e^{-\beta k} } {2a \alpha}$.
    If $\alpha=e^{-\beta k/2}$, this bound becomes $\frac { k e^{-\beta k/2} } { 2a}$.
\end{lemma}
\begin{proof}
    The probability that a man $m$ with public rating at least $a\alpha$ has no match with a woman in or above his cone is at most $e^{-\beta k}$.
    So he can have a match with a woman below his cone with probability at most $e^{-\beta k}$.
    The probability that woman $w$ has an edge to a man $m$ above her cone is $\tau$, and every such man has public rating at least $a\alpha$.
    Consequently, the expected number of edges from $w$ to unmatched men above her cone is at most
    $\tau e^{-\beta k}n$, and therefore by Markov's inequality, the probability that there are one or more edges
    to men above her cone is at most $\tau e^{-\beta k}n$, and clearly this is an upper bound on the probability of a match
    above her cone. Now recall that $\tau= \tfrac {k} {2a\alpha n}$, yielding the stated bound for the women.

    The same argument applies to the men. 
\end{proof}

\begin{corollary}\label{cor::failure-prob-no-men-idio}
Consider a run of the woman-proposing DA in the setting in which men have no private values.
The probability that a man or woman with public rating at least $a\alpha$ has no match is at most
$e^{-\beta k} + \frac {\lambda k e^{-\beta k/2} } {(1-\lambda) 2a}$.
\end{corollary}

Now we are ready to analyze the top-$k$ strategy.
We need to review the proof of \Cref{lem::men-no-match-prob-thresh-str}.
One way to view the top-$k$ strategy is that each woman $w$ has her own threshold $\tau_w$, namely the largest value
which causes her to select exactly $k$ proposals (recall that we assume that for any given woman there are no ties in her private values, which we can safely do as this is a zero probability event).
This affects the bound in \eqref{eqn::bound-man-no-match}.
It becomes $\prod_{w\in S} (1-\tau_w)$ rather than $\prod_{w\in S} (1-\tau)$.
We will show that these two bounds are similar.
\begin{lemma}\label{lem::top-k-no-match-prob-men-no-idio}
    Consider a run of the double-cut woman-proposing DA in the top-$k$ setting.
    Suppose that neither ${\cal B}_1$ nor ${\cal B}_2$ occur.
    Then the probability that a man $m$ with public rating at least $a\alpha$ remains unmatched is at most .
\end{lemma}
\begin{proof}
 
    Let $r_w$ be the number of men in woman $w$'s cone beside man $m$.
    Because neither ${\cal B}_1$ nor ${\cal B}_2$ occur, 
    $r_w\le (2a+1)\alpha (n-1)$. To have a threshold which includes $k$ of these men, in expectation we would need
    the threshold to be $k/r_w$. If the threshold were $k\cdot(1-\delta)/r_w$, then the expected number of men above the
    threshold would be less than $k\cdot(1-\delta)$.
    By a Chernoff bound, the probability that $k$ of these men are above the threshold is given by
        \begin{align*}
        \exp \Big(- \frac {\delta^2k}{3(1-\delta)}  \Big).
    \end{align*}
    Setting $\delta = \big(\tfrac {6c}{k}\big)^{1/2}$, gives a probability of at most $1/e^c$.
    Therefore, the probability that $w$ makes a proposal to $m$ is at most
    \begin{align*}
        &\sum_{c\ge 1} \Big(\frac 1{e^{2(c-1)}} - \frac 1 {e^{2c}}\Big)\cdot \frac {k}{(2a+1)\alpha (n-1)} \cdot \Big[1 - \Big(\frac {6c}{k}\Big)^{1/2}\Big] \\
        &~~~~\le \frac k{(2a+1)\alpha (n-1)}\cdot \Big[1 -\sqrt{\frac 6{k}}\cdot \frac {e^2}{e^2-1} \Big].
    \end{align*}
    Recalling that $s \ge b\alpha n$ as ${\cal B}_2$ does not occur, we conclude that the probability there is no proposal to $m$ is at most
    
    \begin{align*}
        &\Big[1 -  \frac k{(2a+1)\alpha (n-1)}\Big]\cdot \Big[1 -\sqrt{\frac 6{k}}\cdot \frac {e^2}{e^2-1}\Big]^{b\alpha n} \\
        &~~~~\le \exp\Big(-k\cdot\frac{b}{2a+1}\Big[1 -\sqrt{\frac 6{k}}\cdot \frac {e^2}{e^2-1}\Big]\Big).
    \end{align*}
\end{proof}

\subsection{large capacity}

\begin{lemma}\label{lem::large-cap-in-cone-women}
    Suppose each man has capacity $c$, with $ck=\Omega(\ln n)$. Then, with high probability, the DA algorithm run using edges from the women to all men results in each woman, aside those in the bottommost $a\alpha$ range, having an in cone match with probability at least $1 - e^{-\beta k}$.
\end{lemma}
\begin{proof}
    In the woman proposing DA, the men, apart from the bottommost $a\alpha$ range are all matched with high probability \rnote{compute probability as a function of $ck$.}, using only in-cone and possibly edges from women above their cones. As this is the worst stable matching for the men, this means that they are all matched in the man proposing DA also, with the same or better edges. This implies that in the man-proposing DA, the women who are matched use either in-cone edges, or edges from men below their cone. But the double cut DA ensures that each woman, except the bottommost $a\alpha$ range, is matched using in-cone edges or edges to men above their cone with probability at least $1- e^{-\beta k}$, which implies that each of them is matched in-cone with probability at least $1- e^{-\beta k}$.
\end{proof}

\begin{lemma}\label{lem::large-cap-in-cone-men}
    Suppose each man has capacity $c$, with $ck=\Omega(\ln n)$. Then, with probability $1- e^{-\beta k/3}$ \pj{$\beta ck$ instead of $\beta k$ ?}, the DA algorithm run using edges from the women to all men results in all the men, aside those in the bottommost $a\alpha$ range, being fully matched in cone, assuming the cone value range is $de^{-\beta k/3}$, for a suitable constant $d>1$.
\end{lemma}
\rnote{It may be possible to improve the constant.}
\begin{proof}
 We first observe that in each interval $I$ of woman of value range $e^{-\beta k/3}$, above the bottommost $a\alpha$ range,
 by Markov's inequality,
 the number of unmatched women is at most $|I|\cdot e^{-\beta k/3}$, with probability at least $1-e^{-2\beta k/3}$,
 as the expected number of unmatched women is at most $|I|\cdot e^{-\beta k}$.
 Thus, over any interval of women above the bottommost $a\alpha$ range formed by a union of the intervals with range $e^{-\beta k/3}$, the number of unmatched women is at most $n\cdot e^{-\beta k/3}$, with probability at most
 $e^{-\beta k/3}$.

 This means that in computing the surplus, we need to exclude at most $2n \cdot e^{-\beta k/3}$ unmatched women. \rnote{Plus a correction term to account for the variance between the expected and actual number of women in an interval of length $e^{-beta/3}$.} \rnote{There is also a high probability term for the men's matches which needs to be accounted for.}
\end{proof}


\newpage
\rnote{This is old.
}
We turn to the man-proposing version of the double-cut DA.

\begin{proof}
    We will upper bound the probability that woman $w$ receives no proposals. Again, we fix all private values except those concerning woman $w$, i.e.\ of all men for $w$ and of $w$ for all men. The possible computations are governed by a private value cutoff $1-\mu$ for the men's proposals in the double-cut DA and a cutoff $1-\tau$ on the women's private values which determines whether the edge is present and hence available for the men to propose.

    Now, at each possible utility value for a man $m$, there are two reasons it might not propose to $w$: it could be that its private value is smaller than needed for a proposal to $w$ at this point, or it could be that $w$ did not have a edge to $m$. This is now going to lead to a tree of possible computations with no proposals to $m$.

    Now, on each path, for each man, there will be a sequence of nodes corresponding to proposals to women other than $w$,
    in decreasing utility order. In addition, immediately before a node corresponding to a proposal by $m$ to some $w_j\ne w$, there will be a node $v$ corresponding to a potential proposal by $m$ to $w$; there are two edges descending from $v$:
    one, of type 1, has probability $\frac {1 - \sum_{1\le i \le j} \delta_{mi}} { 1 - \sum_{1\le i \le j-1} \delta_{mi} }$, corresponds to $m$ having a lower utility for $w$ than for $w_j$; the second, of type 2, has probability $(1-\tau)\frac {\delta_{mj}} { 1 - \sum_{1\le i \le j-1} \delta_{mi} }$ corresponds to $m$ having a private value in the right range, but $w$ having too low a private utility. The third possibility is that $m$ proposes to $w$, which happens with probability
    $\delta_{mj}\cdot \tau$.

    We call the path in which the first choice is always made the level 0 path (this corresponds to $\widetilde{P}$ in the previous proof). As before, the probability of being on $\widetilde{P}$ is at most $\exp\big(-\beta ks/(2a\alpha n)\big)$, for a suitable constant $\beta >0$.

    Let us say a path is at level 1 if it has one edge of type 2. If man $m$ provides the type 2 edge, the probability weight of these paths is at most 
    \begin{align*}
       (1-\tau)\cdot \exp\big(-\beta k(s-1)/(2a\alpha n)\big)\cdot \sum_j \delta_{mj}
       = (1-\tau)\mu\cdot \exp\big(-\beta k(s-1)/(2a\alpha n)\big).
    \end{align*}
    Summing over all the surplus men, this gives an upper bound of 
    \begin{align*}
        (1-\tau)s \mu \cdot \exp \big(-\beta k(s-1)/(2a\alpha n)\big)
        & \le (1-\tau)s\mu\cdot \exp(k/(2a\alpha n)) \cdot \exp \big( -\beta ks/(2a\alpha n) \big).
    \end{align*}
    
  We define $\nu= (1-\tau)s\mu\cdot \exp(k/(2a\alpha n))$.

    Similarly, if there are two edges of type 2, provided by men $m$ and $m'$, we get an upper bound of
    $\nu^2\cdot \exp\big(-\beta ks/(2a\alpha n)\big)$. And for $h$ edges of type 2, the bound becomes
    $\nu^h\cdot\exp\big(-\beta ks/(2a\alpha n)\big)$. Summing over all $h$ gives an overall upper bound of
    $\nu \cdot\exp\big(-\beta ks/(2a\alpha n)\big)/(1-\nu)$.
\end{proof}


\hide{
We consider two settings, which we refer to as the public school and the medical settings, respectively.
In the public school setting, the men's preferences (corresponding to schools) are all the same; i.e.\ they are only based on the women's public ratings (one can also view this as setting $\lambda=1$.
The women (corresponding to students and/or their parents) have a preference which results from 3 values all chosen uniformly at random from the range $[0,1]$. The first value is the men's public rating; the second is the woman's private value for the man prior to an interview; the third is an additional private value, which we call the interview value,
determined after the interview. Also, there are two global parameters, $\lambda$ and $\mu$, with a woman $w$'s value for man $m$ being calculated as $\lambda r_m + \mu v(w,m) + (1-\lambda -\mu) x(w,m)$, where $v(w,m)$ is $w$'s private value for $m$, and $x(w,m)$ is her incremental post-interview value for $m$. Note that this value is calculated only if $m$ interviews $w$.
In the medical setting both parties have all three values.
\rnote{Maybe drop the private values for the men.}


We will show by induction that each consecutive interval $I$ of value range $2a\tau n$, excluding the bottommost
$a\tau n$ agents, has at most
$|I|\cdot e^{-\beta k/3}$ unmatched agents with failure probability $e^{-2\beta k/3}$.
Hence if $\tau = e^{-\beta k/3}$, excluding the bottommost
$a\tau n$ women, there are at most $ne^{-\beta k/3}$ unmatched women, with
failure probability $e^{-\beta k/3}/2a$; and similarly for the men.
\rnote{The constants may need to be changed.}

\subsection*{Comments, Sept 19}
\rnote{Two observations.}

\begin{itemize}
    \item I think we don't need the elaborate subtraction of out-of-cone matches, because we don't actually need a polynomially small error bound. Instead, we measure the non-matches one cone-full at a time, using non-overlapping cones. For each cone-full we can use the Chebyshev inequality to get a reasonable bound on the failure probability, and then a union bound to get a bound on the number of mismatches above the current man or woman.
    \item When we add in the interview preferences, I think the mismatch probability goes to $1/\sqrt k$. This means that the cone size should be $\Theta(1/\sqrt k)$ I think. So now the way I am thinking about the women is that typically their private score is determining which men they propose to, and the interview score is determining the order of their proposals.
\end{itemize}
}

\newpage
\section{New analysis, October 1}
\rnote{Not completed}

In this section we consider the setting with interviews.
We model a woman $w$'s utility for a man $m$ as $\lambda r(m)+ \mu v(w,m) + \phi i(w,m)$, with $\lambda+\mu+\phi=1$,
where $r(m)$ is man $m$'s public rating, $v(w,m)$ is $w$'s idiosynchratic additional value for man $m$,
and $i(w,m)$ is $w$'s additional post-interview value for $m$, assuming there is an interview.
The parameters $\lambda$ and $\mu$ are chosen so that each of these contributions is non-negative.
We will have two models of a man's utility for a woman.
In the first one, the man's utility is simply $r(w)$, $w$'s public rating.
This corresponds to the K-12 school admissions, where the school's choice is governed by known attributes of the student:
their lottery number, their proximity to the school, diversity requirements, etc.
In the second one, the man's utility is given by $\eta r(m) + (1-\eta)i(m,w)$, where $i(m,w)$ is $m$'s additional post-interview value for $w$, with $0\le \eta\le 1$. This corresponds to the medical school setting, where both sides rate the other. The reason for the women having three components to their scores is that they choose where to seek interviews based on the values $r(m)$ and $v(w,m)$, but the men (hospitals) have no choice here, and it does not seem worthwhile to have two distinct idiosynchratic terms (though this does affect the distribution of the utilities).

For simplicity, in the analysis that follows we consider the case that $\lambda=\mu =\tfrac 13$, and $\eta = \tfrac 12$,
and we rescale the utilities to be $r(m) +v(w,m)+i(w,m)$ and $r(w)+i(m,w)$, respectively.

We consider two rules for selecting the interviews. In the first rule, each women $w$ interviews with a subset of men in her cone, the men with public rating in the range $[r(w)-a\alpha,r(w)+a\alpha)$, for a suitable $\alpha>0$. 
The subset is chosen to have expected size $k$ and consists of the men $m$ for whom $w$'s private score is at least $1-\tau$. Except toward the ends of the rating range, this implies setting $\tau=2ak\alpha$.
The second rule each women chooses the $k$ men in her cone for which she has the highest private values.

We begin by showing that with good probability a man with public rating at least $3a\alpha$ will receive a proposal.
This is mainly to provide intuition for our full construction.

We will be analyzing the outcomes of the woman-proposing and the man-proposing double-cut DA.
An important notion is that of the surplus.

\begin{definition}\label{def::surplus}
    Consider a run of the woman-proposing double-cut DA in which $x$ men and $y$ women participate.
    Suppose the goal is to lower bound the number of proposals to man $m$. Suppose that $z$ women above $m$'s cone are unmatched. Then the surplus $s=y-x-z+1$, the number of women, minus the unmatched women, minus the men other than man $m$. 

    Sometimes we wish to lower bound the number of proposals to the men in an interval $I$.
    If there are $g$ men in the interval, then is this case the surplus $s$ is given by $s=y-x-z+g$.

    Analogous definitions apply to the man-proposing double-cut DA.
\end{definition}

\begin{lemma}\label{lem::one-man-prop-bound}
    Let $m$ be a man with public score $r(m) \ge 3a\alpha$ and let $c(m)< r(m)+2$ be the cutoff utility for the woman-proposing double-cut DA.
    Let $\psi$ be the probability that
    each woman in the woman-proposing double-cut DA has an edge to $m$ which provides her utility at least $c(m)$, the cutoff utility.
    Let $p(s,r)$ be the probability that $s$ women each applying independently to $m$ with probability $\psi$ will make at most $r$ proposals to $m$.
    Suppose there is a surplus of $s$ women in the woman-proposing double-cut DA. Then, the failure probability, the probability that $m$ receives at most $r$ proposals in a run of the woman-proposing double-cut DA, is at most $p(s,r)$.
\end{lemma}
\begin{proof}
We prove this bound holds regardless of the private values of the women for men other than $m$, and of the men other than $m$ for all the women. So let's fix all these private values. We start by eliminating the zero probability events that a woman has the same private value for any two men, or that a man has the same private value for any two women. Clearly, these zero probability events are not going to affect our final bound on the probability that $m$ receives no proposal.

It will be helpful to define a tree $T$ which will represent the possible computations of the double-cut DA. 
These computations depend only on $m$'s private values and on the private values of the women for $m$.
Each random choice of these private values defines a computation path. To make these paths unique, whenever two or more women could make a proposal, we let the one with lower rank proceed.

There will be two types of nodes in $T$. Those that correspond to proposals made to men other than $m$, and those that correspond to possible proposals to $m$, which depend on the random choices of the private values for $m$.
Note that the first type of node represent actions that are fully determined, as both the private values for these men and the private values of these men are already fixed. Each node of the second type  will cover a limited range of utility values for a single woman, and it can have two outcomes corresponding to the two edges that will descend from the node: one edge corresponds to a proposal to $m$ with utility in the specified range, the other to there being no proposal to $m$ with
a utility in this range.

Let's make this more precise.
Consider the actions of a single woman $w$. Suppose $w$'s utilities for the men other than $m$, which are above the cut at $c(m)=r(m)-b\alpha$, are $u_1>u_2>\ldots>u_t$. On each computation path $P$, there will be a subsequence of up to $2t$ nodes corresponding to $w$'s actions. Let $x_1,x_2,\ldots,x_q$ be the type 1 nodes in this subsequence, in the order in which they appear along $P$.
$x_i$ corresponds to the proposal that provides $w$ utility $u_i$. 
To identify the type 2 nodes,
suppose that $u_h\ge r(m)+1> u_{h+1}$ (if either of these is missing, we take $u_0=r(m)+1$ and $u_{t+1}=r(m)+1-b\alpha$). We introduce additional nodes $y_{h+1},y_{h+2},\ldots, y_{q}$; $y_i$ has two children, one corresponding
to $w$ making a proposal to $m$ with utility in the range $(u_{i+1},u_i)$, and one corresponding to not making a proposal to $m$ with utility in this range. Note that on the path on which $y_i$ made a proposal to $m$ with utility in the range
$(u_i,u_{i+1})$, this is the last action taken by $m$ in this run of the double cut DA, i.e.\ in the computations in the subtree rooted at the relevant child.

On each path $P$, the nodes $x_i$ over all the women $w$ participating in the double cut DA are arranged in the order in which they would occur in the corresponding run of the double cut DA. Each node $y_i$ is placed immediately above the corresponding $x_i$.

We now want to upper bound the probability that $m$ receives at most $r$ proposals from the computation continuing from each node $v$ in the tree $T$, which we will do by means of a bottom-up inductive argument on the tree $T$.
To this end, we define the residual proposing probability for woman $w$ at a node $v$ who has not yet proposed
to $m$ as follows:
her residual probability, $p(w,v)$, is given by the probability that she has an edge to $m$ providing utility
in the range $(c(m),u)$,
where the nearest type 2 node for node $w$ above $v$ had utility range $(u,u')$, and if there is no such
node, it is given by $(c(m),r(m)+2)$. 

Suppose there have been $x = x(v)$ proposals to $m$ on the path to $v$,
Let $p_1\le p_2\le \ldots \le p_{s-x}$ be the $s-x$ smallest residual probabilities at node $v$.
Suppose $r>x$, and suppose there are $s-x$ independent attempts to propose to $m$ with respective
probabilities $p_1,p_2,\ldots,p_{s-x}$. Let $\qtilde(v)$ be the probability that these attempted proposals yield
at most $r$ actual proposals. If $r\le x$, we define $\qtilde(v)=0$.
Let $q(v)$ be the probability that in the subtree rooted at $v$ at most $r-x$ proposals to $m$ are made if $r>x$, and otherwise $q(v)=0$.
 

\begin{claim}\label{clm::indpt-is-worst}
For every node $v$ in $T$, $q(v)\le \qtilde(v)$.
\end{claim}
\begin{proof}
We prove this result by induction.

\smallskip\noindent
\emph{Base case}: A leaf node.\\
If there have been more than $r$ proposals to $m$, then $q(v)=\qtilde(v)=0$.
If there had been $x\le r$ proposals, as there are at least $s$ surplus women, at least $s-x$ of them can still propose to $m$ with their residual probability, and these are all independent actions.
Suppose these residual probabilities are $q_1\le q_2\le\ldots\le q_{s-x}$.
These $s-x$ attempted proposals result in a probability $q\ge q(v)$ of at most $r-x$ additional proposals to $m$, as in the actual computation leading to this leaf there may be more that $s$ surplus women, which potentially causes more proposals to $m$.
Attempting to propose with the $s-x$ smallest residual probabilities, $p_1\le p_2\le \ldots \le p_{s-x}$,
yields a probability $\qtilde(v)$ of at most $r-x$ additional proposals to $m$, and as these are the smallest
residual probabilities, $\qtilde(v)\ge q\ge q(v)$.

\smallskip\noindent
\emph{Inductive step}.
\\
\emph{Case 1}.  A node $v$ with a single child $v'$.\\
Clearly, $q(v)=q(v')$ and $\qtilde(v)= \qtilde(v')$. So the result holds at node $v$ given it holds at $v'$.

\smallskip\noindent
\emph{Case 2.} A node $v$ with children $\vl$ and $\vr$.\\
Let $w$ be the woman choosing whether to propose to $m$ at node $v$, and suppose $\vl$ is the node reached
if she makes this proposal. Suppose further that the edge to $\vl$ is taken with probability $\delta$ and
the edge to $\vr$ with probability $1-\delta$.
Clearly, $q(v)= \delta\cdot q(\vl) + (1-\delta)q(\vr)$.
We now show that $\qtilde(v)\ge \delta\cdot \qtilde(\vl) + (1-\delta)\qtilde(\vr)$, and therefore by induction, $\qtilde(v) \ge \delta\cdot q(\vl) + (1-\delta)q(\vr) = q(v)$.

Recall that $p_1(v)\le p_2(v)\le\ldots\le p_{s-x}(v)$ are the $s-x$ smallest residual probabilities which are used to evaluate $\qtilde(v)$, and similarly $p_1(\vr)\le p_2(\vr)\le\ldots\le p_{s-x}(\vr)$ are the $s-x$ smallest residual probabilities which are used to evaluate $\qtilde(\vr)$.

\smallskip\noindent
Case 2.1.  $\{p_1(\vr),p_2(\vr),\ldots,p_{s-x}(\vr)\}$ includes the residual probability $p(w,\vr)$ for $w$ at node $\vr$.\\
Case 2.1.1. $\{p_1(v),p_2(v),\ldots,p_{s-x}(v)\}$ includes the residual probability $p(w,v)$ for $w$ at node $v$.\\
One way to calculate $\qtilde(v)$ is to determine whether $w$ proposes to $m$ in two steps:
first, with probability $\delta$, we decide if $w'$ private value for $m$ is in the range that causes a move to $\vl$;
if so, the residual probabilities $\{p_1(v),p_2(v),\ldots,p_{s-x}(v)\}\setminus\{p(w,v\}$ are used to compute $\qtilde(\vl)$; 
if not, the move is to $\vr$, and the residual probabilities $p_1(v),p_2(v),\ldots,p_{s-x}(v)$, with $p(w,v)$ replaced by
$p(w,\vr)$, are used to compute $\qtilde(\vr)$; but $p(w,\vr)$ is the probability that $w$ has a proposal to $m$ after the possible range for its private value has been reduced by the range that enabled a move to $\vl$.

These residual probabilities yield proposing probabilities
$\qtilde(\vl)$ and $\qtilde(\vr)$ at nodes
$\vl$ and $\vr$, respectively; since these nodes are reached with probabilities $\delta$ and $1-\delta$,
the resulting probability at node $v$ therefore equals $\delta\cdot \qtilde(\vl) + (1-\delta)\qtilde(\vr)$.

\smallskip\noindent
Case 2.1.2.  $\{p_1(v),p_2(v),\ldots,p_{s-x}(v)\}$ does not include the residual probability $p(w,v)$ for $w$ at node $v$\\
We reduce this case to case 2.1.1 as follows. Suppose we increased $p_{s-x}$ so that it became larger than $p(w,v)$.
Then this setting would be an instance of case 2.1, and the modified $\qtilde(v)$, would equal 
$\delta\cdot \qtilde(\vl) + (1-\delta)\qtilde(\vr)$.
Now consider reducing $p_{s-x}$ to its actual value; the effect on the probability of at most $r-x$ proposals is only to increase it, as the only change is for one of the proposal attempts to occur with reduced probability.
Therefore $\qtilde(v)\ge \delta \qtilde(\vl) + (1-\delta) \qtilde(\vr)$, in this case too.

\smallskip\noindent
Case 2.2.  $\{p_1(\vr),p_2(\vr),\ldots,p_{s-x}(\vr)\}$ does not include the residual probability $p(w,\vr)$ for $w$ at node $\vr$.
\\
Then $\{p_1(v),p_2(v),\ldots,p_{s-x}(v)\}$ does not include the residual probability $p(w,v)$ for $w$ at node $v$,
as $p(w,\vr) < p(w,v)$.

We reduce Case 2.2 to Case 2.1.2, as follows.
Imagine reducing both $p(w,\vr)$ and $p(w,v)$ so as to maintain the $\delta$ to $(1-\delta)$ probability split
between choosing to move to  $\vl$ and to $\vr$, stopping when
$p(w,\vr)$ is reduced to $p_{s-x}$. This leaves $\qtilde(v)$ unchanged, so the bound from case 2.1.2 applies.

\hide{
We note that $\qtilde(\vr)=\qtilde(v)$ as these two terms are evaluated with the same residual probabilities,
and $\qtilde(\vl)\ge\qtilde(v)$ for
\begin{align*}
&\qtilde(\vl)=\Pr\big[\text{at most $r-x-1$ proposals occur when individual proposals occur}\\
&\hspace*{2.5in}\text{with probabilities $p_1\le p_2\le\ldots\leq p_{s-x-1}$}\big],
\end{align*}
while 
\begin{align*}
&\qtilde(v)=\Pr\big[\text{at most $r-x$ proposals occur when individual proposals occur}\\
&\hspace*{2.5in}\text{with probabilities $p_1\le p_2\le\ldots\leq p_{s-x}$}\big].
\end{align*}
But if at most $r-x-1$ proposals occur when the first $s-x-1$ attempts are made, for sure at most
$r-x$ proposals occur after $s-x$ attempts, and therefore $\qtilde(\vl)\le \qtilde(v)$ in this case.
So  $\qtilde(v)\ge \delta \qtilde(\vl) + (1-\delta) \qtilde(\vr)$.
}

\smallskip\noindent
By induction, in every subcase, $\qtilde(v)\ge \delta\cdot \qtilde(\vl) + (1-\delta)\qtilde(\vr)$, and therefore, $\qtilde(v) \ge \delta\cdot q(\vl) + (1-\delta)q(\vr) = q(v)$.
\end{proof}

The overall result follows by applying the claim to the root of $T$.
\end{proof}

It is straightforward to extend this bound to the case that each man has capacity $\kappa$.
We will show that with high probability all but the bottommost men are fully matched in the case that each man has capacity $\kappa=\Omega(\ln n)$ when the parameters $\alpha$ and $c(m)$ are suitably chosen.


\begin{lemma}\label{lem::high-cap-men-outcome}
Suppose that $c(m)=r(m)+2-1/\sqrt{k}$ (using the notation from \Cref{lem::one-man-prop-bound}).
Suppose further that each man has capacity $\kappa$, $\sqrt k\ge 4a+ \frac{k^2}{4a\alpha n}$, and $\kappa\cdot \sqrt k\ge 16a(c+2)\ln n+ \frac{\kappa k^2}{8an}$.
Then, with failure probability at most $n^{-(c+2)}$, each man $m$ with public rating at least $3a\alpha$
received $\kappa$ matches, i.e.\ is fully matched.
\end{lemma}
\begin{proof}
Note that as we allow a drop of $1/\sqrt k$ in the utility from the ideal value of $r(m)+2$, we obtain a proposing probability to $m$ of $\psi=\kappa\tau\Big(\frac1{\sqrt{k}} - \frac{\tau}{2}\Big)$.
Also recall that $\tau= k/2a\alpha n$.

With probability $1/n^{c+2}$, the surplus is at least $\alpha n$.
Therefore the expected number of proposals to $m$ is at least $\psi \alpha n$.
By a Chernoff bound, if these were independent proposals, the probability of $m$ receiving at  most $\tfrac 12 \psi \alpha n$ proposals
would be at most $\exp\big(-\psi\alpha n/8\big)$.
By \Cref{lem::one-man-prop-bound}, this bound applies to the run of the double-cut DA also.
If $\tfrac 12\psi\alpha n\ge \kappa$, $m$ receives at least $\kappa$ proposals and therefore obtains $\kappa$ matches.
The failure probability is at most $n^{-(c+2)}$ if $\psi \alpha n\ge 8(c+2)\ln n$.
Substituting for $\tau$ and $\alpha$, we obtain constraints
\begin{align*}
    &\frac {\psi\alpha n}{2} = \frac{\kappa k}{4a}\cdot\Big(\frac1{\sqrt{k}} - \frac{\tau}{2}\Big) \ge \kappa;\\
    &\text{i.e.}~~~~\sqrt{k} \ge 4a + \frac {k^2}{4a\alpha n}.
\end{align*}
And
\begin{align*}
    &\frac{\kappa k} {2a} \Big(\frac1{\sqrt{k}} - \frac{\tau}{2}\Big) \ge 8(c+2)\ln n;\\
    &\text{i.e.}~~~~\kappa \sqrt k \ge 16a(c+2)\ln n + \frac{\kappa k^2}{8an}.
\end{align*}
\end{proof}

Next, we show a high probability upper bound on the number of unmatched men in an interval $I= (l,l+d)$, where the bottom of the interval is at height at least $a\alpha$.
As before we will be using cones of size $2a\alpha$.
This upper bound on the number of unmatched men will be twice the expected upper bound given by \Cref{lem::one-man-prop-bound}.
Using a union bound will then allow us to deduce a high probability upper bound on the number of
unmatched men in any union of these intervals; we obtain a similar bound on the number of unmatched women.
We use these bounds inductively in descending rank order, to prove the bounds for single intervals. 

To show this result, we need some more notation. A woman $w$ selects edges to men her cone (i.e.\ proposals) with a private value cutoff of $1-\tau$, and we then analyze the number of proposals made with edges which achieve utility at least
$l+2-(\tau+\sigma)$. Note that the term $-(\tau+\sigma)$ bounds the sum of the drop in utility due to the private value of the edge in question plus the drop in utility due to the post-interview value increment.

We begin by establishing low probability bounds on some undesirable events.

\begin{definition}\label{def::no-extreme-intervals}
Let ${\cal B}_I$ be the event that an interval $I$ of men (or women) of length $\ell<1$ has either fewer than $\ell n-\alpha n$ or more than $\ell n + \alpha n$ men (resp.\ women).
\end{definition}

\begin{lemma}\label{lem::no-BI}
Suppose that $\alpha \ge [3(c+2)\ln n/n]^{1/2}$.
Then ${\cal B}_I$ occurs with failure probability at most $2/n^{c+2}$.
\end{lemma}
\begin{proof}
    The expected number of men (or women) in $I$ is $\ell n$.
    By a Chernoff bound, the actual number of men is at most $\ell n -\alpha n$ with probability at most
    $\exp(-\alpha^2 n/2\ell)\le \exp(-(c+2)\ln n) = n^{-(c+2)}$.
    Similarly, the actual number is at least $\ell n +\alpha n$ with probability at most
    $\exp(-\alpha^2 n/3\ell)\le \exp(-(c+2)\ln n) = n^{-(c+2)}$.
\end{proof}

Similarly,
\begin{definition}\label{def::no-extreme-short-intervals}
Let ${\cal B}_J$ be the event that an interval $J$ of men (or women) of length $d$ has either fewer than $dn/2$ or more than $2dn$ men (resp.\ women).
\end{definition}
\begin{lemma}\label{lem::no-BJ}
Suppose that $d \ge [8(c+2)\ln n/n]$.
Then ${\cal B}_J$ occurs with failure probability at most $2/n^{c+2}$.
\end{lemma}
\begin{proof}
    The expected number of men in $J$ is $dn$.
    By a Chernoff bound this is at least $2dn$ with probability at most $\exp(-(8(c+2)\ln n)/3)\le n^{-(c+2)}$,
    and it is at most $dn/2$ with probability at most $\exp(-(8(c+2)\ln n)/8)\le n^{-(c+2)}$.
\end{proof}


\begin{lemma}\label{lem::prob-bound-interval-mismatch}
    Let $I=(l,l+d)$ be a interval of men with public rating range $d=[(c+2)e^{\beta k}\ln n]/n$, and with $l\ge a\alpha$,
    where $e^{\beta k}\ge 8$.
    Let $g$ be the number of men in $I$.
    Suppose that 
    \begin{itemize}
        \item $\alpha \ge [3(c+2)\ln n/n]^{1/2}$,
        \item $a\ge 4$,
        \item $d+\tau\le \alpha/4$,
        \item $\sigma\le \alpha/4$,
        \item $e^{\beta k}\ge 8$, subsuming $\beta k \ge 2$ and $d \ge [8(c+2)\ln n/n]$,
        \item $k\sigma\cdot e^{\beta k}\ge 128$, 
        \item $e^{\beta k} \ge 2 e^{\sigma k/16}$,
        \item $e^{g\tau\sigma}\le \tfrac 32$,
        \item and $n\ge (c+2)^2(2a+1)k^2 e^{2\beta k}\ln^2 n/\alpha$.
    \end{itemize}
    Then, in a run of the woman-proposing DA, the number of unmatched men in $I$ is at most $2ge^{-k\sigma/16}$, with additional failure probability at most $[8/n^{c+2}+1/n^{c+1}]$, assuming inductively that the higher intervals observed this bound also.

    Summing over all $2n/d\le n$ disjoint intervals of men and women, gives an overall failure probability of at most
    $n^{-c}$.
\end{lemma}
\begin{proof}
We begin by excluding the low probability case that the number of men in $I$ is less than half the expectation or more than twice the expectation. By \Cref{lem::no-BJ}, the failure probability is at most $2/n^{c+2}$.

We will run the woman-proposing double-cut DA with a cut at utility $l+2-(\tau+\sigma)$, and at any proposal to a man in $I$.
But we also prevent a few women from participating at all.
Specifically, we eliminate all women that have an edge to a man in $I$ with utility in the range $(l+2,l+d+2)$, and all women that have two or more proposals to men in $I$. This ensures that if there is a proposal with utility $x$ to a man in $I$, it could be to any man in $I$. What this means is that we can view a proposal to a man in $I$ as a proposal to the whole set, and handle it in a way that treats the proposal as being equally likely to be to any man in $I$.
This then allows us to use a lower bound on the number of proposals by these women to men to $I$ to deduce an upper bound on the number of unmatched men in $I$ (both of these statements will be with high probability).

The expected number of women eliminated for having a utility in the range $(l+2,l+d+2)$ is the product of the following terms:
\begin{itemize}
\item 
the number of women in-cone for all the men in the interval $I$, which is the number of women contained in the public rating interval $[l+d-a\alpha,l+a\alpha]$,
which, by \Cref{lem::no-BI}, is at most $(2a+1)\alpha n$ with failure probability at most $1/n^{c+2}$, 
\item 
the number of men in the interval $[l,l+d]$,
which, by \Cref{lem::no-BJ} is at most $2dn$ with failure probability at most $1/n^{c+2}$,
\item 
the probability that there is an edge between a specified man and woman, namely
$k/2a\alpha n$, 
\item
the probability $d$ that the interview increment to the utility ensures an overall utility in the range $(l+2,l+d+2)$,
conditioned on the idiosyncratic utility being at least $1-\tau$,
\end{itemize}
namely,
\begin{align*}
    (2a+1)\alpha n \cdot 2dn\cdot \frac{k}{2a\alpha n} \cdot d
    &= \frac {4(2a+1)}{2a}d^2n
    \le 5(c+2)^2 e^{2\beta k}\ln^2 n,
\end{align*}
as $a\ge 4$.
This brings the running total on the failure probability to $4/n^{c+2}$.

By a Chernoff bound, the number of women eliminated is at most
$10(c+2)^2 e^{2\beta k}\ln^2 n$,
with failure probability $\exp(-5(c+2)^2 e^{2\beta k}\ln^2 n/3) \le 1/n^{c+2}$, if
$(c+2) e^{2\beta k}\ln n\ge \tfrac 35$, which holds as $\beta k > 0$.
Now the running total on the failure probability is $5/n^{c+2}$.

The number of women eliminated for having two proposals into $I$ is at most the number of women in-cone for all the men in the interval, times the number of choices of pairs of men in the interval,
which, by \Cref{lem::no-BJ} is at most $(2dn)^2$ (note the failure probability for this event was counted in the itemized list above), times the probability that there are edges from any one woman to both these men, namely,
$(k/2a\alpha n)^2$, yielding the following bound on this number:
\begin{align*}
  (2a+1)\alpha n \cdot \frac{(dn)^2}{2} \cdot \Big(\frac{k}{2a\alpha n}\Big)^2
  &\le \frac{(2a+1)k^2d^2n}{\alpha}\\
  & \le \frac{(2a+1)k^2 (c+2)^2e^{2\beta k}\ln^2 n}{\alpha n}
  \le 1,
\end{align*}
if $n\ge (c+2)^2(2a+1)k^2 e^{2\beta k}\ln^2 n/\alpha$.
Therefore, by a Chernoff bound, at most $(\ln (c+2) n)/\ln 2$ women are eliminated, with failure probability $1/n^{c+2}$.
Now the running total on the failure probability is $6/n^{c+2}$.

As we show in \Cref{lem::prob-bound-interval-mismatch-women},
the number of unmatched women in each interval of rating length $d$ is at most $2g e^{-\beta k}$ with failure probability
$1/n^{c+2}$. So above the intersection of the cones for the men in $I$, the number of unmatched women is at most
$2ne^{-\beta k}$ with probability at most $1/n^{c+1}$.
Now the running total on the failure probability is $6/n^{c+2}+1/n^{c+1}$.

Therefore the surplus $s$ is at least the number of women in or above the cones for all men in $I$,
i.e.\ with public rating at least $l+d-a\alpha$, which is at least $[1-l-d+(a-1)\alpha]n$ women,
minus the number of men above the cut, namely those with
public rating at least $l-(\tau+\sigma)$, which is at most $[1-l+\tau+\sigma+\alpha]n$ men,
minus the number of unmatched women above the cones for all men in $I$,
minus the number of eliminated women.
This is lower bounded by
\begin{align*}
&\big[(1-l-d+(a-1)\alpha) - (1-l+\tau+\sigma+\alpha) - 2e^{-\beta k}\big]n - 2(c+2)^2 e^{2\beta k}\ln^2 n -(\ln (c+2) n)/\ln 2 +g \\
&~~~~\ge (a-3)\alpha n \ge  \alpha n,
\end{align*}
if  $a\ge 4$, $d+\tau\le \alpha/4$, $\sigma\le \alpha/4$, $2e^{-\beta k}\le \alpha/4$, $2(c+2)^2 e^{2\beta k}\ln^2 n\le \alpha n/4$, and $g\ge (\ln (c+2) n)/\ln 2$; 
the third condition is satisfied as $n\ge (c+2)^2(2a+1)k^2 e^{2\beta k}\ln^2 n/\alpha$ and $a\ge 4$, and
the last condition is satisfied
if $\tfrac 12(c+2)e^{\beta k}\ln n \ge (\ln (c+2) n)/\ln 2$, which is satisfied if $n \ge c+2$, and
$\tfrac 14 \ln 2\cdot (c+2)\cdot e^{\beta k}\ge 1$, which holds as $\beta k\ge 2$.

Now the bound from \Cref{lem::one-man-prop-bound} applies with I replacing the single man $m$.
% and with the probability of a proposal into $I$ increased by a factor of $g\ge \tfrac 12 e^{\beta k}\ln n$. 
The expected number of proposals to $I$ is calculated as follows:
an edge from a woman $w$ is present with probability $\tau=k/2a\alpha n$ and
it is used if its utility is in the range $(l+2-\tau-\sigma, l+2)$; note that for each possible private value, there is a probability $\sigma$ that the interview value yields a utility in this range, which gives a probability of $\tau\cdot \sigma$. But the overall probability has to be reduced to account for the possibility of
two or more such edges from $w$ into $I$, which occurs with probability
\begin{align*}
\sum_{i\ge 2} i\cdot {g \choose i} (\tau\sigma)^i \le \sum_{i\ge 2}(g\tau\sigma)\frac{(g\tau\sigma)^{i-1}}{i-1} \le g\tau\sigma e^{g\tau\sigma}\le \tfrac 32 g\tau\sigma, 
\end{align*}
if $e^{g\tau\sigma}\le \tfrac 32$.
Then the expected number of edges is at least $\tfrac12 sg\tau\sigma$.
Now,
\begin{align*}
\frac 12 sg\tau\sigma &\ge \frac a4 \alpha n \cdot g \cdot \frac {k}{4a\alpha n}\cdot \sigma
\ge \frac{kg\sigma}{8}.
\end{align*}
By \Cref{lem::one-man-prop-bound}, applying a Chernoff bound, 
shows that the number of proposals is at least $r=\tfrac{kg\sigma}{16}$ with failure probability at most
$p(s,r)=\exp(-kg\sigma/128)\le \exp(-ke^{\beta k}\sigma(c+2)\ln n/128)\le n^{-(c+2)}$, if $k\cdot e^{\beta k}\sigma\ge 128$.
Now the running total on the failure probability is $7/n^{c+2}+1/n^{c+1}$.

As the proposals into $I$ that we are considering are uniform over $I$, this amounts to a balls and bins problem.
The question we are asking is how many bins remain empty. In expectation, a bin is empty (i.e.\ a man is unmatched)
with probability at most $e^{-k\sigma/16}$, and so in expectation, at most $ge^{-k\sigma/16}$ bins are empty.
Now, as the indicator variables for whether a bin is empty are negatively correlated, we can apply Chernoff bounds
to this setting, and therefore at most $2ge^{-k\sigma/16}$ bins are empty with failure probability at most
$\exp(-2ge^{-k\sigma/16}/3)\le n^{-(c+2)}$, if $e^{\beta k} e^{-k\sigma/16} \ge 3$.
Now the running total on the failure probability is $8/n^{c+2}+1/n^{c+1}$.
\end{proof}

Next, we need to obtain similar bounds on the numbers of unmatched women.

\begin{lemma}\label{lem::one-woman-prop-bound}
    Let $w$ be a woman with public score $r(w) \ge 3a\alpha$ and let $c(w)< r(w)+1$ be the cutoff utility for the double-cut DA.
    Let $\psi$ be the probability that
    each man in the man-proposing double-cut DA has an edge to $w$ which provides him utility at least $c(w)$, the cutoff utility.
    Let $p(s,r)$ be the probability that $s$ men each applying independently to $m$ with probability $\psi$ will make at most $r$ proposals to $w$.
    Suppose there is a surplus of $s$ men in the man-proposing double-cut DA. Then, the failure probability, the probability that $w$ receives at most $r$ proposals in a run of the man-proposing double-cut DA, is at most $p(s,r)$.
\end{lemma}
The proof for this lemma is very similar to the one for \Cref{lem::one-man-prop-bound} and is deferred to the appendix.

Next, we show the analog of \Cref{lem::prob-bound-interval-mismatch} for the man-proposing double-cut DA.

\begin{lemma}\label{lem::prob-bound-interval-mismatch-women}
    Let $I=(l,l+d)$ be a interval of women with public rating range $d=[(c+2)e^{\beta k}\ln n]/n$, and with $l\ge a\alpha$,
    where $e^{\beta k}\ge 8$.
    Let $g$ be the number of women in $I$.
    Suppose that 
    \begin{itemize}
        \item $\alpha \ge [3(c+2)\ln n/n]^{1/2}$,
        \item $a\ge 4$,
        \item $d\le \alpha/4$,
        \item $\sigma\le \alpha/4$,
        \item $e^{\beta k}\ge 8$, subsuming $\beta k \ge 2$ and $d \ge [8(c+2)\ln n/n]$,
        \item $k\sigma\cdot e^{\beta k}\ge 128$, 
        \item $e^{\beta k} \ge 2 e^{\sigma k/16}$,
        \item $e^{g\tau\sigma}\le \tfrac 32$,
        \item and $n\ge (c+2)^2(2a+1)k^2 e^{2\beta k}\ln^2 n/\alpha$.
    \end{itemize}
    Then, in a run of the man-proposing DA, the number of unmatched women in $I$ is at most $2ge^{-k\sigma/16}$, with additional failure probability at most $[8/n^{c+2}+1/n^{c+1}]$, assuming inductively that the higher intervals observed this bound also.

    Summing over all $2n/d\le n$ disjoint intervals of men and women, gives an overall failure probability of at most
    $n^{-c}$.
\end{lemma}
Again, we defer the proof to the appendix as it is very similar to the proof for \Cref{lem::prob-bound-interval-mismatch}.

\hide{
\newpage
\subsection{Making Exactly $k$ Proposals}\label{sec::k-prop-setting}

To carry out some of the analyses for this setting we need to average over all utility values.
We are no longer able to focus on the utilities related to a single man (or interval of men) in the case of the woman-proposing DA with all the other values fixed.
To enable this approach, we discretize the setting for the purposes of analysis, and then take the limit as the
discretization tends to 0 to obtain a result for the continuous setting, as was done in \cite{AgarwalCole2023}.
In this discretization, if a woman (or man) has the same utility for two men (resp.\ for two women), we do not run the double cut DA.

\begin{claim}
\label{clm::discrete-dist}
For any $\delta>0$, there is a discrete utility space in which
for every woman the probability of selecting each man is unchanged or reduced,
and the probability of having any differences
in the sequence of actions in the original continuous setting and the discrete setting is at most $\delta$.
\end{claim}
\begin{proof}
$z\ge n^3/2\delta$ will be an integer in our construction.
We partition the range $[0,3]$ into $3z$ intervals each of length $1/z$.
To do this, we round down each utility to the nearest integer multiple of $1/z$.
Note that for each man $m$, the range of utilities he can provide is given by $[r(m),r(m)+2]$;
on rounding, this creates at most $1+2/z$ possible utilities, each one occurring with probability
at most $1/z$ (to see this consider the random choice of the interview value). Therefore the probability that a woman has the same utility for two men is at most
$\tfrac 12 n(n-1)/z$, and so the probability that any woman has the same utility for two men is at most
$n^2(n-1)/2z\le n^3/2z=\delta$.

We set aside all settings in which a woman has the same utility for any pair of men.

Recall that in the run of double-cut DA, each woman repeatedly makes the next highest utility proposal.
We view this as happening as follows. For each successive discrete utility value, woman $w$ has the following choices.

i. she selects some man 
to propose to (among the men she has not yet proposed to); or 

ii. she takes ``no action''. This corresponds 
to $w$ making no proposal achieving the current utility.
\\
Every run of DA in the continuous setting that does not have a woman selecting two men over the course of a single
utility interval will result in the identical run in the discrete setting in terms of the order in which each
woman proposes to the men.
\end{proof}
Let ${\cal B}_8$ be the event that some woman has the same utility for a pair of men.
By \Cref{clm::discrete-dist}, ${\cal B}_8$ occurs with probability at most $\delta$.

We need some additional parameters. $1-\overline{\tau}$ is a lower bound on the value probability which ensures
that with high probability each woman will have $k$ edges in her cone that all have private value at least
$-1\overline{\tau}$. $1-\overline{\psi}$  is a lower bound on the interview value that we use to help ensure that
the women have only a small loss. More specifically, we will ensure that with a good probability, a non-bottommost woman $w$ will obtain a match that provides her utility at least $r(w)+2-\overline{\tau}-\overline{\psi}$.
By choosing the cone size and $\psi$ appropriately, we will ensure that for the non-bottommost women,
in expectation, the only improving deviations from the recommended strategy would be in-cone, and as a result any deviation, in expectation, will provide modest gains at best.

\begin{lemma}\label{lem::value-of-taubar}
    Let $b>2$ and $c>0$ be constants.
    Suppose $\taubar\ge \frac{b\kappa(c+2)\ln n} {(2a-\frac 12)\alpha n}$. Then, with failure probability at most $n^{-(c+2)}$, if $k \le \Big(1-\sqrt{\frac 2b}\Big) (c+2)\ln n$,
    every woman has at least $k$ in-cone edges with private value $1-\taubar$ or larger.
\end{lemma}
\begin{proof}
    Let $w$ be a woman. The expected number of $w$'s in-cone edges with private value $1-\taubar$ or larger
    is at least $\taubar$ times the number of men in her cone, i.e.\ $\taubar (2a-\tfrac12)\alpha n/\kappa$.
    As $\taubar \ge \frac{b\kappa(c+2)\ln n} {(2a-\frac12)\alpha n}$, then, by a Chernoff bound, the probability that she
    has fewer than $k$ such edges is at most $\exp\Big[-\tfrac b2 (c+2)\ln n \big(1 - \frac k{(c+2)\ln n}\big)^2\Big]
    \ge n^{c+2}$, if $k \le \Big(1-\sqrt{\frac 2b}\Big) (c+2)\ln n$.
\end{proof}
Let ${\cal B}_7$ be the event that some woman has fewer than $k$ in-cone edges with private value $1-\taubar$ or larger.

Let ${\cal B}_6$ be the event that in the discretization of \Cref{clm::discrete-dist}, a women has the same rounded utility for two men.

Now we show that in the discrete setting, if none of ${\cal B}_6$ , ${\cal B}_7$, or ${\cal B}_8$ occur, then each man will receive $\kappa$ proposals with high probability. 


\begin{lemma}\label{lem::high-cap-men-outcome}
Suppose that none of ${\cal B}_6$, ${\cal B}_7$, or ${\cal B}_8$ occur.
Suppose that $c(m)=r(m)+2-\taubar -\psibar$ (using the notation from \Cref{lem::one-man-prop-bound}).
Suppose further that each man has capacity $\kappa$, the surplus $s\ge \alpha n$, and
$\frac12 \alpha n\psi \big[1 - \frac {\kappa}{s\psibar}\big]^2 \ge (c+2)\ln n$.
Then, with failure probability at most $n^{-(c+2)}$, each man $m$ with public rating at least $3a\alpha$
received $\kappa$ matches, i.e.\ is fully matched.
\end{lemma}
\begin{proof}
We build a tree $T$ to represent the possible runs of the double-cut DA, but now nodes will have high degree.
Each node corresponds to an action by a particular woman at her current utility: the action consists of her doing one of the following:
\begin{itemize}
    \item She proposes to some man $m'$.
    \item She makes no proposal with the present utility $u$.
    \end{itemize}
As before, let $q(v)$ be the probability that at node $v$ the continuation of the run of the double-cut DA results in at most $r=\kappa-1$ proposals to man $m$, let $w$'s residual probability at node $v$, $p(w,v)$, be the probability that $w$ proposes to man $m$ in the computation starting at node $v$ if she has not already done so, let $s$ be the minimum surplus over all the possible paths in the computation,
and let $\qtilde(v)$ be the probability that if $x$ women have already proposed to $m$,
then if the $s-x$ women with the smallest residual probabilities propose independently to $m$ with their residual probabilities, it results in at most $r$ proposals to $m$. As before, in \Cref{clm::fixed-k-stoc-dom},
we will show that $\qtilde(v)\ge q(v)$.

Therefore, the probability that $s$ women independently attempting to propose to $m$ at the root $z$ of $T$ produce fewer than $\kappa$ proposals
is an upper bound on the probability that the double-cut DA results in fewer than $\kappa$ proposals to $m$.

But at the root $z$ each of these women has probability at least $\psibar$ of proposing to $m$.
In expectation, they produce at least $s\cdot \psibar$ proposals.
By a Chernoff bound, they produce fewer than $\kappa$ proposals with probability
at most $\exp\Big(-\frac12 s\psi \big[1 - \frac {\kappa}{s\psibar}\big]^2\Big)$.
\end{proof}

\begin{lemma}\label{lem::women-surplus-no-idio}
    Suppose that neither ${\cal B}_1$ or yyy occur. Suppose also that $a\ge 4$.
    Then the surplus $s\ge alpha n$.
    
\end{lemma}
\begin{proof}
    As ${\cal B}_1$ does not occur, the number of men with public value at least $r(w)-\alpha$ is at most
    $[1+\frac 32\alpha-r(w)]n$. Likewise, the number of women with public value at least $r(w)-a\alpha$ is at least
    $[1-r(w) +(a-\frac12)\alpha]n$.
    As yyy does not occur, the number of unmatched women above $m$'s cone is at most $ne^{k\psi/2a}\le \alpha n$.
    Thus the surplus is at least 
    \begin{align*}
        [1+\frac 32\alpha-r(w)]n - [1-r(w) +(a-\frac12)\alpha]n - \alpha  \ge (a-3)\alpha n \ge \alpha n.
    \end{align*}
    \end{proof}

\begin{claim}\label{clm::fixed-k-stoc-dom}
    For every node $v$ in $T$, $\qtilde(v)\ge q(v)$.
\end{claim}
\begin{proof}
We prove the result by an induction from the leaves to the root of tree $T$.

\smallskip\noindent
\emph{Base case: a leaf node}\\
At a leaf node $v$ all the random decisions have been made, so each woman has either proposed to $m$ or not. This results
in either at least $r$ proposals to $m$ or fewer than $r$ proposals; in the first case, $q(v)=1=\qtilde(v)$ and in the second case $q(v)=0=\qtilde(v)$.

\smallskip\noindent
\emph{Inductive step at internal node $v$}\\
Let $w$ be the woman making a random choice at node $v$.
Suppose $m$ has been proposed to $x$ times prior to reaching node $v$.
Then $\qtilde(v)$ is calculated using $s-x$ residual probabilities,
and for each child $u$ of $v$, $\qtilde(u)$ is calculated using $s-x$ residual probabilities, with the exception of the child $\overline{u}$ corresponding to a proposal to man $m$, where $\qtilde(\overline{u})$ is calculated using $s-x-1$ residual probabilities. Furthermore, in the calculation of $\qtilde(u)$, all the residual probabilities except at most one are unchanged; the only one that may change is due to the fact that $p(w,v)>p(w,u)$ at each node $u\ne \overline{u}$.

\smallskip\noindent
\emph{Case 1.} $p(w,v)$ is among the smallest $s-x$ residual probabilities at node $v$, and $p(w,u)$ is among the smallest $s-x$ residual probabilities at each child $u\ne \overline{u}$ of $v$.\\
One way to make the random choices involved in evaluating $\qtilde(v)$ is to determine if $w$'s utility for
$m$ equals the utility at node $v$; then, the probability that the remaining
$s-x-1$ residual probabilities at node $v$ generate at most $r-x-1$ proposals to $m$ is given by $\qtilde(\overline{u})$;
otherwise, at any child $u\ne \overline{u}$ of $v$, the probability that the $s-x$ residual probabilities generate at most $r-x$ proposals to $m$ is given by $\qtilde(u)$.
Thus $\qtilde(v)=\sum_{\text{$u$ a child of $v$}} p_u\cdot \qtilde(u)$, where $p_u$ is the probability that the edge to $u$ is followed.
As $q(v)=\sum_{\text{$u$ a child of $v$}} p_u\cdot q(u)$, it follows by induction that $\qtilde(v)\ge q(v)$ in this case.

\smallskip\noindent
\emph{Case 2}.  $p(w,v)$ is not among the smallest $s-x$ residual probabilities at node $v$, and $p(w,u)$ is not among the smallest $s-x$ residual probabilities at any child $u\ne \overline{u}$ of $v$.\\
At every child $u\ne \overline{u}$ of $v$, $\qtilde(u)=\qtilde(v)$, as these probabilities are being computed
using the same residual probabilities.
At node $v$, let $p_1\le p_2\le \ldots\le p_{s-x}$ be the residual probabilities being used to calculate
$\qtilde(v)$, the probability that at most $r-x$ proposals to $m$ are made. 
$\qtilde(\overline{u})$ is the probability that at most $r-x-1$ proposals to $m$ occur with the residual probabilities $p_1\le p_2\le \ldots\le p_{s-x-1}$.
This is smaller than $\qtilde(v)$ for even if $r-x$ proposals to $m$ occurred at $\overline{u}$,
with the same $s-x-1$ random decisions at node $v$, the probability $p_{s-x}$ choice at node $v$ could
result in another ``no proposal'', yielding a total of $r-x$ proposals.

So in this case
$\qtilde(v)>\sum_{\text{$u$ a child of $v$}} p_u\cdot \qtilde(u)$, but $q(v)=\sum_{\text{$u$ a child of $v$}} p_u\cdot q(u)$ still, and again by induction, $\qtilde(v)\ge q(v)$.

\smallskip\noindent
\emph{Case 3}.  $p(w,v)$ is not among the smallest $s-x$ residual probabilities at node $v$, but for at least one child $u\ne \overline{u}$ of $v$, $p(w,u)$ is among the smallest $s-x$ residual probabilities at $u$.\\
The difficulty we face is that if $p(w,u)<p_{s-x}$, then $\qtilde(u)>\qtilde(v)$, while
$\qtilde(\overline{u})<\qtilde(v)$, and if $p(w,u)>p_{s-x}$, then $\qtilde(u)<\qtilde(v)$.
So it would seem that to show
$\qtilde(v)\ge\sum_{\text{$u$ a child of $v$}} p_u\cdot \qtilde(u)$, and then by induction deduce that
$\qtilde(v)\ge q(v)$, we would need to know something about the relative sizes of the various $p_u$.
However, we will sidestep this obstacle by means of the following reduction.

What we need to show is that
\begin{align}\label{eqn::tree-dom-holds}
    \sum_{\text{$u$ a child of $v$}} p_u\cdot\qtilde(v)\ge\sum_{\text{$u$ a child of $v$}} p_u\cdot \qtilde(u).
\end{align}
Let's first remove the nodes $u$ for which $\qtilde(v)= \qtilde(u)$, i.e.\ the nodes $u$ for which $p(w,u)$ is not among the smallest $s-x$ residual probabilities.
Now, let's increase $p_{s-x}$ until it is equal to the smallest of the remaining $\qtilde(u)$.
This leaves the remaining $\qtilde(u)$ unchanged, as their smallest residual probabilities are unchanged.
However, it reduces $\qtilde(v)$ as the residual probability $p_{s-x}$ which is used in its evaluation is being increased.
We now remove the $u$ for which $p_{s-x}=p(w,u)$ and iterate.
Eventually, only node $\overline{u}$ remains.
But $\qtilde(\overline{u})<\qtilde(v)$.
Iterating through these changes in reverse order, we repeatedly increase $\qtilde(v)$,
and at each iteration add equal valued terms to each side. We conclude that \eqref{eqn::tree-dom-holds} holds.
\end{proof}

Now we obtain a high-probability upper bound on the number of women who fail to match.

\begin{lemma}\label{lem::women-interval-non-match}
Let $I=(b,b+\ell)$ be an interval of women, based on their public ratings, with $b\ge a\alpha$.
Let $g$ be the number of women in $I$.
Suppose ${\cal B}_1$ does not occur.
Suppose also that
\begin{itemize}
    \item $\ell= 6(c+2)\ln n\exp\big(1+k/[2a+\frac12]\big)/n$.
    \item $l \le \frac 12 \alpha$.
    \item $k\ge 2a + \frac 12$.
    \item $a\ge 3$.
    \item $n \ge\frac{k^2g}{(2a + \frac12 )\alpha}$.
    \item $\alpha\ge 4e\exp\big(-k/[2a+\frac12]\big)$.
\end{itemize}
Then, with failure probability at most $5n^{-(c+2)}$, at most $\frac 12 g\alpha$
of the women in $I$ fail to match in a run of the man-proposing double-cut DA.
\end{lemma}
\begin{proof}
The expected number of women in $I$ is $\ell n$.
Therefore, by a Chernoff bound, $g$, the number of women in $I$, is less than $\frac 12 \ell n$ with
probability at most $\frac 14 \ell n\le n^{-(c+2)}$.
Similarly, the number of women in $I$ is more than $2 \ell n$ with
probability at most $\frac 13 \ell n\le n^{-(c+2)}$.
In the remainder of this proof we suppose these bad events do not occur, and so $3(c+2)\ln n\exp\big(1+k/[2a+\frac12]\big)\le g \le 12(c+2)\ln n\exp\big(1+k/[2a+\frac12]\big)$.

We run the double-cut DA slightly differently here.
We include the men with public rating in the range $(b+\ell-a\alpha,b+a\alpha) \cup (b+\ell+a\alpha,1]$.
The first interval comprises those men for whom all of $I$ is in their cone, and the second interval
comprises those men whose cones are completely above $I$.
The participating women are those will public utility in the range $(b,1]$.
To ensure exactly this set of women participate, we cut at utility $b+1$ (recall that this is the utility the men are getting).
As ${\cal B}_1$ does not occur, the surplus is at least
$s = \big([1-b-\ell+(a+\frac12) \alpha] + [(2a-\frac 12)\alpha-\ell] - [1-b-\ell+\frac 12 \alpha]\big)n =[(a-\frac32)\alpha -\ell]n\ge \alpha n$.

Let $S$ denote the set of men in the surplus. 
We want to determine how many of the edges to $S$ go to a man receiving two or more edges.
Clearly, at most $kg$ men in $S$ can receive edges from $I$.
We can think of this as a process which randomly throws each edge to a set of bins of size at least
$(2a-\frac 12)\alpha n$ and which includes at least $s$ bins that correspond to $s$ men in $S$.
Let's imagine having each woman in turn make $k$ throws of edges. Now, let's consider the $k$ throws by the $i$th woman in $I$.
The probability that a throw is to an unused location in $S$ is at least $\frac{s - k(i-1)}{(2a + \frac12)\alpha n}
=\frac{1 - \frac{k(i-1)}{\alpha n}} {2a + \frac12}$, 
and therefore the probability that this woman has no edges to a single-edge recipient in $S$ is at most
$\Big(1-\frac{1 - \frac{k(i-1)}{\alpha n}} {2a + \frac12}\Big)^k
\le \exp\Big(-k\cdot\frac{1 - \frac{k(i-1)}{\alpha n}} {2a + \frac12}\Big)$.
These probability bounds are independent as they do not depend on the outcomes for the earlier women, and so we
can apply a Chernoff bound.
The expected number of women with no such edges is at most $g$ times this probability,
and the probability that there are more than $2g \exp\Big(-k\frac{1 - \frac{k(g-1)}{\alpha n}} {2a + \frac12}\Big)$ such women is at most
$\exp\Big[-\frac 13g \exp\Big(-k\cdot\frac{1 - \frac{kg}{\alpha n}} {2a + \frac12}\Big)\Big]$.
As $\frac{k^2g}{(2a + \frac12 )\alpha n} \le 1$, the probability bound is at most $n^{-(c+2)}$.
Also, the number of women is at most
$2g\exp\big(1-k/[2a+\frac 12]\big)$.
As $\alpha\ge 4e\exp\big(-k/[2a+\frac12]\big)$, this is at most $\frac 12 g \alpha$ women.

The overall failure probability bound is at most $5n^{-(c+2)}$.
\end{proof}

\begin{lemma}\label{lem::women-high-value-match-prob}
    Let $w$ be a woman with public rating at least $a\alpha$.
    Suppose that ${\cal B}_1$ does not occur.
    Then she fails to receive a match with probability at most
    $exp\big(-k\frac {a-1}{2a+\frac12} \big)$.
\end{lemma}
\begin{proof}
    Consider running the man-proposing double-cut DA with a cut at $w$, using men with public rating
    at least $r(w)-a\alpha$. As ${\cal B}_1$ does not occur, the surplus is at least $(a-1)\alpha n$.
    Now let's calculate the probability that none of $w$'s edges go to the surplus men.
    It's given by:
    \begin{align*}
        \Big(1 - \frac{(a-1)\alpha n} {(2a+\frac 12 a)\alpha n}  \Big)^k \le \exp\big(-k\frac {a-1}{2a+\frac12}\big).
    \end{align*}
\end{proof}

\begin{lemma}\label{lem::outcome-woman-prop-DA}
 For each woman $w$ with public rating at least $a\alpha$, her outcome in the run of the full woman-proposing DA
 is at least as good as her outcome in the man-proposing double-cut DA for $w$.
\end{lemma}
\begin{proof}
    Because every man who proposed to $w$ in the double-cut DA prefers her to women with a lower public rating,
    adding additional woman does not affect the proposals $w$ receives. And adding additional men can only improve the proposals she receives. So $w$'s outcome in the full man-proposing DA is only better than her outcome in the double-cut DA.

    But the outcome in the full man-proposing DA is the worst stable matching for $w$.
    Therefore the outcome in the full woman-proposing DA can only be better.
\end{proof}

We first show that for a non-bottommost woman, a woman with public rating at least $a\alpha$,
changing strategies will not significantly improve her outcome in expectation.

\begin{lemma}\label{lem::typical-woman-eps-nash}
    Let $w$ be a woman with public rating at least $a\alpha$.
    In expectation, ex-ante, $w$ could improve her utility by at most $2a\alpha+52\exp\big(-k\frac {a-1}{2a+\frac12}\big)$.
\end{lemma}
\begin{proof}
  By \Cref{lem::high-cap-men-outcome}, with probability xxx all the men above $w$'s cone are matched to women above $w$.
  Therefore these men would reject a proposal from $w$.
  For a man in-cone, ex-ante, if she is matched, her utility could increase in expectation by at most $2a\alpha$.
  If she is not matched, her expected gain is at most $\big(r(w)+\frac32\big)\cdot\exp\big(-k\frac {a-1}{2a+\frac12}\big)\le \frac 52\exp\big(-k\frac {a-1}{2a+\frac12}\big)$, using \Cref{lem::women-high-value-match-prob} to bound her non-match probability.
  Below cone, if she is giving up an in-cone match, her gain is at most $\taubar$ in expectation,
  and if she is replacing a non-match, her gain is at most $\frac 52\exp\big(-k\frac {a-1}{2a+\frac12}\big)$.
\end{proof}
\noindent
\emph{Comment}. This is not to imply that there is a strategy that enables this size of improvement.
We conjecture that the possible expected improvement is in fact $O(\exp(-O(k))$.

The strategies of the bottommost women do not affect the bounds on the gains of higher up women, so it does not have a broader impact whether they follow the designated strategy or not. The only potential impact is on the men with public rating in the interval $[a\alpha, 2a\alpha)$, for whom the claim that they are fully matched may no longer hold.
But this has no impact on the women with public rating at least $a\alpha$.
It also means that if the modeling of these bottommost women is not particularly accurate, it does not affect the results for the remaining women.
Still, we give a bound on the match probabilities for the bottommost women and deduce bounds on their expected gains.

\begin{lemma}\label{lem::bottom-women-gains}
    Let $w_i$ have the $i$th smallest public rating. If $i\ge (2a+\frac 12)\alpha n/k$ her probability of failing to match
    is at most $\exp\big(-k\exp\big(-ki/(2a+\frac 12)\alpha n\big)$, and if $i<(2a+\frac 12)\alpha n/k$, her probability of matching is still $\Theta(1)$ with probability $n^{-(c+2)}$, if $n\ge \frac{4(c+2)k e^{1+1/k}} {\alpha (a + \frac 12)}$.
\end{lemma}
\begin{proof}
    Suppose we run the woman-proposing DA, allowing each women in turn to propose continuing until she matches
    or goes through all $k$ of her proposals. Consider what happens when woman $w_i$ makes her proposals. Given that the men above her cone are fully matched, it must be
    that there are at least $i$ unmatched men in $w_i$'s cone; as her private values provide a uniform
    random selection among the men in her cone, the probability that she fails to match is at most
   $\big(1 - \frac {i}{(2a+\frac 12}\alpha n\big)^k \le \exp\big(-ki/(2a+\frac 12)\alpha n\big)$.
    
    To get a $\Theta(1)$ bound for $i<(2a+\frac 12)\alpha n/k$, we argue as follows.
    Suppose there are no more than $(a-\frac 12)\alpha n/k$ unmatched men remaining.
    Then $w_i$ fails to match with probability at least $(1-\frac 1k))^k\ge e^{-(1+1/2k)}$, for $k\ge 2$.
    If there are at most $\frac 12 (a-\frac 12)\alpha n/k$ unmatched women when the number of unmatched men is first reduced to  $(a-\frac 12)\alpha n/k$, then at least $\frac 12 (a-\frac 12)\alpha n/k$ remain unmatched.
    Otherwise, in expectation at least $e^{-(1+1/2k)}\cdot \frac 12 (a-\frac 12)\alpha n/k$ women and therefore men
    remain unmatched, and by a Chernoff bound, the probability that fewer than $\frac 14 e^{-(1+1/2k)}\cdot (a-\frac 12)\alpha n/k$ women (and men) remain unmatched is at most 
    $\exp(-\frac 14 e^{-(1+1/2k)}\cdot (a-\frac 12)\alpha n/k)\le n^{-(c+2)}$, if $n\ge \frac{4(c+2)ke^{1+1/k}}{\alpha (a + \frac 12)}$.
\end{proof}
}

\hide{
\newpage
\subsection{The School Choice Setting}

Here we suppose that one side (the men) has utilities determined solely by the public ratings for the other side (the women). In addition, we focus on the high capacity case on the men's side: we suppose each man has a capacity
$\kappa =\Omega(\ln n)$.

In this case, a good parameter choice is to have $\alpha =\Theta(\ln k/k)$.
We will find that all but some of the bottommost men are fully matched with high probability
(the possible exceptions are those men with public ratings less than $a\alpha n$).
For the non-bottommost women, the individual probability of failing to match will be at most $e^{-k(a-1)/2a}$.
For the bottommost women, the match probability will gradually reduce to a constant in the range
$(1/e^2,1/e)$ as their public ratings decrease to 0.
We can also deduce a type of $\epsilon$-Nash equilibrium:
for all but the bottommost women, $\epsilon= O(\alpha)$, regardless of what the bottommost women do.
For the bottommost women, $\epsilon$ is the minimum of $O(\alpha)$ and 1 minus their match probability.
Note that for the bottommost women, this is the bound we can show; it does not mean that we see an improved
strategy that they might follow.

Each woman will choose the edges with the highest private values in her window as the men with whom to interview.
Then, because the range of the interview values is significantly larger than the range of the public ratings in her window, and the (much smaller) range of the highest private values, the ordering of her edges for the DA algorithm will be largely driven by her interview values. This might seem counter-intuitive. It is natural to ask whether the parameter $\phi$ governing the contribution of the interview values should be significantly smaller.
But in fact the correct response to a smaller $\phi$ is to have $\alpha =\Theta(\phi \ln k /k)$, so long as $\phi=\Omega(\sqrt{kn})$. The interview values continue to govern the ordering of each woman's proposals.

Let ${\cal B}_3$ be the event that some man with public rating $a\alpha$ or larger is not fully matched.
Let ${\cal B}_4$ be the event that more than $2e^{-k(a-1)/2a}n$ women with public rating $a\alpha$ or larger are not matched.

\begin{lemma}\label{lem::some-man-not-fully-matched}
    ${\cal B}_3$ occurs with probability at most $n^{-(c+1)}$.
\end{lemma}

\begin{lemma}\label{lem::many-women-not-matched}
    ${\cal B}_4$ occurs with probability at most $n^{-(c+1)}$.
\end{lemma}

\begin{lemma}\label{lem::non-match-prob-bottommost-women}
With failure probability at most $n^{-(c+1)}$,
each bottommost woman fails to match with a probability at most $1/e^{1/2e}$. \rnote{Need to update.}
\end{lemma}
\begin{proof}
Suppose there are $\overline{n}$ bottommost men. If ${\cal B}_1$ does not occur, then $\overline{n}\ge (2a-1)\alpha n$.
  Consider the situation when only $\overline{n}/k$ men remain unmatched. 
  Let $\tilde{n}$ be the number of unmatched bottommost women at this point.
  Necessarily $\tilde{n} \le \overline{n}$.
  They are all in the window of the bottommost women
  as higher up men are all matched. Each woman, using her private values, chose a random subset of these men to propose to uniformly at random, and in expectation, $k$ of them.
  The probability that she fails to match is $(1- 1/k)^k\ge e^{-(k+1)/k}$, if $k\ge 3$.
  \rnote{This bound is correct for the choose k edges setting.}
  In expectation at least $\tilde{n} \cdot e^{-(k-1)/k}$ of these women fail to match,
  and therefore, in expectation, the number of men that remain unmatched is at least
  \begin{align*}
  \frac{\overline{n}}{k} - \tilde{n} e^{-(k+1)/k} 
  \ge \frac{\overline{n}}{k}\big(1 - e^{-(k+1)/k}\Big).
  \end{align*}
  By a Chernoff bound, the probability that fewer than $\frac 12 \cdot \frac{\overline{n}}{k}\big(1 - e^{-(k+1)/k}\Big)$ men remain unmatched is at most
  $\exp\big(-\frac {1}{16}\cdot \frac{\overline{n}}{k}\big[1 - e^{-(k+1)/k}\big]\big)$.
  Call this bad event ${\cal B}_5$.

  Assuming ${\cal B}_5$ does not occur, the probability that a woman fails to match is at most
  \begin{align*}
      \Big[1 - \frac 12 \cdot \frac{\overline{n}}{k}\big(1 - e^{-(k+1)/k}\Big)\Big]^k
      &\le \exp\Big(-\frac k2 \cdot \frac{(2a-1)\alpha n}{k}\big[1 - e^{-(k+1)/k}\big]\Big)\\
      & \le \exp\Big(-\frac{(2a-1)\alpha n}{2}\big[1 - e^{-(k+1)/k}\big]\Big)
  \end{align*}
\end{proof}
}

\subsection{Approximate Nash Equilibrium}

We show that on choosing the parameters suitably,
the non-bottommost women achieve an $\epsilon$-Nash equilibrium with
$\epsilon = O(\ln k/\sqrt{k})$.
We set $\sigma_m=\sigma_w= 4\sqrt{\ln k}/\sqrt{k}$.
\rnote{We need another lemma on the probability of not obtaining an edge that gives both the man and woman a loss of at most $1-a\sqrt{\ln k/k}$; this probability is $1/k^{O(1)}$.}
We set $\alpha=\sqrt{\ln k/k}$.

Now consider what happens if a women $w$ proposes to a man $m$ above her cone.
With probability at least $1- 1/k^{O(1)}$, $m$ has received a proposal with utility greater than $r(w)+1$,
and therefore will reject the proposal from $w$.

\subsection{The Outcome for the Bottommost Women}

We show that in the high-capacity setting, 
the women with public rating less than $2a\alpha n$ also have a good probability of matching.

The first observation is that all the men with public rating more than $2a\alpha n$ are fully matched with high probability when we run the woman-proposing double-cut DA.
This implies that at the end of the run of the double-cut DA, the number of unmatched woman who still have available proposals is at most the number of unmatched men, who all have public rating less than $2a\alpha$.

Let us first allow the unmatched women with public rating at least $2a\alpha$ to continue proposing.
The previous matching bounds for the man-proposing double-cut DA, implies that there are at most $n e^{-\nu\sqrt{k}}$ unmatched women at the end of this step, for a suitable constant $\nu>0$, and each of these women obtains utility
$1-O(d\sqrt{k})$ with probability $1-1/e^d$.

Let us consider what happens with each of the remaining women. We will show that the outcome is quite similar to what happens in the setting with random private values and no common component to the values.
The reason is as follows. Each woman selects her edges based on her private values and this causes a uniform random selection over the in-cone men, and in particular for the men with public rating at most $2a\alpha n$.
Then, each woman orders her proposals based on her overall utility.
The most significant component of her utility for the selected edges is the interview component, for it varies from $[0,1]$,
whereas the variation in public rating is in the range $[0,2a\alpha)$, and the variation in private value is in the range 
$[1-\tau,1]$. This ensures that the ordering of the edges is going to be similar to that in the random value case.
In a similar way, each man's ratings for the proposals he receives are going to be largely driven by his interview corrections, because again the public ratings are in the range $[0,2a\alpha)$, while the interview components are in the range $[0,1]$.

\bigskip


\noindent
Results with exactly $k$ proposals. \\
Idea: Use individual $\tau$ values for the women and in the women-proposing DA, block the women with the largest values of $\tau_i$. w.h.p., the  results are only a little worse. For the man-proposing case, each woman has her own value of $\tau_i$ and this determines her individual match rate. For the interval bound when man-proposing, the bound depends on the $\tau_i$ values. w.h.p., in each interval only an $2e^{-k/6}$ fraction of the women have $\tau_i<\tau/2$.
For the remaining women, a man's proposal is distributed roughly uniformly, which suffices.

\smallskip
\noindent
The high-capacity scenario.\\
Suppose each man has capacity $c$, and $ck=\Omega(e^{\beta k}\ln n)$.
The woman's proposal probability is increased by a factor of $c$. This reduces a man's non-match rate to be polynomially small in $n$. i.e.\  w.h.p.\ all but the bottommost $3a\alpha$ men match.
For the man proposing case, the interval bound needs the most care. But so long as the intervals $I$ are $\nu\cdot a\alpha /(ck))$ in length, the probability that a man makes two or more proposals to $I$ is $O(\nu^2)$, which leaves an adequate surplus. (This needs checking.)

\smallskip\noindent
$\epsilon$-Nash bounds. The priority is the high-capacity case.\\
1. The interview case.\\
a. No men idiosyncrasy.\\
Then women cannot bump higher up women, which means a polynomially small probability of gain from applying above one's cone. Since, the failure rate for non-bottommost women is $\exp(-\beta k)$, this suffices as the $\epsilon$ for all but the bottommost women. 
Because, there are no mismatches among the men apart from the bottommost, there are at least as many slots for women as there are bottommost women. Therefore random proposals, which is basically what is happening: private values are used to select a random subset of bottommost men, then the interview ratings cause a near uniform random distribution over this selection. This means the women cannot do much better than follow the recommended strategy. \rnote{This has to be analyzed more closely.}\\
b. Men have idiosyncrasy.\\
Here we need a much larger $\epsilon= \Theta\big(1/\sqrt{k}\big)$. Then the probability that a non-bottommost man does not receive
a match with private value at least $1-1/\sqrt{k}$ is $\exp\big(-\sqrt{k}\big)$. Then the expected gain from a woman proposing above her cone is $O(1/k\sqrt{k})$ per proposal, and so is not worthwhile. For a non-bottommost woman, proposing below is also not useful, as her match probability is $1-\exp(-\beta k)$.
For the bottommost women, the men's idiosyncrasy means that they have a good probability of bumping, so this becomes quite similar to the random case; following the strategy leads to an $\exp\big(-\Theta(\sqrt{k})\big)$ mismatch probability.
\\
Another case to consider is non-equal capacities. My guess is that so long as they are all large enough, it does not matter.\\
2. The no-interview setting.\\
Now, at the bottom, the women's proposals are more or less in men's public rank order.
I am not yet clear on how to analyze this. Definitely a less important setting given the motivation for the problem.
